How Does Automation Shape the Process of Narrative Visualization: A Survey of Tools

In recent years, narrative visualization has gained much attention. Researchers have proposed different design spaces for various narrative visualization genres and scenarios to facilitate the creation process. As users' needs grow and automation technologies advance, increasingly more tools have been designed and developed. In this study, we summarized six genres of narrative visualization (annotated charts, infographics, timelines & storylines, data comics, scrollytelling & slideshow, and data videos) based on previous research and four types of tools (design spaces, authoring tools, ML/AI-supported tools and ML/AI-generator tools) based on the intelligence and automation level of the tools. We surveyed 105 papers and tools to study how automation can progressively engage in visualization design and narrative processes to help users easily create narrative visualizations. This research aims to provide an overview of current research and development in the automation involvement of narrative visualization tools. We discuss key research problems in each category and suggest new opportunities to encourage further research in the related domain.

==> 01-Notes.tex <==
%-----------------------------20221112开会内容--------------------------------------
% 1. 按照之前收集论文的那种方式写（我的design space、authoring tool，你的AI—supported tool，AIgenerator），最后写出来内容后，会统一矫正全文的逻辑

% 2. 商业类工具如果是分散在每一个类型中的话就放进去，如果都是集中在一个类型中，就少放一些，全文中的商业类工具最好不要超过10个。

% 3. 之前的分类中Infographics中的3个类型（magazine-style、annotated chart，infographic） 现在需要重新划分一下。取消掉Infographics的大类，把magazine-style和Infographic合并在一起，annotated chart归类到Chart中。

% 4. 再做一张表格，把之前做的timeline以表格的形式进行呈现，其中关于的design space,authoring tool, ai-supported tool, ai generator,四个类型的年份也要标注出来（就是相当于table1和table2的结合体）
% 5. introduction这部分内容陈老师之后写，关于2.2和2.3的内容，咱们在之后写完各类型的内容后返回来写这部分东西【2.2的内容是写咱们和已经有的survey文献的差异点事什么；2.3的内容是咱们如何去收集文献的、如何筛选的论文等过程的一个描述】
% 6. 每一个类型中的design space、authoring tool, ai-supported tool, ai generator, 需要有一个小的总结， 这一个类型全部写完后需要有一个总的总结（总的总结内容是：现有的不足+未来的方向；或者是在哪些领域中研究较多，哪些领域中研究相对缺乏；在研究多的领域中还存在怎样的问题）



%----------20221212开会内容----------------%

% design space:
%Design space的概念是用来强调从许多选项中选择和探索替代方案的自由(例如:Fischer & Giaccardi 2004, McKerlie & MacLean 1994, Sanders 2001, Westerlund 2005)。 有时它似乎也指的是设计过程中的所有与设计相关的信息(如Hassenzahl & Wessler 2000)。 另一个常见的用法是将其描述为一个在过程中因项目变化而扩展和收缩的领域(例如:Gero & Kumal 1993)。 设计空间描述了所有可能的设计选择。定义设计空间的最普遍的策略是从一组现有的可视化技术中提取共同的设计原则。一旦确定，这些共同的原则就可以作为轴来跨越设计空间。除此之外，可视化设计空间使我们能够捕捉到可视化设计师的一些隐性知识。一旦被明确，设计空间就可以被用来访问原本分散的、庞大的可视化技术集（Schulz, H.2011）。在本研究中，我们认为designspace是试图从计算机的角度去理解一副设计作品，也就是将一副设计作品解构成若干设计元素， 以及对于这些元素的排列组合。一个清晰的设计空间会让设计变得结构化而且有规律可循，可以让设计师在进行设计创作时不再依靠感觉进行，是让计算机读懂设计并最终实现自动设计的基础。

% authoring tools: Authoring tools encapsulate key software functionalities and features for content creation (Zikas, P.,2020).它是指为针对用户的某种特殊应用目的所撰写的应用程序。它可以和用户进行交互，一般具有可视的用户界面。每一个Authoring tools运行于独立的进程、他们拥有自己独立的地址空间，用户可以借助Authoring tools进行自由创作。

%AI supported tool：AI Supported tool是基于Authoring Tools的一种由算法支撑的工具， 在创作过程中， 会针对某一环节内容提供推荐方案，最终通过用户自行组合设计内容，构成完善的可视化设计方案。

% AI generator：
% AI generator tools是一种更智能的创作用具，在整个创作过程中，用户几乎不需要参与决策或参与少量决策。当用户上传数据后，AI generator tools会对数据进行自动化分析与处理，在不借助用户干预的情况下可以生成一套完整的可视化设计方案。

%【针对于单个图表】
%1. 自动选取数据中的信息  + 2. 自动生成数据可视化的编码
%【针对于Dashboard】
%1.自动选取数据中的信息+自动生成数据可视化的编码
%2. 生成相关图表之间的逻辑，不能是简单的布局


%----------20220114----------------%

% Authoring tools -> Basic Authoring tools

% fact sheet归类到data comics中（参考文献：ChartStory: Automated Partitioning, Layout, and Captioning of Charts into Comic-Style Narratives）将多个可视化并置到一系列面板组成的连环画布局中，每个面板都适当的有注释和装饰的视觉和文本元素，并排列成一个序列，逐步介绍漫画中讲述的主要故事，尽管传统的漫画可能会有很多的装饰，但是在叙事性可视化中，即使存在少量漫画元素的fact sheet也属于data comic的一种类型。



%%----------20220119----------------%
%1. \cite{zhao2020iconate} %这是关于多维icon的生成，是否要放到glyph中（保留）
%2. 杂志风格找到了3篇文献，是同一组人进行的研究，3篇文献围绕共同的一个主题：自适应干预措施对用户识别杂志风格叙事可视化的影响。论文中没有提到关于杂志风格的design space，这类型的是否放到survey中。（去掉）
%3.treemap等可视化图表是否也进行survey 



%-----------20220121-------------%
% \cite{satyanarayan2014authoring} 这生成的是什么内容
% \cite{bostock2011d3} D3什么图表都可以生成，应该放到哪一类？

%20220123任务：完成Data comics+Data viedos

% 1. InfoMotion，它可以自动将静态信息图形转化为动画演示。这一类应该放到infographic中还是data video中？如果从呈现形式来看，更像是data GIF，目前data gif是归类到了data video中？—— 目前是把它放到了data video中，因为将静态转化为动态还有一个软件data animator也在data video这个章节中。

%2.有些文献中，作者在开发Authoring tools前面会先介绍设计空间，Authoring tool是基于这样的设计空间进行开发的，在论文写作时，应该是把设计空间和Authoring tool放在Authoring tool部分一起进行说明呢，还是要分成两段，分别介绍内容是什么。例如\cite{ren2017chartaccent}

%20220124任务：完成annotated chart（OK） + Glyph（OK）

%20220125：完成Timeline（OK）

%20220126-0127任务：Infographic
%把flow chart归类到infographic中


% \cite{yuan2021infocolorizer} To facilitate the creation of an aesthetic infographic, researchers have developed many authoring tools, which fall into three main categories:\textbf{ programming toolkits, interactive design environments, and semi- or fully-automated tools.} authoring tools -> interactive design environments? 为了促进审美信息图形的创建，研究人员已经开发了许多创作工具，它们分为三个主要类别:编程工具包、交互式设计环境和半自动化或全自动工具。}编辑工具->交互式设计环境?
 
% \cite{tyagi2021user}  The manual tools have a steep learning curve and require a high level of expertise to design infographics from scratch, hindering the adoption of novice designers. The semi-automated approaches focus on automating low-level designs, making it easier for novice designers to create infographics, but they only support either a particular class of infographics or specific pieces within an infographic. On the other hand, the fully automated techniques have the fastest turnaround time for generating infographics, but they are limited by prescribed whole-infographic templates, restricting users’ freedom.  authoring tools -> manual tools? 手工工具有一个陡峭的学习曲线，需要高水平的专业知识从头开始设计信息图，这阻碍了新手设计师的采用。半自动化的方法专注于自动化低级设计，使新手设计师更容易创建信息图，但它们只支持特定类型的信息图或信息图中的特定部分。另一方面，完全自动化的技术在生成信息图方面有最快的周转时间，但它们受到规定的全信息图模板的限制，限制了用户的自由。
 
% \cite{zhu2020survey} [ Firstly, programmatic step for visualizing data includes imperative languages and libraries. Designers need to have an ability of programming to get infographics, These tools are designed for users who are familiar with coding and visualizations. Secondly, visual building step for easy visualizations includes template editing,These tools are designed for users who are familiar with coding but not familiar with visualizations. Thirdly, the semi-automatic step is involved with few interactions to efficiently obtain visualizations. Lastly, automatic step is designed for no-human involved tools to efficiently get visualization recommendations These tools are gradually emerging for users who are not familiar with visualization or coding.  首先，可视化数据的编程步骤包括命令式语言和库。设计师需要有编程的能力来获得信息图形，这些工具是为熟悉编码和可视化的用户设计的。其次，便于可视化的可视化构建步骤包括模板编辑，这些工具是为熟悉编码但不熟悉可视化的用户设计的。第三，半自动步骤涉及很少的交互，有效地获得可视化。最后，自动步骤是为不需要人工参与的工具设计的，以有效地获得可视化建议。这些工具是为不熟悉可视化或编码的用户逐渐出现的。

%类似于tree&networks这样的内容是在一个章节中，将tree和networks分开进行阐述各自的design space等呢还是将两部分内容融合在一起进行说明呢？

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
20220128 之后的内容
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Task List
%20220131-0201 写Map模块的内容
%20220202-0203 写Text（Tag Cloud）的内容
%20220204-0205  写Statistical Chart的内容
%20220206 写了data comics和data video的Summary
%20220207 写Scrollytelling的内容
%20220208-0209 写dashboard的内容
%20220211-0212 写Graph的内容（Node-link diagram、adjacency matrix、nodetrix、heatmap）
%20220213 写Tree可视化的内容
%20220214 写Immersive可视化内容+重新制作3张表格

疑问：
% 1. \cite{hullman2013contextifier} 应该是AI supported tools还是 AI -generator tools
% 2. 变更：有两篇关于Table的文献，文中所提到的工具是将table转化成了常用的Chart，根据工具类型划分，放到Statistical chart中更为合适。如果把table的内容放到chart中，那这部分就只能以text或tag cloud命名了。
% 3. slideshow中有两篇文献不确定：
% Semantic High-Level Features for Automated Cross-Modal Slideshow Generation./ Generating Audio-Visual Slideshows from Text Articles Using Word Concreteness 这两篇文献与我们的研究是否有关。
% 4. ToonNote: Improving Communication in Computational Notebooks Using Interactive Data Comics（在展现形式上很像Scrollytelling）。
% 5. treemap中的拓扑结构是什么？
% 6.很多论文是把matrix和node-link放在一起进行研究，咱们的内容是否要合并。关于treemap这部分的内容，大部分的研究是基于算法，有点不太好理解。
% 7.是否可以network和matrix合并在一起，称为graph visualization。单独把tree拿出来称为Tree visualization。 好几篇论文中都把network等同于graph(AniMatrix: A Matrix-Based Visualization of Software Evolution) 
% 把Node-Link and Matrix结合在一起的文献：（A Comparison of the Readability of Graphs Using Node-Link and Matrix-Based Representations）
% 8.Borkin 将 heatmap归类到了Grid & Matrix一类中，但是不清楚graph vis 中是否可以将heatmap包含进去。
% 9. Immersive可视化这部分的内容有些不太理解，从论文整体框架来看，感觉Immersive内容很突兀，不像是这篇论文中应该有的内容。
%10.是否还要放通用可视化设计指南，现在是将其单独放到了Chart章节的上面
%11.类似于tableau这一类的工具，既可以生成statistical chart，也可以生成dashboard，在表格中应该放到哪一部分好呢？
%12. \cite{shu2021dancingwords} 这个应该是authoring tools还是supported tools

%%%%%%%%%%%%%%%%%%%%%20220216%%%%%%%%%%%%%%%%%%%%
%slideshow这部分内容中，关于PowerPoint,Keynote,google slide这样的工具是否是我们所讨论的范围呢？而且关于scorytelling也更多的是在阐述narrative，并非是data visualizaiton。
%tree的研究并不是只针对于treemap，主要集中于可视化技术、视觉编码、空间布局3个层面进行的，现在是将3部分分开进行阐述了，所以保留了很多关于设计空间的文献。

%20220217 - 20220224：完成了正文的部分的初稿
%疑问：graph中是否要把heatmap添加进去？现在的graph中是node-link，adjacency matrix，nodetrix三个部分，三部分都是用来表示数据元素之间的关系的。heatmap是否也属于这一类呢（具体来说heatmap可以充当adjacency matrix的一个子元素吗）？如果放在graph中不合适，heatmap是否要去掉呢还是在新增一个小节去单独阐述这个内容呢？

%有一些工具开发出来的时间特别早，例如\cite{ahlberg1996spotfire}\cite{datapine2012}\cite{thoughtspot2012}\cite{QlikSense2010}，是在后续版本迭代过程中逐渐添加了很多的功能。像这一类的工具放在table2和table3中，就感觉在2010年就出现了generator的tools，可能会产生误解。

%20220225之后的内容
%1. 重新制作了表格
%2. introduction中的design space、Authoring tools、AI-supported、AI-generator的定义
%2. 整理了下面的工具所得出的future work


%statistical chart、text、graph、tree、Infographic、annotated chart、Dashboard、Scrollytelling、

%工具多的可以结合总结出来一些内容，工具少的map、Immersive两部分很难通过tools总结出相应的design space。

%待解决：Timeline、glyph、data videos。



%glyph中：\cite{ropinski2011survey}  \cite{maguire2012taxonomy}这两个是探讨医学和生物学领域的glyph，好像是属于科学可视化的相关内容，在我们的研究中这一类的是否要放呢？

Related Survey的参考文献。设计领域的design space和可视化领域的design space





As the demand for rapid analysis of visualization grows, there is an increasing requirement to design visualization tools, which allow users to efficiently generate visualizations. 

Shown in Fig. 1, authoring tools are increasingly towards automatic. The evolution of them can be divided into four steps. 

%Firstly, programmatic step for visualizing data includes imperative languages and libraries. Designers need to have an ability of programming to get infographics, such as D3 (Bostock et al., 2011), VegaLite (Satyanarayan et al., 2016), ECharts (Li et al., 2018), and VisComposer (Honghui et al., 2018). These tools are designed for users who are familiar with coding and visualizations. 

%Secondly, visual building step for easy visualizations includes template editing (iCharts (García et al., 2007) and RAWGraphs (Mauri et al., 2017), shelf configuration (Polestar (Pioch and Everett, 2006), Voyager (Wongsuphasawat et al., 2015), and Voyager 2 (Wongsuphasawat et al., 2017)), visual building (iVisDesigner (Ren et al., 2014), Data Illustrator (Liu et al., 2018), VisComposer (Mei et al., 2018a), and Charticulator (Ren et al., 2018a)). These tools are designed for users who are familiar with coding but not familiar with visualizations.
Users need to pre-conceive blueprints, then interact with the system, such as clicking or dragging with visual items, to get more expressive and aesthetic visualizations.

Thirdly, the semi-automatic step is involved with few interactions to efficiently obtain visualizations, such as SAGE (Roth et al., 1995) and BDVR (Gotz and Wen, 2009). 

Lastly, automatic step is designed for no-human involved tools to efficiently get visualization recommendations, such as Text-to-Viz (Cui et al., 2019) and Click2Annotate (Chen et al., 2010a). These tools are gradually emerging for users who are not familiar with visualization or coding.


%%%%
• Diversity-supporting of input datasets: A measurement is required on diversity-supporting involved with types (such as numeral data, textual data, images, and video), format(such as JSON, CSV, and hybrid format) and content(such as timeline, geographic, and network) of data.

• The degree of automation during the process: Qualitative or quantitative measurements are required to reveal how intelligent the techniques are in terms of the procedure of inputting datasets to outputting visualizations.

• The quality of output visualizations: Expressing information correctly is the most important condition for automatically generating a visualization. Meanwhile, other criteria are also required, such as comprehensivity (Bateman et al., 2010; Borkin et al., 2013), aesthetic (Harrison et al., 2015), and creativity-supporting (Borgo et al., 2012).

• Learnability of models: Automatically generating visualizations needs to reduce the user’s learning input as much as possible (Chen et al., 2009).


1.重新写text部分的设计空间。(完成)
2.补充Authoring tool和ai-supported的概念；再去找一下有没有类似地替换词
3.完成data video、Timeline、glyph 3部分summary

Authoring tools -> manual tools \cite{tyagi2021user} %Infographic generation tools can be classified into three main categories: manual, semi-automated, and fully automated tools.
AI supported tools -> semi automated tools.\cite{yuan2021infocolorizer} \cite{tyagi2021user} \cite{zhu2020survey}(semi-automatic step)
AI generator tools -> fully automated tools. \cite{yuan2021infocolorizer} \cite{tyagi2021user} \cite{zhu2020survey}(automatic step)


% User centric Semi-Automated Infographics Authoring and Recommendation(里面有对3款工具的定义)

% 根据\cite{satyanarayan2019critical}的描述，可视化创作有编程式和工具式（交互式系统）两种。工具式中又可以分为手动工具，辅助工具，全自动工具。

%疑问：这篇文献中所探讨的是关于叙事性可视化的相关工具，但是chart中的statistical chart、graph、tree、tag cloud，Infographics中的glyph、以及dashboard这几部分内容并不是很明确的就是用来指示叙事性可视化的相关内容。

%按照\bibliographystyle{unsrt}这样的方式排列之后，参考文献的作者变成了全称

%写完了RELATED SURVEY的内容

%为什么要从narrative的角度写这些内容？

%关于分类这块有疑问，不知道如何去叙述为什么要加glyph和Immersive narrative两部分内容，dashboard放在chart中可能会更好


%信息图主要是用图形设计的图标、图像、颜色和元素来说明数据和文本信息。
%现有分析的内容只有statistical chart和annotated chart有编程工具

1. other chart(text&map&graph&tree)这部分内容没找到一个合适的逻辑可以把这些串在一起
2.现在的表格中没有放编程工具，但是在论文中提到了编程工具(Statistical chart、annotated chart)


1.偏叙事性
2.偏探索性（最右侧：复杂的可视化分析工具）
dashboard中部分叙事部分探索，会讨论。
想一个场景，为什么要用这个内容。使用这张表的用户

四象限

上方：叙事？
下方：探索？

左侧：设计者
右侧：分析人员

timeline < dashbaord < annotated chart = Infographics = Scrollytelling < data comics < data videos

complexity
statistical chart/glyph < other charts/timeline < annotated chart/dashboard/infographic/scrollytelling < data comics < data video

narrative (exploratory -> explanatory)
statistical chart/other chart/glyph < dashboard < annotated chart < infographic/timeline/scrollytelling < data comics/data video

复杂性
统计图表/字形<其他图表/时间线<带注释的图表/仪表盘/信息图表/ scrolllytelling <数据漫画<数据视频

叙述性(探索性->解释性)
统计图表/其他图表/字形< dashboard <带注释的图表< infographic/timeline/scrollytelling < data comics/data video


future work: narrative workflow

工作：
1.画四象限的图及图标

%motivation 
- traditional visualizations are the foundations of narrative visualization
- abundant research on guidelines and AI tools for traditional visualization
- but for narrative visualization, the research is still lacking

- case: why use creation tools for narrative visualization (effective, efficient, without technical background)



other/ 新兴类型(immersive\ data 实物可视化- Physical visualization \ 游戏)

多媒体 multimedia（声音）

工具的icon
design space-人工（简单）



8个可视化的代表性图。table3隐藏，表格2中使用色彩进行区分工具，加other部分的内容。

20220418修改内容：
% 1.fig2中横轴和纵轴的sum色彩更改 （搞定）
% 2.fig3：Dashboard、Annotated chart、Scrollytelling、data comics、Network、treemap的图标更改；pie和bar两个合并在一起；Timeline和map保持水平(搞定)
% 3. fig6中的1图替换成timeline的结构图；3图换成Timeline和storyline各一张图 （搞定）
% 4.fig9 的1图缩小 (搞定)
% 5. 按照可视化的难以程度进行排序(搞定)
% 6.在calliope工具部分，添加一段说明fact sheet归类到data comics的内容(搞定)
% 7.将LAN的6种叙事形式、scrollytelling的fig1、A Design Space for Applying the Freytag's Pyramid Structure to Data Stories\ Visualizing Nonlinear Narratives with Story Curves 内容单独拿出来放到2.3.1章节



20220420:
% 1.dashboard - 实时性  在tableau中的故事板 + storytelling \cite{suprata2019data} \cite{fernandez2022beyond} \cite{madni2016exploiting}
% 2. infographic - 滞后性 icon（添加非可视化图表的元素）
% 3. data video icon 背景透明度 
% 4. 定义中区分说明dashboard，Infographic (infographic poster) [放到了Taxonomy的51行]
% 5. 把2.3.1章节放到2.1中,注意逻辑关系
% 6.整理Immersive, Physicalization

directed - undirected

疑问：
% 1.Compilations\cite{roth2021cartographic}这种形式是否属于annotated chart 放到scrollytelling
% 2.有些只提到了概念，并没有产出实际的工具，这一类型应该怎么放？\cite{dabbebi2017towards} \cite{santos2017data} \cite{kandogan2012just}


%1. 去掉Understanding Infographics through Textual and Visual Tag Prediction
% 2. 增加Finding Their Data Voice: Practices and Challenges of Dashboard Users


7. 叙事性结构、交互方式
叙事结构:
linear: A story sequence path in linear order is prescribed by the author.

user-directed/interactive:The user selects a path among multiple alternatives or creates their own path. 用户在多个可选路径中选择一个路径或创建自己的路径。

parallel: several paths can be traversed or visualized at the same time.

random：There is no prescribed path. There is currently no literature prescribing random order. Therefore we replace this with a column called “overview”.（没有指定的路径。目前尚无随机顺序处方的文献。因此，我们将其替换为一个名为“概述”的列。）

overview:

random和overview是一个意思
Ordering refers to the ways of arranging the path viewers take through the visualization. Sometimes this path is prescribed by the author (linear), sometimes there is no path suggested at all (random access), and other times the user must select a path among multiple alternatives (user-directed).




交互方式：Hover Highlighting / Details 
Filtering / Selection / Search 
Navigation Buttons 
Very Limited Interactivity 
Explicit Instruction 
Tacit Tutorial：隐性教程通过对演示文稿中的交互组件进行动画化来介绍可视化的交互功能，以明确如何操作显示。
Stimulating Default Views：刺激默认视图提供数据和分析的初始呈现，旨在激发用户的兴趣，类似于新闻线索。

8. 仿照\cite{segel2010narrative}的fig7制作工具图（后续工作）
annotated chart中研究较多的是Memorable。

关于交互中注释这个内容理解：1.一种是在创作过程中弹出用于帮助进行解释的对话框，另一种是创建annotated chart这种注释。



Select: mark something as interesting 
Explore: show me something else 
Reconfigure: show me a different arrangement 
Encode: show me a different representation
Abstract/Elaborate: show me more or less detail 
Filter: show me something conditionally 
Connect: show me related items

parallel是指：故事结构+画面布局（也是会影响叙事结构的）

去掉Explicit Instruction 、Tacit Tutorial、Stimulating Default Views三种交互方式

新增2.4.3去阐述工具的那个表

InfoMotion和 属于ai-generator

20220428会议内容：
% 1.重新梳理2.4.1的内容（叙事性可视化-叙事性可视化工具的结构-工具的表-传统可视化-传统可视化的难易程度(简要描述，并不是重点)-二维坐标轴-为什么要绘制二维坐标轴）

% 2. 绘制工具的图表并放到论文中

% 3.论文中所提到的关于叙事性越弱的工具交互效果越强的这部分描述放到discussion部分

% 4.矫正论文中出现的所有文献格式



先说工具分类在说叙事性可视化的分类




% 1. Input datasets support diversity and need to keep the measurement of diversity in type, format, and data content.

% 2. The degree of automation of the process, which requires qualitative or quantitative measurements to explain the degree of intelligence of the technology in the process of inputting the data set to the output visualization.

% 3. The quality of the output visualization, the correct expression of information when automatically generated essential visualization conditions, and pay attention to the comprehensiveness, aesthetics, and creative support.

% 4. The learnability of the model, the automatically generated visualization model, needs to minimize the learning input of the user.

%1.Which major activities are involved in the visualization design and visual narrative process?  在视觉化设计和视觉叙述过程中主要涉及哪些活动?
%1.traditional visualization design (visualization attributes and properties %What Makes a Visualization Memorable?) + narrative visualization design (narrative style - 2010)

% Segel \& Heer\cite{segel2010narrative} propose seven classifications of narrative visualization, magazine-style, annotated charts, partitioned poster, flow charts, comic strips, slide show, film/video/animation. Roth\cite{roth2021cartographic} classified visual storytelling genres into seven Static visual stories, long-form infographics, dynamic slideshows, narration animation, multimedia visual experiences, personalized story maps, and compilations. 

% Table 1. Summary of our visualization taxonomy, including visualization properties and attributes, for the memorability experiment. 
 
%2.To what extend can automation help facilitate these activities?
 %自动化在视觉设计过程中所涉及的范围

% 3.What are the communication requirements of those visual narratives? Which is the final output narrative form of these tools? readability, learnability, memorability, engagement 



%基础概念不需要解释
%The term "information visualization" was first introduced in 1989 by Stuart K. Card, Jock D. Mackinlay, and George G. Robertson in their article "Cognitive Coprocessor for Interactive User Interface"\cite{defanti1989visualization}. 
%一句话描述visualization，接着说visualization的分类，需要补充解释和加reference的地方标了[TODO]，每个我们做的分类choice需要说明原因或依据。
% Information visualization attempts to enhance human cognitive activity by using human visual abilities to understand the meaning of abstract information~\cite{keller2005visualizing}. %In this way, humans with fixed perceptual abilities can control an increasing amount of data. The graphical form of information visualization first appeared in the 18th century. Playfair, a historian and political scientist, and Lambert, a mathematician, first created visualization charts. They believed that converting complex data into charts could help people understand the data. French scientists Minard and Marey in the 19th century first charted by non-manual methods\cite{simkin1987information}.
% Borkin et al.\cite{borkin2013makes} classifies visualizations into 12 types (Area, Bar, Circle, Diagram, Distribution, Grid \& Matrix, Line, Map, Point, Table, Text, Tree \& Networks) based on [TODO]. 
% In this section, we reorganize the 12 types and simplify them into 6 categories according to the form of the visualization output. %This section reclassifies the 12 visualization types according to their output forms. 重复
% Six common visualization types used in statistics, area, bar, circle, line, point, and distribution charts, are classified in Statistical Chart, and two related visualization types, Table and Text, are grouped into one category. %其他还有几个没补充 %area, bar, circle, line, point, distribution, and table as a statistical chart. Since most researchers place grid and network together for study, and both visualization types belong to graph visualization, we refer to grid and network collectively as graph visualization. Finally, we divided the chart into five parts: statistical chart, text, map, graph, and trees.
% Therefore, we classify visualization charts into five general types, namely, Statistical Chart, Text, Map, Graph, and Tree in this paper.

% 总共收集到文献与工具408篇，本研究中使用了201篇与叙事性可视化相关的文献与工具。其中商业类工具共15款


% Tableau
% Datapine
% Sisense
% Thoughtspot
% Qliksense
% Visme
% Infogram
% Canva
% Tiki-toki
% Dipity. 
% Timelinejs.
% Timelinesetter. 

% 下面3个工具需要放reference吗？
% Powerpoint.
% Keynote
% Prezi.


% 编程工具：ggplot2、(有具体文献)
% D3、(有具体文献)
% swoopydrag.js、


% 下午开完会后修改内容:
% 1.梳理122个文献之后不重要的文献
% 2.删除同样意思不同句子表达的句子
% 3.一句话后面使用到多个reference的，要删除相对不重要的
% 4.introduction、method、discussion三部分再次梳理

目前审查委员提到的意见几乎都已经改了。关于每一章的summary，结合了工具的用户以及4种工具的重点重新进行了梳理。


遇到的问题：
1. 如何说明研究中为什么不研究personalizaed story maps这一类型。
2.McKenna(2017)在研究中提到了document这一个类型，但是看图解和scrollytelling是一样的，这个表述在论文中如何说，可以直接说他研究的是scrollytelling吗？
3. 3位作者的叙事性可视化的chart，没办法做到一一对应。
4. 专业用户：experts 
   中间用户：intermediate users
   非专业用户：amateurs
   %non-experts users / non-experts / general users / ordinary users / laymen / 
   
   In HCI and ML literature, people who build ML models fall into three categories: experts, intermediate users of ML, and amateurs \cite{Grounding Interactive Machine Learning Tool Design in How Non-Experts Actually Build Models}\cite{Making Machine-Learning Applications for Time-Series Sensor Data Graphical and Interactive}
   
基于规则（rule-base） - 机器学习(Machine learning) - 强化学习(reinforcement learning)

% 20220919 
1. ML/AI-Supported tool? ML/AI-Supported Tool? ML/AI-supported tool?
ML/AI-supported tool
ML/AI-generator tool

2. 关于3种用户群体只放到了cover letter中，还没放到论文中， 不太清楚这部分应该放在哪块更合适一些

3.canva属于ai-generator tools 吗?

在论文中加入网站+网址

在2.4章节前不要提expert和amateurs，直接写users

%20220926
1. 论文中出现的工具是software好还是tool
2. 回复审查委员的时候，出现的一些参考文献如何写
   
之前提交的论文中文献158篇，table中有122篇文献。去掉了Dashboard中的21篇文献，新增了3篇annotated chart文献，1篇data comics的文献，在Discussion中添加了13篇。 因此这次提交的论文中共有154篇文献。table的总文献为105篇。


#20221129: 

Shin, M., Kim, J., Han, Y., Xie, L., Whitelaw, M., Kwon, B. C., ... & Elmqvist, N. (2022). Roslingifier: Semi-Automated Storytelling for Animated Scatterplots. IEEE Transactions on Visualization and Computer Graphics.


Yeuk- Yin Chan and Huamin Qu. Finavistory: Using narra-tive visualization to explain social and economic relation-ships in financial news. In 2016 International Conferenceon Big Data and Smart Computing (BigComp), pages32-39, 2016.

Katie Watson, Samuel S Sohn, Sasha Schriber, Markus Gross, Carlos Manuel Muniz, and Mubbasir Kapadia. Storyprint: an interactive visualization of stories. In Proceedings of the 24th International Conference on Intelligent User Interfaces, pages 303–311, 2019.

Laura South, Michail Schwab, Nick Beauchamp, Lu Wang, John Wihbey, and Michelle A Borkin. Debatevis: Visualizing political debates for non-expert users. In 2020 IEEE Visualization Conference (VIS), pages 241–245. IEEE, 2020.

Jo Wood, Alexander Kachkaev, and Jason Dykes. Design exposition with literate visualization. IEEE transactions on visualization and computer graphics, 25(1):759–768, 2018.

Wei Chen, Tianyi Lao, Jing Xia, Xinxin Huang, Biao Zhu, Wanqi Hu, and Huihua Guan. Gameflow: narrative visualization of nba basketball games. IEEE Transactions on Multimedia, 18:2247–2256, 2016.

Ronald Metoyer, Qiyu Zhi, Bart Janczuk, and Walter Scheirer. Coupling story to visualization: Using textual analysis as a bridge between data and interpretation. In 23rd International Conference on Intelligent User Interfaces, pages 503–507, 2018.

Qiyu Zhi, Suwen Lin, Poorna Talkad Sukumar, and Ronald Metoyer. Gameviews: Understanding and supporting data-driven sports storytelling. In Proceedings of the 2019 CHI Conference on Human Factors in Computing Systems, pages 1–13, 2019.

% 20230315
% Data comics: Fig.6 design space comics 换图

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> Table/backup/table-0228/table1-0228.tex <==
\renewcommand\arraystretch{1.5}
\biboptions{numbers,sort\&compress}
\begin{table*}


\textbf{\caption{Listed by narrative visualization tool type}}
\begin{tabular}{cm{2.5cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|c|} \hline

\multicolumn{2}{|c|}{} & \textbf{Design Space} & \textbf{Authoring Tools} & \textbf{AI Supported Tools} & \textbf{AI Generator Tools} & \textbf{SUM} \\ \hline


\multicolumn{1}{|c|}{\multirow{11}*{\rotatebox{90}{\textbf{Chart}}}} & 

\textbf{Statistical Chart} %搞定20220227
&\cite{sarikaya2017scatterplots} \cite{luo2019enhancing} \cite{saket2018task} \cite{huron2014constructing} \cite{wun2016comparing} \cite{wang2020cheat} \cite{javed2012exploring} \cite{gramazio2014relation} \cite{lyi2020comparative}\cite{spence2005no}
& \cite{becker2019microsoft} \cite{mackinlay2007show} \cite{mauri2017rawgraphs}\cite{liu2018data} \cite{satyanarayan2014lyra} \cite{zong2020lyra} \cite{mendez2016ivolver} \cite{ren2014ivisdesigner} \cite{bostock2011d3} \cite{satyanarayan2016vega} \cite{li2018echarts} \cite{mei2018viscomposer} 
&\cite{kong2012graphical} \cite{srinivasan2018augmenting} \cite{ren2018charticulator} \cite{zhang2020viscode}\cite{fu2020chartem} \cite{li2020research} \cite{ge2020canis} \cite{ge2021cast} \cite{moritz2018formalizing} \cite{hopkins2020visualint} \cite{chen2021vizlinter} \cite{lin2020dziban} \cite{chen2021augmenting}
&\cite{wongsuphasawat2015voyager} \cite{vartak2015seedb} \cite{wongsuphasawat2016towards}
\cite{heer2007voyagers} \cite{zhao2020chartseer} \cite{luo2018deepeye} \cite{dibia2019data2vis} \cite{zhou2020table2analysis} \cite{zhou2021table2charts} \cite{hu2019vizml} 
& 45 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Text}   %待调整-design space内容太多
& \cite{chi2015morphable}\cite{felix2017taking}\cite{hearst2019evaluation}\cite{wu2011semantic}\cite{paulovich2012semantic}\cite{gansner2013interactive}\cite{cui2010context}\cite{lee2010sparkclouds}\cite{collins2009parallel}\cite{murakami2018depth}\cite{kim2011wordbridge}\cite{bateman2008seeing}\cite{rivadeneira2007getting}\cite{halvey2007assessment}\cite{schrammel2009visual}\cite{shaw2005utilizing}\cite{dubinko2007visualizing}\cite{bielenberg2005groups}\cite{seifert2008beauty}\cite{kaser2007tag}
%这3个出自概念 \cite{burch2013prefix}\cite{steele2010beautiful}\cite{kuo2007tag}
&\cite{viegas2009participatory}\cite{koh2010maniwordle}\cite{strobelt2012rolled}\cite{jo2015wordleplus}\cite{oesper2011wordcloud}\cite{waldner2013facetclouds} \cite{heimerl2014word}
& \cite{xu2016semantic}\cite{lohmann2015concentri}\cite{shu2021dancingwords}\cite{wang2017edwordle}
&\cite{jin2017development}\cite{cheng2014synonym}\cite{wang2019shapewordle}
&34 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Map}  %搞定20220227             
&\cite{roth2021cartographic}\cite{denil2016storied} \cite{biriukov2021storytelling} \cite{marta2015story} \cite{dent2008thematic} \cite{harrower2001visualizing}\cite{harrower2003tips} \cite{battersby2010considerations}
% \cite{haklay2008web}\cite{sui2011convergence}\cite{sieber2016doing} (概念中出现的3篇文献，没有阐明design space)
& \cite{arcgis2012} \cite{mapme2015} \cite{scribblemaps2020} \cite{mapcreator2007} 
&  
&\cite{gao2014newsviews}  
& 13 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Graph}  %搞定20220227
& \cite{abuthawabeh2013finding} \cite{okoe2018node} \cite{ghoniem2004comparison} \cite{rufiange2014animatrix}  \cite{romat2018animated} \cite{dunne2013motif} \cite{duncan2010lombardi}
&\cite{smith2009analyzing}  \cite{ellson2004graphviz} \cite{bastian2009gephi} \cite{auber2004tulip} \cite{dohleman2006exploratory} \cite{rufiange2013diffani} \cite{romat2019expressive} \cite{linhares2017dynetvis} \cite{hagberg2008exploring} \cite{Peixoto2014graphtool} \cite{aslak2019netwulf} \cite{henry2007matlink} \cite{henry2007nodetrix} \cite{rufiange2012treematrix} \cite{angori2019chordlink} \cite{khomtchouk2014heatmapgenerator} \cite{fernandez2017clustergrammer} \cite{gove2011netvisia}
& \cite{abello2006ask}\cite{liu2017egocomp}\cite{wang2019deepdrawing} 
& 
&28  \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Trees} %搞定20220227(删掉了间接引用的文献)
&\cite{schulz2011treevis} \cite{kong2010perceptual} \cite{schulz2007interactive} \cite{schulz2010design} \cite{schulz2013generative} \cite{kopp2018temporal}  \cite{baudel2012capturing} \cite{balzer2005voronoi} \cite{wattenberg2005note} \cite{scheibel2020taxonomy} \cite{scheibel2020survey} \cite{soares2018visualizing}
& \cite{blanch2015dendrogramix}\cite{eaton2020toytree} 
& 
& 
&14  \\ \hline


\multicolumn{1}{|c|}{\multirow{7}*{\rotatebox{90}{\textcolor{black}{\textbf{Infographics}}}}}   %搞定20220226
& \textcolor{black}{\textbf{Infographic}} 
&\cite{albers2014infographics}\cite{artacho2008influence}  \cite{santos2018influence} \cite{dunlap2016getting}
\cite{harrison2015infographic} \cite{lyra2016infographics} \cite{lan2021smile} \cite{otten2015infographics} \cite{diakopoulos2011playable} \cite{naparin2017infographics} \cite{albers2015infographics} \cite{jones2015information} \cite{cmeciu2016beyond} \cite{risch2008role} \cite{moere2011role} \cite{smiciklas2012power} \cite{kosara2016presentation}      
%\cite{martix2014teaching} \cite{noh2015use}\cite{haroz2015isotype}  \cite{oliveira2020visual}\cite{amit2018digital} \cite{balkac2018role}（领域中的应用）
& \cite{lee2013sketchstory} \cite{kim2016data} \cite{madan2018synthetically}\cite{xia2018dataink}  \cite{wang2018infonice} \cite{zhang2020dataquilt} \cite{coelho2020infomages} \cite{cui2021mixed}  \cite{kim2019dataselfie}
&\cite{infogram2012} \cite{visme2013} \cite{lu2020exploring} \cite{tyagi2021user} \cite{yuan2021infocolorizer} 
& \cite{CANVA2018}\cite{cui2019text}\cite{qian2020retrieve}
& 34 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& {\textbf{Timeline \& Storyline}} %搞定20220226       
& \cite{aigner2011visualization} \cite{havre2002themeriver}  \cite{byron2008stacked} \cite{tanahashi2012design}  \cite{gronemann2016crossing} \cite{tanahashi2015efficient} \cite{di2020storyline} \cite{lan2021understanding}  \cite{bach2015time}
& \cite{Preceden2010}  \cite{dukes2010dipity} \cite{webalon2011tiki} \cite{llc2012timeglider} \cite{TimelineJS2013} \cite{TimelineSetter2011} \cite{brehmer2019timeline} \cite{kim2017visualizing} \cite{qiang2016storycake} \cite{agarwal2020set}  \cite{brehmer2016timelines}
& \cite{nguyen2016timesets} \cite{tang2018istoryline} \cite{tang2020plotthread} \cite{liu2013storyflow}  \cite{fulda2015timelinecurator} \cite{chen2019towards}\cite{satyanarayan2014authoring} 
& 
&27 \\ \cline{2-7} 
 
\multicolumn{1}{|c|}{}& {\textbf{Annotated Chart}} %搞定20220226
& \cite{borkin2013makes} \cite{borkin2015beyond} \cite{brath2018automated} \cite{kandogan2012just} \cite{kong2017internal} 
& \cite{gomez2017ggplot2} \cite{swoopyDragjs2016} \cite{wongsuphasawatlabella2015} \cite{ren2017chartaccent} 
& \cite{hullman2013contextifier} \cite{latif2021kori} 
 \cite{bryan2016temporal} \cite{bylinskii2017understanding} \cite{chen2010click2annotate} \cite{chen2010touch2annotate} %后面这两个属于authoring tools还是ai-supported tools
& \cite{park2018graphoto} \cite{liu2020autocaption}
&17 \\ \cline{2-7}  

\multicolumn{1}{|c|}{}& {\textbf{Glyph}}  %搞定20220226 - 两篇有疑问
&\cite{borgo2013glyph} \cite{yost2005single} \cite{klippel2009colour}  
\cite{fuchs2014influence} \cite{fuchs2016systematic} \cite{roberts2005haptic} \cite{ward2008multivariate}
%\cite{ropinski2011survey}[医学领域] \cite{maguire2012taxonomy}[生物学领域]
& \cite{brehmer2021generative} \cite{tsandilas2020structgraphics} \cite{tong2016glyphlens}  \cite{ribarsky1994glyphmaker}
&\cite{zhao2020iconate}  
&\cite{ying2021glyphcreator} 
&13  \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Comics}} %搞定20220225
&\cite{wang2020data}\cite{bach2018design} \cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding} \cite{zhao2015data} \cite{bach2017emerging}
& \cite{wang2021interactive}  \cite{kang2021toonnote} \cite{kim2019datatoon}
& \cite{zhao2021chartstory}
& \cite{wang2019datashot}  \cite{shi2020calliope}
&13 \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Videos}} %搞定20220225
& \cite{amini2015understanding}  \cite{cao2020examining} \cite{thompson2020understanding}  \cite{shi2021communicating} \cite{tang2020design} \cite{wang2016animated} \cite{li2020improving} \cite{lan2021kineticharts}  \cite{shu2020makes} 
& \cite{amini2016authoring}  \cite{chen2021augmenting}
&\cite{thompson2021data} \cite{wang2021animated} 
& \cite{shi2021autoclips} 
&14 \\ \hline

\multicolumn{2}{|c|}{\textbf{Dashboard}} %搞定20220225
& \cite{laubheimer2017dashboards} \cite{vazquez2019extending} \cite{vazquez2019information}\cite{sarikaya2018we} \cite{froese2016lessons}\cite{chen2020composition}\cite{qu2017keeping}
%\cite{schwendimann2016perceiving}\cite{sedrakyan2019guiding}\cite{molenaar2018teachers}\cite{cha2019applying}\cite{elias2012annotating}\cite{bajzek2007inventing}\cite{few2007dashboard}前面这些是学习仪表盘的内容，因为是特殊领域的所以没有放到正文中。 %\cite{park2015development}\cite{brouns2015d2}\cite{ji2014ddart}\cite{faiola2015supporting}\cite{wilbanks2014review}\cite{gray2016collecting}\cite{mattern2015mission} 这些是概念+在某一个领域中的应用。
&  \cite{tableau2006} \cite{ahlberg1996spotfire} \cite{cutroni2007google} \cite{filonik2013customisable} \cite{elias2011exploration}
& \cite{belo2014restructuring} \cite{dabbebi2017towards} \cite{santos2017data} \cite{elshehaly2020qualdash} \cite{ma2020ladv}
&   \cite{datapine2012}\cite{thoughtspot2012}\cite{QlikSense2010}\cite{SisenseFusionAnalytics2019}
&21 \\ \hline

\multicolumn{2}{|c|}{\textbf{Scrollytelling}}  %搞定20220225
&\cite{seyser2018scrollytelling}\cite{roth2021cartographic}
\cite{elias2018towards}\cite{hullman2013deeper}
&\cite{bocklandt2021sandslide}\cite{conlen2018idyll}\cite{sultanum2021leveraging} %\cite{powerpoint2016}\cite{keynote2003}\cite{googleslide2006} \cite{prezi2007}
&\cite{winters2019automatically}
&\cite{lu2021automatic} 
&9 \\ \hline

\multicolumn{2}{|c|}{\textbf{Immersive Narrative}}  %搞定20220225
&\cite{kraus2021value} \cite{isenberg2018immersive}\cite{vierjahn2017towards} \cite{liu2020design}\cite{bach2017hologram}  \cite{bach2017drawing} \cite{raja2004exploring}
&\cite{cordeil2016immersive}  \cite{butscher2018clusters} \cite{sicat2018dxr} 
\cite{chen2019marvist}  \cite{filonik2016glance} \cite{donalek2014immersive}
&
& 
&13  \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} &129 & 89 & 48 & 28 & 295 \\ \hline


\end{tabular}
\end{table*}

==> Table/backup/table-0228/table2-0228-edit.tex <==
\begin{table*}[]
\begin{tabular}{c|m{2cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|}
\hline

\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{}  \\ \hline


%---------------------Charts-------------------
\multicolumn{1}{|c|}{\multirow{6}{*}{\rotatebox{90}{\textbf{Chart}}}}

%---------------------Statistical Chart  %20220227-搞定-------------------
& \textbf{Statistical Chart}
&% \cite{spence2005no}\cite{mackinlay2007show}\cite{heer2007voyagers}
&%
&%\cite{bostock2011d3}
&%\cite{javed2012exploring}\cite{kong2012graphical}
&%
&%\cite{huron2014constructing} \cite{gramazio2014relation}\cite{satyanarayan2014lyra}\cite{ren2014ivisdesigner}
&%\cite{wongsuphasawat2015voyager} \cite{vartak2015seedb}
&%\cite{wun2016comparing} \cite{mendez2016ivolver}\cite{satyanarayan2016vega}\cite{wongsuphasawat2016towards}
&%\cite{sarikaya2017scatterplots}\cite{mauri2017rawgraphs}
&%\cite{saket2018task}\cite{liu2018data}\cite{li2018echarts}\cite{mei2018viscomposer} \cite{srinivasan2018augmenting}\cite{ren2018charticulator}\cite{moritz2018formalizing} \cite{luo2018deepeye}
&%\cite{luo2019enhancing}\cite{becker2019microsoft}\cite{dibia2019data2vis}\cite{hu2019vizml}
&%\cite{wang2020cheat}\cite{lyi2020comparative}\cite{zong2020lyra}\cite{zhang2020viscode}\cite{fu2020chartem} \cite{li2020research} \cite{ge2020canis}\cite{hopkins2020visualint} \cite{lin2020dziban}\cite{zhao2020chartseer}\cite{zhou2020table2analysis}
&%\cite{ge2021cast}\cite{chen2021vizlinter}\cite{chen2021augmenting} \cite{zhou2021table2charts}
&%45
\\\cline{2-16} 

%---------------------Text  %20220227-搞定-------------------
\multicolumn{1}{|c|}{} & \textbf{Text}
&% \cite{collins2009parallel}\cite{fujimura2008topigraphy}\cite{bateman2008seeing}\cite{rivadeneira2007getting}\cite{halvey2007assessment}\cite{schrammel2009visual}\cite{shaw2005utilizing}\cite{dubinko2007visualizing}\cite{bielenberg2005groups}\cite{seifert2008beauty}\cite{kaser2007tag}\cite{viegas2009participatory}
&%\cite{cui2010context}\cite{lee2010sparkclouds}\cite{koh2010maniwordle}
&%\cite{wu2011semantic}\cite{kim2011wordbridge}\cite{oesper2011wordcloud}
&%\cite{paulovich2012semantic}\cite{strobelt2012rolled}
&%\cite{gansner2013interactive}\cite{waldner2013facetclouds}
&%\cite{heimerl2014word}\cite{cheng2014synonym}
&%\cite{chi2015morphable}\cite{jo2015wordleplus}\cite{lohmann2015concentri}
&%\cite{xu2016semantic}
&%\cite{felix2017taking}\cite{wang2017edwordle}\cite{jin2017development}
&%\cite{murakami2018depth}
&%\cite{hearst2019evaluation}\cite{wang2019shapewordle}
&%
&% \cite{shu2021dancingwords}
&%35
\\ \cline{2-16} 

%---------------------Map  %20220227-搞定-------------------
\multicolumn{1}{|c|}{} & \textbf{Map} 
&%% \cite{dent2008thematic} \cite{harrower2001visualizing}\cite{harrower2003tips}\cite{mapcreator2007}
&% \cite{battersby2010considerations}
&%
&%\cite{arcgis2012}
&%
&%\cite{gao2014newsviews}
&%\cite{marta2015story}\cite{mapme2015}
&%\cite{denil2016storied}
&%
&%
&%
&%\cite{scribblemaps2020}
&%\cite{roth2021cartographic}\cite{biriukov2021storytelling}
&%13
\\ \cline{2-16} 

%---------------------Graph %20220227-搞定-------------------
\multicolumn{1}{|c|}{} &\textbf{Graph}
&% \cite{ghoniem2004comparison}\cite{smith2009analyzing}\cite{ellson2004graphviz} \cite{bastian2009gephi} \cite{auber2004tulip} \cite{dohleman2006exploratory}  \cite{hagberg2008exploring} \cite{henry2007matlink} \cite{henry2007nodetrix}\cite{abello2006ask}
&%\cite{duncan2010lombardi}
&% \cite{gove2011netvisia}
&%\cite{rufiange2012treematrix}
&%\cite{abuthawabeh2013finding}\cite{dunne2013motif}\cite{rufiange2013diffani}
&%\cite{rufiange2014animatrix}\cite{Peixoto2014graphtool}\cite{khomtchouk2014heatmapgenerator}
&%
&%
&% \cite{linhares2017dynetvis}\cite{fernandez2017clustergrammer}\cite{liu2017egocomp}
&%\cite{okoe2018node}\cite{romat2018animated}
&%\cite{romat2019expressive}\cite{aslak2019netwulf}\cite{angori2019chordlink}\cite{wang2019deepdrawing} 
&%
&%
&%28
\\ \cline{2-16} 


%---------------------Trees %20220227-搞定 -------------------
\multicolumn{1}{|c|}{} & \textbf{Trees}
&% \cite{schulz2007interactive}\cite{balzer2005voronoi} \cite{wattenberg2005note}
&%\cite{kong2010perceptual}\cite{schulz2010design}
&%\cite{schulz2011treevis}
&%\cite{baudel2012capturing}
&%\cite{schulz2013generative}
&%
&%\cite{blanch2015dendrogramix}
&%
&%
&%\cite{kopp2018temporal}\cite{soares2018visualizing}
&%
&%\cite{scheibel2020taxonomy}\cite{scheibel2020survey}\cite{eaton2020toytree}
&%
&%14
\\ \hline

%---------------------Infographics %20220227-搞定-------------------
\multicolumn{1}{|c|}{\multirow{6}{*}{\rotatebox{90}{\textbf{Infographics}}}}& \textbf{Infographic} 
&% \cite{artacho2008influence}\cite{risch2008role}
&%
&%\cite{diakopoulos2011playable}\cite{moere2011role}
&%\cite{smiciklas2012power}\cite{infogram2012}
&%\cite{lee2013sketchstory}\cite{visme2013}
&%\cite{albers2014infographics}
&%\cite{harrison2015infographic}\cite{otten2015infographics}\cite{albers2015infographics}\cite{jones2015information}
&%\cite{dunlap2016getting}\cite{lyra2016infographics}\cite{cmeciu2016beyond}\cite{kosara2016presentation}\cite{kim2016data}
&%\cite{hearst2017teaching}\cite{naparin2017infographics}
&%\cite{santos2018influence}\cite{madan2018synthetically}\cite{xia2018dataink}  \cite{wang2018infonice} \cite{CANVA2018}
&%\cite{cui2019text}\cite{kim2019dataselfie}
&%\cite{zhang2020dataquilt} \cite{coelho2020infomages}\cite{lu2020exploring}\cite{qian2020retrieve}
&% \cite{lan2021smile}\cite{cui2021mixed}\cite{tyagi2021user} \cite{yuan2021infocolorizer} 
&%35
\\ \cline{2-16} 

%---------------------Timelines  %20220227-搞定-------------------
\multicolumn{1}{|c|}{} & \textbf{Timeline} 
&% \cite{havre2002themeriver}  \cite{byron2008stacked}
&%\cite{Preceden2010}  \cite{dukes2010dipity}
&%\cite{aigner2011visualization}\cite{webalon2011tiki}\cite{TimelineSetter2011}
&%\cite{tanahashi2012design}\cite{llc2012timeglider}
&%\cite{TimelineJS2013}\cite{liu2013storyflow}
&%\cite{satyanarayan2014authoring}
&%\cite{tanahashi2015efficient}\cite{bach2015time}\cite{fulda2015timelinecurator}
&%\cite{gronemann2016crossing}\cite{qiang2016storycake}\cite{brehmer2016timelines}\cite{nguyen2016timesets}
&%\cite{kim2017visualizing}
&%\cite{tang2018istoryline}
&%\cite{brehmer2019timeline}\cite{chen2019towards}
&%\cite{di2020storyline}\cite{agarwal2020set} \cite{tang2020plotthread}
&%\cite{lan2021understanding}
&%27
 \\ \cline{2-16} 

%---------------------Annotated Chart  %20220227-搞定-------------------
\multicolumn{1}{|c|}{} & \textbf{Annotated Chart} 
&% 
&%\cite{chen2010click2annotate}\cite{chen2010touch2annotate}
&%
&%\cite{kandogan2012just}
&%\cite{borkin2013makes}\cite{hullman2013contextifier}
&%
&%\cite{borkin2015beyond}\cite{wongsuphasawatlabella2015}
&%\cite{swoopyDragjs2016} \cite{bryan2016temporal}
&%\cite{kong2017internal}\cite{gomez2017ggplot2}\cite{ren2017chartaccent}\cite{bylinskii2017understanding}
&%\cite{brath2018automated}\cite{park2018graphoto}
&%
&%\cite{liu2020autocaption}
&%\cite{latif2021kori}
&%17
\\ \cline{2-16} 

%---------------------Glyph %20220227-搞定-------------------
\multicolumn{1}{|c|}{} & \textbf{Glyph} 
&% \cite{yost2005single}\cite{klippel2009colour}\cite{roberts2005haptic}\cite{ward2008multivariate}\cite{ribarsky1994glyphmaker}
&%
&%
&%
&%\cite{borgo2013glyph}
&%\cite{fuchs2014influence}
&%
&%\cite{fuchs2016systematic}\cite{tong2016glyphlens}
&%
&%
&%
&%\cite{tsandilas2020structgraphics}\cite{zhao2020iconate}
&%\cite{brehmer2021generative}\cite{ying2021glyphcreator} 
&%13
\\ \hline

%----------------Data Comics %20220227-搞定------------------
\multicolumn{2}{|c|}{\textbf{Data Comics}} 
& 
&
&
&
&
&
&\cite{zhao2015data}
&
&\cite{bach2017emerging}
&\cite{bach2018design}
&\cite{wang2019teaching}\cite{wang2019comparing}\cite{wang2019datashot} \cite{zhao2019understanding}\cite{kim2019datatoon}
&\cite{wang2020data}\cite{shi2020calliope}
&\cite{wang2021interactive}  \cite{kang2021toonnote}\cite{zhao2021chartstory}
& 13        \\ \hline


%----------------Data Videos %20220227-搞定------------------
\multicolumn{2}{|c|}{\textbf{Data Videos}} 
& 
&
&
&
&
&
&\cite{amini2015understanding}
&\cite{wang2016animated}\cite{amini2016authoring}
&
&
&
&\cite{cao2020examining}\cite{thompson2020understanding}\cite{tang2020design}\cite{li2020improving}\cite{shu2020makes} 
&\cite{shi2021communicating}\cite{lan2021kineticharts}\cite{chen2021augmenting}\cite{thompson2021data} \cite{wang2021animated} \cite{shi2021autoclips}
& 14
\\ \hline

%----------------Dashboard %20220227-搞定------------------
\multicolumn{2}{|c|}{\textbf{Dashboard}} 
&\cite{tableau2003}\cite{ahlberg1996spotfire} \cite{cutroni2007google}
&\cite{QlikSense2010}
&\cite{elias2011exploration}
&\cite{choosel2012} \cite{datapine2012}\cite{thoughtspot2012}
&\cite{filonik2013customisable}
&\cite{belo2014restructuring}
&
&\cite{froese2016lessons}
&\cite{laubheimer2017dashboards}\cite{qu2017keeping}\cite{dabbebi2017towards}\cite{santos2017data}
&\cite{sarikaya2018we}
&\cite{vazquez2019extending}\cite{vazquez2019information}\cite{SisenseFusionAnalytics2019}
&\cite{chen2020composition}\cite{elshehaly2020qualdash} \cite{ma2020ladv}
&
&22
\\ \hline

%-------------Scrollytelling %20220227-搞定-----------------
\multicolumn{2}{|c|}{\textbf{Scrollytelling}}
& 
&
&
&
&\cite{hullman2013deeper}
&
&
&
&
&\cite{seyser2018scrollytelling}\cite{elias2018towards}\cite{conlen2018idyll}
&\cite{winters2019automatically}
&
&\cite{roth2021cartographic}\cite{bocklandt2021sandslide}\cite{sultanum2021leveraging}\cite{lu2021automatic}
&9\\ \hline

%-------------Immersive%20220227-搞定-----------------
\multicolumn{2}{|c|}{\textbf{Immersive}} 
&\cite{raja2004exploring}
&
&
&
&
&\cite{donalek2014immersive}
&
&\cite{cordeil2016immersive}\cite{filonik2016glance}
&\cite{vierjahn2017towards}\cite{bach2017hologram}\cite{bach2017drawing}
&\cite{isenberg2018immersive}\cite{butscher2018clusters}\cite{sicat2018dxr}
&\cite{chen2019marvist}
&\cite{liu2020design}
&\cite{kraus2021value}
& \\ \hline

\multicolumn{2}{|c|}{\textbf{}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

\end{tabular}
\end{table*}


==> Table/backup/table-0228/table2-0228.tex <==
\renewcommand\arraystretch{1.5}
\begin{table*}
\textbf{ \caption{Listed by year of narrative visualization publication}}
\begin{tabular}{c|m{2cm}<{\centering}|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline

\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM}  \\ \hline


%---------------------Charts-------------------
\multicolumn{1}{|c|}{\multirow{5}{*}{\rotatebox{90}{\textbf{Chart}}}}

& \textbf{Statistical Chart} & 3 &  & 1 & 2 &  & 4 & 2 & 4 & 2 & 8 & 4 & 11 & 4 & 45  \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Text} & 11 & 3 & 3 & 2 & 2 & 2 & 3 & 1 & 3 & 1 & 2 &  & 1 & 34 \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Map} & 4 & 1 &  & 1 &  & 1 & 2 & 1 &  &  &  & 1 & 2 & 13 \\\cline{2-16} 

\multicolumn{1}{|c|}{} &\textbf{Graph} & 10 & 1 & 1 & 1 & 3 & 3 &  &  & 3 & 2 & 4 &  &  & 28  \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Trees}  & 3 & 2 & 1 & 1 & 1 &  & 1 &  &  & 2 &  & 3 &  & 14 \\ \hline

%---------------------infographic-------------------
\multicolumn{1}{|c|}{\multirow{5}{*}{\rotatebox{90}{\textbf{Infographics}}}}& \textbf{Infographic} 
& 2 &  & 2 & 2 & 2 & 1 & 4 & 5 & 1 & 5 & 2 & 4 & 4 & 34  \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Timeline} & 2 & 2 & 3 & 2 & 2 & 1 & 3 & 4 & 1 & 1 & 2 & 3 & 1 & 27  \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Annotated Chart}&  & 2 &  & 1 & 2 &  & 2 & 2 & 4 & 2 &  & 1 & 1 & 17  \\\cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Glyph}  & 5 &  &  &  & 1 & 1 &  & 2 &  &  &  & 2 & 2 & 13   \\ \hline


%---------------------Data Comics-------------------
\multicolumn{2}{|c|}{\textbf{Data Comics}} &  &  &  &  &  &  & 1 &  & 1 & 1 & 5 & 2 & 3 & 13  \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Videos}}  &  &  &  &  &  &  & 1 & 2 &  &  &  & 5 & 6 & 14 \\ \hline

\multicolumn{2}{|c|}{\textbf{Dashboard}}  & 3 & 1 & 1 & 2 & 1 & 1 &  & 1 & 4 & 1 & 3 & 3 &  & 21   \\ \hline

\multicolumn{2}{|c|}{\textbf{Scrollytelling}}  &  &  &  &  & 1 &  &  &  &  & 3 & 1 &  & 4 & 9  \\ \hline

\multicolumn{2}{|c|}{\textbf{Immersive Narrative}} & 1 &  &  &  &  & 1 &  & 2 & 3 & 3 & 1 & 1 & 1 & 13  \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}}  & 44 & 12 & 12 & 14 & 15 & 15 & 19 & 24 & 22 & 29 & 24 & 36 & 29 & 295 \\ \hline

\end{tabular}
\end{table*}

==> Table/backup/table1-0315.tex <==
\renewcommand\arraystretch{1.5}
% \biboptions{numbers,sort\&compress}
\begin{table*}


\textbf{\caption{Listed by narrative visualization tool type}}
\begin{tabular}{cm{2.5cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|m{2.9cm}<{\centering}|c|} \hline

\multicolumn{2}{|c|}{} & \textbf{Design Space} & \textbf{Authoring Tools} & \textbf{AI Supported Tools} & \textbf{AI Generator Tools} & \textbf{SUM} \\ \hline


\multicolumn{1}{|c|}{\multirow{5}*{\rotatebox{90}{\textbf{Chart}}}} & 

\textbf{Statistical Chart} %搞定20220227
&\cite{sarikaya2017scatterplots,luo2019enhancing,saket2018task,huron2014constructing,wun2016comparing,wang2020cheat,javed2012exploring,gramazio2014relation,lyi2020comparative,spence2005no}
& \cite{becker2019microsoft,mackinlay2007show,mauri2017rawgraphs,liu2018data,satyanarayan2014lyra,zong2020lyra,mendez2016ivolver,ren2014ivisdesigner,bostock2011d3,satyanarayan2016vega,li2018echarts,mei2018viscomposer} 
&\cite{kong2012graphical,srinivasan2018augmenting,ren2018charticulator,zhang2020viscode,fu2020chartem,li2020research,ge2020canis,ge2021cast,moritz2018formalizing,hopkins2020visualint,chen2021vizlinter,lin2020dziban,chen2021augmenting}
&\cite{wongsuphasawat2015voyager,vartak2015seedb,wongsuphasawat2016towards,heer2007voyagers,zhao2020chartseer,luo2018deepeye,dibia2019data2vis,zhou2020table2analysis,zhou2021table2charts,hu2019vizml} 
& 45 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Text}   %待调整-design space内容太多
& \cite{chi2015morphable,felix2017taking,hearst2019evaluation,wu2011semantic,paulovich2012semantic,gansner2013interactive,cui2010context,lee2010sparkclouds,collins2009parallel,murakami2018depth,kim2011wordbridge,bateman2008seeing,rivadeneira2007getting,halvey2007assessment,schrammel2009visual,shaw2005utilizing,dubinko2007visualizing,bielenberg2005groups,seifert2008beauty,kaser2007tag}
%这3个出自概念 \cite{burch2013prefix}\cite{steele2010beautiful}\cite{kuo2007tag}
&\cite{viegas2009participatory,koh2010maniwordle,strobelt2012rolled,jo2015wordleplus,oesper2011wordcloud,waldner2013facetclouds,heimerl2014word}
& \cite{xu2016semantic,lohmann2015concentri,shu2021dancingwords,wang2017edwordle}
&\cite{jin2017development,cheng2014synonym,wang2019shapewordle}
&34 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Map}  %搞定20220227             
&\cite{roth2021cartographic,denil2016storied,biriukov2021storytelling,marta2015story,dent2008thematic,harrower2001visualizing,harrower2003tips,battersby2010considerations}
% \cite{haklay2008web}\cite{sui2011convergence}\cite{sieber2016doing} (概念中出现的3篇文献，没有阐明design space)
& \cite{arcgis2012,mapme2015,scribblemaps2020,mapcreator2007}
&  
&\cite{gao2014newsviews}  
& 13 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Graph}  %搞定20220227
& \cite{abuthawabeh2013finding,okoe2018node,ghoniem2004comparison,rufiange2014animatrix,romat2018animated,dunne2013motif,duncan2010lombardi} 
&\cite{smith2009analyzing,ellson2004graphviz,bastian2009gephi,auber2004tulip,dohleman2006exploratory,rufiange2013diffani,romat2019expressive,linhares2017dynetvis,hagberg2008exploring,Peixoto2014graphtool,aslak2019netwulf,henry2007matlink,henry2007nodetrix,rufiange2012treematrix,angori2019chordlink,khomtchouk2014heatmapgenerator,fernandez2017clustergrammer,gove2011netvisia}
& \cite{abello2006ask,liu2017egocomp,wang2019deepdrawing}
& 
&28  \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Trees} %搞定20220227(删掉了间接引用的文献)
&\cite{schulz2011treevis,kong2010perceptual,schulz2007interactive,schulz2010design,schulz2013generative,kopp2018temporal,baudel2012capturing,balzer2005voronoi,wattenberg2005note,scheibel2020taxonomy,scheibel2020survey,soares2018visualizing}
& \cite{blanch2015dendrogramix,eaton2020toytree}
& 
& 
&14  \\ \hline


\multicolumn{1}{|c|}{\multirow{5}*{\rotatebox{90}{\textcolor{black}{\textbf{Infographics}}}}}   %搞定20220226
& \textcolor{black}{\textbf{Infographic}} 
&\cite{albers2014infographics,artacho2008influence,santos2018influence,dunlap2016getting,harrison2015infographic,lyra2016infographics,lan2021smile,otten2015infographics,diakopoulos2011playable,naparin2017infographics,albers2015infographics,jones2015information,cmeciu2016beyond,risch2008role,moere2011role,smiciklas2012power,kosara2016presentation}   
%\cite{martix2014teaching} \cite{noh2015use}\cite{haroz2015isotype}  \cite{oliveira2020visual}\cite{amit2018digital} \cite{balkac2018role}（领域中的应用）
& \cite{lee2013sketchstory,kim2016data,madan2018synthetically,xia2018dataink,wang2018infonice,zhang2020dataquilt,coelho2020infomages,cui2021mixed,kim2019dataselfie}
&\cite{infogram2012,visme2013,lu2020exploring,tyagi2021user,yuan2021infocolorizer} 
& \cite{CANVA2018,cui2019text,qian2020retrieve}
& 34 \\ \cline{2-7} 

\multicolumn{1}{|c|}{}& {\textbf{Timeline \& Storyline}} %搞定20220226       
& \cite{aigner2011visualization,havre2002themeriver,byron2008stacked,tanahashi2012design,gronemann2016crossing,tanahashi2015efficient,di2020storyline,lan2021understanding,bach2015time} 
& \cite{Preceden2010,dukes2010dipity,webalon2011tiki,llc2012timeglider,TimelineJS2013,TimelineSetter2011,brehmer2019timeline,kim2017visualizing,qiang2016storycake,agarwal2020set,brehmer2016timelines}
& \cite{nguyen2016timesets,tang2018istoryline,tang2020plotthread,liu2013storyflow,fulda2015timelinecurator,chen2019towards,satyanarayan2014authoring}
& 
&27 \\ \cline{2-7} 
 
\multicolumn{1}{|c|}{}& {\textbf{Annotated Chart}} %搞定20220226
& \cite{borkin2013makes,borkin2015beyond,brath2018automated,kandogan2012just,kong2017internal} 
& \cite{gomez2017ggplot2,swoopyDragjs2016,wongsuphasawatlabella2015,ren2017chartaccent} 
& \cite{hullman2013contextifier,latif2021kori,bryan2016temporal,bylinskii2017understanding,chen2010click2annotate,chen2010touch2annotate} %后面这两个属于authoring tools还是ai-supported tools
& \cite{park2018graphoto,liu2020autocaption} 
&17 \\ \cline{2-7}  

\multicolumn{1}{|c|}{}& {\textbf{Glyph}}  %搞定20220226 - 两篇有疑问
&\cite{borgo2013glyph,yost2005single,klippel2009colour,fuchs2014influence,fuchs2016systematic,roberts2005haptic,ward2008multivariate}
%\cite{ropinski2011survey}[医学领域] \cite{maguire2012taxonomy}[生物学领域]
& \cite{brehmer2021generative,tsandilas2020structgraphics,tong2016glyphlens,ribarsky1994glyphmaker}
&\cite{zhao2020iconate}  
&\cite{ying2021glyphcreator} 
&13  \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Comics}} %搞定20220225
&\cite{wang2020data,bach2018design,wang2019teaching,wang2019comparing,zhao2019understanding,zhao2015data,bach2017emerging}
& \cite{wang2021interactive,kang2021toonnote,kim2019datatoon}
& \cite{zhao2021chartstory}
& \cite{wang2019datashot,shi2020calliope}
&13 \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Videos}} %搞定20220225
& \cite{amini2015understanding,cao2020examining,thompson2020understanding,shi2021communicating,tang2020design,wang2016animated,li2020improving,lan2021kineticharts,shu2020makes} 
& \cite{amini2016authoring,chen2021augmenting} 
&\cite{thompson2021data,wang2021animated}
& \cite{shi2021autoclips} 
&14 \\ \hline

\multicolumn{2}{|c|}{\textbf{Dashboard}} %搞定20220225
& \cite{laubheimer2017dashboards,vazquez2019extending,vazquez2019information,sarikaya2018we,froese2016lessons,chen2020composition,qu2017keeping} 
%\cite{schwendimann2016perceiving}\cite{sedrakyan2019guiding}\cite{molenaar2018teachers}\cite{cha2019applying}\cite{elias2012annotating}\cite{bajzek2007inventing}\cite{few2007dashboard}前面这些是学习仪表盘的内容，因为是特殊领域的所以没有放到正文中。 %\cite{park2015development}\cite{brouns2015d2}\cite{ji2014ddart}\cite{faiola2015supporting}\cite{wilbanks2014review}\cite{gray2016collecting}\cite{mattern2015mission} 这些是概念+在某一个领域中的应用。
&  \cite{tableau2006,ahlberg1996spotfire,cutroni2007google,filonik2013customisable,elias2011exploration} 
& \cite{belo2014restructuring,dabbebi2017towards,santos2017data,elshehaly2020qualdash,ma2020ladv} 
& \cite{datapine2012,thoughtspot2012,QlikSense2010,SisenseFusionAnalytics2019}
&21 \\ \hline

\multicolumn{2}{|c|}{\textbf{Scrollytelling}}  %搞定20220225
&\cite{seyser2018scrollytelling,roth2021cartographic,elias2018towards,hullman2013deeper}
&\cite{bocklandt2021sandslide,conlen2018idyll,sultanum2021leveraging} %\cite{powerpoint2016}\cite{keynote2003}\cite{googleslide2006} \cite{prezi2007}
&\cite{winters2019automatically}
&\cite{lu2021automatic} 
&9 \\ \hline

\multicolumn{2}{|c|}{\textbf{Immersive Narrative}}  %搞定20220225
&\cite{kraus2021value,isenberg2018immersive,vierjahn2017towards,liu2020design,bach2017hologram,bach2017drawing,raja2004exploring} 
&\cite{cordeil2016immersive,butscher2018clusters,sicat2018dxr,chen2019marvist,filonik2016glance,donalek2014immersive}
&
& 
&13  \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} &129 & 89 & 48 & 28 & 295 \\ \hline


\end{tabular}
\end{table*}

==> Table/backup/table1-0327.tex <==
\renewcommand\arraystretch{1.5}
% \biboptions{numbers,sort\&compress}
\begin{table*}

\textbf{\caption{Listed by narrative visualization tool type}}

\begin{tabular}{|c|m{2.8cm}<{\centering}|m{2.8cm}<{\centering}|m{2.8cm}<{\centering}|m{2.8cm}<{\centering}|m{2.5cm}<{\centering}|c|} \hline

\multicolumn{2}{|c|}{}  & \textbf{Design Space} & \textbf{Authoring Tools} & \textbf{AI-Supported Tools} & \textbf{AI-Generator Tools} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Traditional\\visualization\end{tabular}}}}} 
& \textbf{Statistical chart} 
&\cite{saket2018task}  \cite{lyi2020comparative} \cite{luo2019enhancing} \cite{huron2014constructing} \cite{wun2016comparing} \cite{wang2020cheat}
&\cite{mauri2017rawgraphs} \cite{mendez2016ivolver} \cite{zong2020lyra} \cite{chen2021augmenting}  \cite{satyanarayan2014lyra} %\cite{ren2018charticulator} % 后面跟着3个是编程工具 \cite{bostock2011d3} \cite{satyanarayan2016vega} \cite{mei2018viscomposer}
&\cite{hopkins2020visualint} \cite{chen2021vizlinter} \cite{moritz2018formalizing} \cite{lin2020dziban} \cite{zhang2020viscode} \cite{fu2020chartem} \cite{ge2020canis} \cite{ge2021cast} \cite{li2020research}
& \cite{luo2018deepeye} \cite{vartak2015seedb} \cite{wongsuphasawat2016towards} \cite{wongsuphasawat2015voyager} \cite{zhao2020chartseer} \cite{hu2019vizml} \cite{zhou2020table2analysis} \cite{zhou2021table2charts} \cite{dibia2019data2vis}
& 29 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{\begin{tabular}[c]{@{}c@{}}Other Charts\\(Text\&Map\\ \&Graph\&Tree)\end{tabular}} 
&
&
&
&
&  
\\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Dashboard} 
& \cite{sarikaya2018we} \cite{vazquez2019extending} \cite{froese2016lessons} \cite{javed2012exploring} \cite{qu2017keeping} \cite{chen2020composition}
& \cite{tableau2006} \cite{ahlberg1996spotfire} \cite{cutroni2007google} \cite{elias2011exploration} \cite{elias2012annotating}
& \cite{belo2014restructuring} \cite{dabbebi2017towards} \cite{elshehaly2020qualdash} \cite{santos2017data} \cite{ma2020ladv}
& \cite{datapine2012} \cite{SisenseFusionAnalytics2019} \cite{thoughtspot2012} \cite{QlikSense2010}
& 20
\\ \cline{2-7} 

\multicolumn{1}{|c|}{}& \textbf{Glyphs} 
&\cite{borgo2013glyph} \cite{yost2005single} \cite{ward2008multivariate} \cite{klippel2009colour} \cite{fuchs2014influence} \cite{fuchs2016systematic} \cite{albo2015off} 
&\cite{ribarsky1994glyphmaker} \cite{ren2018charticulator} \cite{brehmer2021generative} \cite{tsandilas2020structgraphics} \cite{tong2016glyphlens}
&\cite{zhao2020iconate}
&\cite{ying2021glyphcreator}
& 14 \\ \hline

\multicolumn{1}{|c|}{\multirow{9}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Narrative\\visualization\end{tabular}}}}} & \textbf{Infographic} 
&\cite{albers2014infographics}  \cite{artacho2008influence} \cite{santos2018influence}  \cite{dunlap2016getting} \cite{harrison2015infographic} \cite{lyra2016infographics} \cite{lan2021smile} 
&\cite{zhang2020dataquilt} \cite{coelho2020infomages} \cite{kim2016data} \cite{cui2021mixed} \cite{wang2018infonice} \cite{kim2019dataselfie} \cite{xia2018dataink} \cite{lee2013sketchstory}
&\cite{lu2020exploring} \cite{tyagi2021user} \cite{chen2019towards} \cite{yuan2021infocolorizer} \cite{visme2013} \cite{infogram2012}
&\cite{qian2020retrieve} \cite{cui2019text} \cite{CANVA2018}
& 24 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Timeline\&Storyline} 
&\cite{brehmer2016timelines} \cite{lan2021understanding} \cite{bach2015time}  \cite{tanahashi2012design}\cite{gronemann2016crossing}  \cite{di2020storyline}
&\cite{dukes2010dipity}\cite{webalon2011tiki}\cite{llc2012timeglider}\cite{TimelineJS2013}\cite{TimelineSetter2011} \cite{brehmer2019timeline} \cite{kim2017visualizing}
&\cite{tang2020plotthread} \cite{liu2013storyflow} \cite{tang2018istoryline} \cite{nguyen2016timesets} \cite{satyanarayan2014authoring} \cite{fulda2015timelinecurator}
&
& 19 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Annotated Chart} 
&\cite{borkin2013makes} \cite{borkin2015beyond} \cite{kong2017internal} 
&\cite{ren2017chartaccent} %后面跟着这3个全是编程工具 \cite{gomez2017ggplot2} \cite{swoopyDragjs2016}\cite{wongsuphasawatlabella2015} 
&\cite{chen2010click2annotate} \cite{chen2010touch2annotate} \cite{kandogan2012just} \cite{bryan2016temporal} \cite{latif2021kori}
&\cite{hullman2013contextifier}  \cite{bylinskii2017understanding} \cite{liu2020autocaption}
& 12 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Data Comics} 
&\cite{zhao2015data} \cite{bach2018design} \cite{zhao2019understanding}  \cite{wang2019comparing} \cite{wang2019teaching} \cite{wang2020data} \cite{bach2017emerging}
&\cite{wang2021interactive} \cite{kim2019datatoon} \cite{kang2021toonnote}
&\cite{zhao2021chartstory}
&\cite{wang2019datashot} \cite{shi2020calliope}
& 13 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Data Videos} 
&\cite{amini2015understanding} \cite{cao2020examining} \cite{shi2021communicating} \cite{tang2020design} \cite{thompson2020understanding} \cite{shu2020makes} \cite{lan2021kineticharts} \cite{wang2016animated} \cite{li2020improving}
&\cite{amini2016authoring} 
&\cite{thompson2021data} \cite{liu2018data} \cite{wang2021animated}
&\cite{shi2021autoclips}
& 14 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & \textbf{Scrollytelling} 
& \cite{seyser2018scrollytelling} \cite{elias2018towards} \cite{hullman2013deeper} \cite{roth2021cartographic}
&\cite{bocklandt2021sandslide} \cite{conlen2018idyll} \cite{sultanum2021leveraging}
&\cite{winters2019automatically}
&\cite{lu2021automatic}
& 9 \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} & 55 & 38 & 37 &24  &154  \\ \hline

\end{tabular}
\end{table*}


==> Table/backup/table1-edit.tex <==
% table1：不同的可视化工具

\renewcommand\arraystretch{1.3}
\begin{table*}[]

\textbf{\caption{Listed by narrative visualization tool type}}
\begin{tabular}{c|m{2cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|c|} \hline

\multicolumn{2}{|c|}{} & \textbf{Design Space} & \textbf{Authoring Tools} & \textbf{AI Suppporte Tools} & \textbf{AI Generator} & \textbf{SUM} \\ \hline


\multicolumn{1}{|c|}{}  & Statistical Chart 
& \cite{grammel2010information} \cite{wang2020cheat} \cite{luo2019enhancing} \cite{spence2005no} \cite{lyi2020comparative}  \cite{kosslyn1989understanding} 
& \cite{fu2020chartem} \cite{cui2021mixed} \cite{liu2018data} \cite{sarvghad2018embedded}  \cite{zong2020lyra} \cite{kong2012graphical}\cite{stolte2002polaris}\cite{ahlberg1996spotfire}\cite{heer2005prefuse} \cite{ren2014ivisdesigner}
&\cite{felix2016texttile}\cite{ren2014weiboevents}\cite{srinivasan2018augmenting}
\cite{satyanarayan2014lyra}\cite{mauri2017rawgraphs}\cite{satyanarayan2016vega} \cite{ren2018charticulator}
\cite{ge2021cast} %\cite{TouchGraph}
&\cite{wongsuphasawat2015voyager}  %\cite{heer2007voyagers}%\cite{borkin2013evaluation}
\cite{luo2018deepeye}\cite{dibia2019data2vis} \cite{hu2019vizml} \cite{moritz2018formalizing}
& 29\\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Timeline 
&  \cite{brehmer2016timelines} \cite{kim2017visualizing} \cite{lan2021understanding} \cite{bach2015time}                  
& \cite{chen2019towards} \cite{fulda2015timelinecurator} % \cite{TimelineJS} \cite{TimelineSetter}
& \cite{nguyen2016timesets} \cite{tang2018istoryline} \cite{tang2020plotthread}
& &9 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Tag Cloud
&  \cite{felix2017taking} \cite{hearst2019evaluation}
& \cite{shu2021dancingwords} \cite{heimerl2014word} \cite{oesper2011wordcloud} \cite{cui2010context}  
& \cite{xu2016semantic} %\cite{wordcloudmaker}         
&\cite{jin2017development}\cite{cheng2014synonym} \cite{wang2017edwordle} %\cite{vizzlo}\cite{wordclouds.com}\cite{wordart}  \cite{WordCloudGenerator}  
&10 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Annotated Chart           
& \cite{borkin2013makes}  \cite{brath2018automated} \cite{borkin2015beyond}                    
& \cite{ren2017chartaccent} \cite{latif2021kori} \cite{liu2020autocaption} \cite{hopkins2020visualint}                            
& \cite{hullman2013contextifier}
& %\cite{kolman2012infomaps}%不应该是generator
&8 \\ \cline{2-7} 

\multicolumn{1}{|c|}{\multirow{}{}{\textbf{Chart}}}    & Other     
& \cite{albo2015off} \cite{roth2021cartographic} %这是一个map
& \cite{henry2007nodetrix} \cite{tsandilas2020structgraphics} \cite{satyanarayan2014authoring}  \cite{fekete2004infovis} \cite{bostock2011d3} \cite{hoelscher2018using} \cite{bostock2009protovis} \cite{dunne2013motif}
%\cite{Cytoscape}\cite{highcharts}
&\cite{abello2006ask}%节点链接图（力导向图）
 %\cite{bastian2009gephi}（不属于期刊论文）
 \cite{gao2014newsviews}%geomap
&%\cite{QuantumGIS} 
&12 \\ \hline


\multicolumn{2}{|c|}{\textbf{Infographics}}               
&  \cite{otten2015infographics} \cite{hearst2017teaching}    \cite{lan2021smile} %\cite{lalle2019gaze}
&  \cite{yuan2021infocolorizer} \cite{xia2018dataink}  \cite{kim2016data} \cite{coelho2020infomages} \cite{wang2021animated}  \cite{lu2020exploring} \cite{wang2018infonice} \cite{tyagi2021user}  %后面这两篇文献是flow chart 
& \cite{visme2013}\cite{infogram2012}
%\cite{CANVA}\cite{lucidpress}\cite{venngage}\cite{piktochart} \cite{visme}\cite{snappa}
&\cite{cui2019text} \cite{CANVA2018}%公司成立于2013年，该软件在2018年推出
& 15 \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Comics}} 
&\cite{wang2020data}\cite{bach2018design} \cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding} \cite{zhao2015data} \cite{bach2017emerging}
& \cite{wang2021interactive}  \cite{kang2021toonnote} \cite{kim2019datatoon}
& \cite{zhao2021chartstory}
& \cite{wang2019datashot}  \cite{shi2020calliope}
&13 \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Videos}} & \cite{shi2021communicating} \cite{amini2015understanding} \cite{thompson2020understanding} \cite{lan2021kineticharts} \cite{li2020improving} \cite{shu2020makes} \cite{tang2020design} \cite{cao2020examining}  
& \cite{wang2016animated} \cite{amini2016authoring}  \cite{chen2021augmenting} 
&\cite{thompson2021data} 
& \cite{shi2021autoclips} &13 \\ \hline


\multicolumn{2}{|c|}{\textbf{Dashboard}} 
& \cite{schwendimann2016perceiving} \cite{froese2016lessons} \cite{sarikaya2018we} \cite{sedrakyan2019guiding} \cite{molenaar2018teachers} \cite{cha2019applying}    \cite{qu2017keeping} \cite{chen2020composition} \cite{few2007dashboard}   \cite{elias2012annotating}
& \cite{elias2011exploration} \cite{bajzek2007inventing} \cite{ma2020ladv}  \cite{becker2019microsoft}
& 
&   \cite{datapine2012} \cite{thoughtspot2012}%这两款工具都是开发于2012年，在后续的版本迭代中逐渐增加了AI功能
\cite{QlikSense2010}\cite{IBMCognosAnalytics}
\cite{SisenseFusionAnalytics2019}%重新确认这三个是否是全自动的
&19 \\ \hline


\multicolumn{2}{|c|}{\textbf{Scrollytelling}} 
&\cite{joshi2021learning} %\cite{chen2006tiling}
& \cite{wang2018narvis}\cite{sultanum2021leveraging} 
&\cite{lu2021automatic} 
&% \cite{leake2020generating}
%\cite{hinrichs2008emdialog} %表示怀疑  
%\cite{dunker2009semantic}%这一个工具是对自动化幻灯片的一个概念，应该放到design space还是Authoring tools中。%\cite{Flourish}
&4 \\ \hline
 
\multicolumn{2}{|c|}{\textbf{Glyph}} 
&\cite{fuchs2014influence} \cite{roberts2005haptic} \cite{borgo2013glyph} \cite{fuchs2016systematic} \cite{maguire2012taxonomy}  \cite{chung2014glyph}  
\cite{ropinski2011survey} 
& \cite{brehmer2021generative}  
&\cite{zhao2020iconate} %这是关于多维icon的生成，是否要放到glyph中
&\cite{ying2021glyphcreator} &10  \\ \hline

\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Immersive\\ Narrative Tools\end{tabular}}} 
&\cite{kraus2021value} \cite{isenberg2018immersive} \cite{zikas2020immersive} 
&\cite{chen2019marvist} \cite{sicat2018dxr}
& \cite{dang2021gesturemap}
& %\cite{palmas2014movexp} %\cite{jing2021eyemr} %最后两个虽然是Immersive vis，但是和数据可视化没有关系
&6  \\ \hline
 
\multicolumn{2}{|c|}{\textbf{SUM}} &57  &  51   & 21 & 20 & 149                                        \\ \hline



\end{tabular}
\end{table*}

==> Table/backup/table1.tex <==
% table1：不同的可视化工具

%已确定，不再更改

%20220112前编辑好的内容
\renewcommand\arraystretch{1.3}
\begin{table*}[]

\textbf{\caption{Listed by narrative visualization tool type}}
\begin{tabular}{c|m{2cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|m{2.7cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{{\color[HTML]{333333} \textbf{Type}}}                                         & {\color[HTML]{333333} \textbf{Design Space}} & {\color[HTML]{333333} \textbf{Authoring Tool}} & {\color[HTML]{333333} \textbf{AI-Supported Tools}} & {\color[HTML]{333333} \textbf{AI Generator}} & {\color[HTML]{333333} \textbf{SUM}}\\ \hline

\multicolumn{1}{|c|}{}  & Statistical Chart 
& \cite{grammel2010information} \cite{wang2020cheat} \cite{luo2019enhancing} \cite{spence2005no} \cite{lyi2020comparative}  \cite{kosslyn1989understanding} 
& \cite{ren2018charticulator} \cite{fu2020chartem} \cite{cui2021mixed} \cite{liu2018data} \cite{sarvghad2018embedded}  \cite{zong2020lyra} \cite{kong2012graphical}\cite{stolte2002polaris}\cite{ahlberg1996spotfire}\cite{heer2005prefuse}
&\cite{vartak2015seedb}\cite{coene2018sigmajs}\cite{saket2016visualization}\cite{eirich2021irvine}\cite{harrison2017petminer}\cite{felix2016texttile}\cite{felix2015revex}\cite{ren2014weiboevents}\cite{ge2020canis}\cite{srinivasan2018augmenting}\cite{ren2014ivisdesigner}\cite{satyanarayan2014lyra}\cite{mauri2017rawgraphs}\cite{satyanarayan2016vega} %\cite{TouchGraph}
&\cite{kandel2012profiler}\cite{heer2007voyagers}\cite{wongsuphasawat2015voyager}\cite{mackinlay2007show}\cite{gratzl2013lineup} \cite{borkin2013evaluation}\cite{luo2018deepeye}\cite{abello2006ask}\cite{dibia2019data2vis}\cite{GoldenSoftware} \cite{datawrapper} \cite{visme}& 42\\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Timeline 
&  \cite{brehmer2016timelines} \cite{kim2017visualizing} \cite{lan2021understanding} \cite{bach2015time}                  
& \cite{chen2019towards} \cite{fulda2015timelinecurator} % \cite{TimelineJS} \cite{TimelineSetter}
& 
&\cite{nguyen2016timesets} &7 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Tag Cloud
&  \cite{felix2017taking} 
& \cite{shu2021dancingwords} \cite{heimerl2014word} \cite{oesper2011wordcloud} \cite{wang2017edwordle} \cite{cui2010context}                 
& \cite{jin2017development}  %\cite{wordcloudmaker}                                              
& %\cite{vizzlo}\cite{wordclouds.com}\cite{wordart}  \cite{WordCloudGenerator}  
&7 \\ \cline{2-7} 

\multicolumn{1}{|c|}{} & Annotated Chart           
&   \cite{borkin2013makes}  \cite{brath2018automated} \cite{borkin2015beyond}                    
& \cite{ren2017chartaccent} \cite{latif2021kori} \cite{liu2020autocaption} \cite{hopkins2020visualint}                            
& 
& \cite{kolman2012infomaps}&8 \\ \cline{2-7} 

\multicolumn{1}{|c|}{\multirow{}{}{\textbf{Chart}}}    & Other     
& \cite{roth2021cartographic} %这是一个map
& \cite{henry2007nodetrix} \cite{tsandilas2020structgraphics} \cite{satyanarayan2014authoring}  \cite{fekete2004infovis} \cite{bostock2011d3} \cite{hoelscher2018using} \cite{bostock2009protovis}
%\cite{Cytoscape}\cite{highcharts}
& \cite{bastian2009gephi}
&\cite{gao2014newsviews}%\cite{QuantumGIS} 
&10 \\ \hline


\multicolumn{2}{|c|}{\textbf{Infographics}}               
&  \cite{otten2015infographics} \cite{hearst2017teaching}    \cite{lan2021smile} \cite{lalle2019gaze}
&  \cite{yuan2021infocolorizer} \cite{xia2018dataink}  \cite{kim2016data} \cite{coelho2020infomages}  \cite{lu2020exploring} \cite{tyagi2021user} %后面这两篇文献是flow chart 
&%\cite{CANVA}\cite{lucidpress}\cite{venngage}\cite{piktochart} \cite{visme}\cite{snappa}

\multicolumn{2}{|c|}{\textbf{Data Comics}} &\cite{wang2020data}\cite{bach2018design} \cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding} & \cite{wang2021interactive}  \cite{kang2021toonnote} \cite{wang2019datashot}
& \cite{zhao2021chartstory}\cite{kim2019datatoon} &\cite{tobita2015comic}\cite{shi2020calliope}
&12 \\ \hline

\multicolumn{2}{|c|}{\textbf{Data Videos}}
& \cite{shi2021communicating} \cite{amini2015understanding} \cite{thompson2020understanding} \cite{lan2021kineticharts} \cite{li2020improving} \cite{shu2020makes} \cite{tang2020design}  
& \cite{wang2016animated} \cite{amini2016authoring}  \cite{chen2021augmenting} \cite{cao2020examining} \cite{wang2021animated} 
&\cite{thompson2021data} 
&  \cite{shi2021autoclips} &14 \\ \hline


\multicolumn{2}{|c|}{\textbf{Dashboard}} 
& \cite{schwendimann2016perceiving} \cite{froese2016lessons} \cite{sarikaya2018we} \cite{sedrakyan2019guiding} \cite{molenaar2018teachers} \cite{cha2019applying}    \cite{qu2017keeping} \cite{chen2020composition} \cite{few2007dashboard}  \cite{elias2012annotating} 
& \cite{elias2011exploration} \cite{bajzek2007inventing} \cite{ma2020ladv} % \cite{datapine}\cite{tiwari202170} 
&  \cite{becker2019microsoft}\cite{loorak2015timespan}  
&  \cite{siddiqui2017fast}\cite{ai2015neuroblocks}\cite{hullman2013contextifier}\cite{nadhani2012fusioncharts} \cite{Metabase} \cite{Geckoboard} \cite{infogram} \cite{datapine} \cite{thoughtspot} \cite{Einbrick}
&25 \\ \hline


\multicolumn{2}{|c|}{\textbf{Slideshow}} &\cite{joshilearning}  & \cite{wang2018narvis}\cite{sultanum2021leveraging} &\cite{tang2020plotthread}\cite{lu2021automatic} &\cite{hinrichs2008emdialog} %\cite{Flourish} 
&6 \\ \hline
 
\multicolumn{2}{|c|}{\textbf{Glyph}} &\cite{fuchs2014influence} \cite{roberts2005haptic} \cite{borgo2013glyph} \cite{fuchs2016systematic} \cite{maguire2012taxonomy} \cite{ropinski2011survey} \cite{chung2014glyph} \cite{albo2015off}  & \cite{brehmer2021generative} \cite{dunne2013motif}  
&\cite{sanyal2010noodles}\cite{chevalier2018using}\cite{zhao2020iconate} & &13  \\ \hline

\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Immersive\\ Narrative Tools\end{tabular}}} &\cite{kraus2021value}\cite{spaulding2013design} \cite{isenberg2018immersive} \cite{chen2017exploring}
&\cite{chen2019marvist} & \cite{sicat2018dxr} &\cite{dang2021gesturemap}\cite{palmas2014movexp}\cite{jing2021eyemr} \cite{nebeling2020mrat}&10  \\ \hline
 
\multicolumn{2}{|c|}{\textbf{SUM}} &54  &  50   & 28 & 35 & 167                                        \\ \hline



\end{tabular}
\end{table*}




==> Table/backup/table2-0329-edit.tex <==
\renewcommand\arraystretch{1.5}
\begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}

\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Traditional\\visualization\end{tabular}}}}} & \textbf{Statistical Chart} 
&
&
&
&
&
&\cite{huron2014constructing}\cite{satyanarayan2014lyra}
&\cite{vartak2015seedb}\cite{wongsuphasawat2015voyager}
& \cite{wun2016comparing}\cite{mendez2016ivolver}\cite{wongsuphasawat2016towards}
&\cite{mauri2017rawgraphs}
&\cite{saket2018task}\cite{moritz2018formalizing}\cite{luo2018deepeye}
&\cite{luo2019enhancing}\cite{hu2019vizml}\cite{dibia2019data2vis}
&\cite{lyi2020comparative}\cite{wang2020cheat}\cite{zong2020lyra}\cite{hopkins2020visualint}\cite{lin2020dziban} \cite{zhang2020viscode} \cite{fu2020chartem}\cite{zhou2020table2analysis} \cite{ge2020canis}\cite{li2020research}\cite{zhao2020chartseer}
&\cite{chen2021augmenting}\cite{chen2021vizlinter}\cite{ge2021cast}\cite{zhou2021table2charts}
& 29
\\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Other} 
&
&
&
&
&
&
&
&
&
&
&
&
&
&  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Dashboard} 
&\cite{tableau2006}\cite{ahlberg1996spotfire} \cite{cutroni2007google}
&\cite{QlikSense2010}
&\cite{elias2011exploration}
&\cite{javed2012exploring}\cite{elias2012annotating}\cite{datapine2012}\cite{thoughtspot2012}
&
&\cite{belo2014restructuring}
&
&\cite{froese2016lessons}
&\cite{qu2017keeping}\cite{dabbebi2017towards}\cite{santos2017data}
&\cite{sarikaya2018we}
&\cite{vazquez2019extending}\cite{SisenseFusionAnalytics2019}
&\cite{chen2020composition}\cite{elshehaly2020qualdash}\cite{ma2020ladv}
&
&20  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Glyph} 
&\cite{yost2005single} \cite{ward2008multivariate} \cite{klippel2009colour}\cite{ribarsky1994glyphmaker}
&
&
&
&\cite{borgo2013glyph}
&\cite{fuchs2014influence}
&\cite{albo2015off} 
&\cite{fuchs2016systematic}\cite{tong2016glyphlens}
&
&\cite{ren2018charticulator}
&
&\cite{tsandilas2020structgraphics}\cite{zhao2020iconate}
&\cite{brehmer2021generative}\cite{ying2021glyphcreator}
& 14 \\ \hline

\multicolumn{1}{|c|}{\multirow{6}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Narrative\\visualization\end{tabular}}}}} 
& \textbf{Infographic}

&\cite{artacho2008influence}
&
&
&\cite{infogram2012}
&\cite{lee2013sketchstory}\cite{visme2013} 
&\cite{albers2014infographics}
&\cite{harrison2015infographic}
&\cite{dunlap2016getting}\cite{lyra2016infographics}\cite{kim2016data}
&
&\cite{santos2018influence} \cite{wang2018infonice}\cite{xia2018dataink}\cite{CANVA2018}
&\cite{kim2019dataselfie}\cite{chen2019towards}\cite{cui2019text}
&\cite{zhang2020dataquilt}\cite{coelho2020infomages}\cite{lu2020exploring}\cite{qian2020retrieve}
&\cite{lan2021smile} \cite{cui2021mixed}\cite{tyagi2021user} \cite{yuan2021infocolorizer}
& 24 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Timeline} 
&
&\cite{dukes2010dipity}
&\cite{webalon2011tiki}\cite{TimelineSetter2011}
&\cite{tanahashi2012design}\cite{llc2012timeglider}
&\cite{TimelineJS2013}\cite{liu2013storyflow}
&\cite{satyanarayan2014authoring}
&\cite{bach2015time}\cite{fulda2015timelinecurator}
&\cite{brehmer2016timelines}\cite{gronemann2016crossing} \cite{nguyen2016timesets}
&\cite{kim2017visualizing}
&\cite{tang2018istoryline}
&\cite{brehmer2019timeline}
&\cite{di2020storyline}\cite{tang2020plotthread}
&\cite{lan2021understanding}
& 19 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Annotated Chart} 
&
&\cite{chen2010click2annotate} \cite{chen2010touch2annotate}
&
&\cite{kandogan2012just}
&\cite{borkin2013makes}\cite{hullman2013contextifier}
&
&\cite{borkin2015beyond}
&\cite{bryan2016temporal}
&\cite{kong2017internal} \cite{ren2017chartaccent} \cite{bylinskii2017understanding}
&
&
&\cite{liu2020autocaption}
&\cite{latif2021kori}
& 12 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Data Comics} 
&
&
&
&
&
&
&\cite{zhao2015data}
&
&\cite{bach2017emerging}
&\cite{bach2018design}
&\cite{zhao2019understanding}  \cite{wang2019comparing} \cite{wang2019teaching}\cite{kim2019datatoon}\cite{wang2019datashot}
&\cite{shi2020calliope}\cite{wang2020data}
&\cite{wang2021interactive}\cite{kang2021toonnote}\cite{zhao2021chartstory}
& 13 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Data Videos} 

&
&
&
&
&
&
&\cite{amini2015understanding}
&\cite{wang2016animated}\cite{amini2016authoring} 
&
&\cite{liu2018data}
&
&\cite{cao2020examining}\cite{tang2020design} \cite{thompson2020understanding} \cite{shu2020makes}\cite{li2020improving}
&\cite{shi2021communicating} \cite{lan2021kineticharts}\cite{thompson2021data}\cite{wang2021animated}\cite{shi2021autoclips}
&14 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Scrollytelling} 
&
&
&
&
&\cite{hullman2013deeper}
&
&
&
&
&\cite{seyser2018scrollytelling}\cite{elias2018towards}\cite{conlen2018idyll}
&\cite{winters2019automatically}
&
&\cite{roth2021cartographic}\cite{bocklandt2021sandslide}\cite{sultanum2021leveraging}\cite{lu2021automatic}
& 9 \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}}
&
&
&
&
&
&
&
&
&
&
&
&
&
&  \\ \hline
\end{tabular}
\end{table*}

==> Table/backup/table2-0329.tex <==
\renewcommand\arraystretch{1.5}
\begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Traditional\\visualization\end{tabular}}}}} & \textbf{Statistical Charts} 
&  &  &  &  &  & 2 & 2 & 3 & 1 & 3 & 3 & 11 & 4 & 29   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Other Charts} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Dashboard} & 3 & 1 & 1 & 4 &  & 1 &  & 1 & 3 & 1 & 2 & 3 &  & 20  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Glyphs} & 4 &  &  &  & 1 & 1 & 1 & 2 &  & 1 &  & 2 & 2 & 14  \\ \hline

\multicolumn{1}{|c|}{\multirow{6}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Narrative\\visualization\end{tabular}}}}} & \textbf{Infographic} & 1 &  &  & 1 & 2 & 1 & 1 & 3 &  & 4 & 3 & 4 & 4 & 24  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Timeline\&Storyline} &  & 1 & 2 & 2 & 2 & 1 & 2 & 3 & 1 & 1 & 1 & 2 & 1 & 19  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Annotated Chart} &  & 2 &  & 1 & 2 &  & 1 & 1 & 3 &  &  & 1 & 1 & 12  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Data Comics} &  &  &  &  &  &  & 1 &  & 1 & 1 & 5 & 2 & 3 & 13  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Data Videos} &  &  &  &  &  &  & 1 & 2 &  & 1 &  & 5 & 5 & 14 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Scrollytelling} &  &  &  &  & 1 &  &  &  &  & 3 & 1 &  & 4 & 9 \\ \hline
\multicolumn{2}{|c|}{\textbf{SUM}} & 8 & 4 & 3 & 8 & 8 & 6 & 9 & 15 & 9 & 15 & 15 & 30 & 24 & 154 \\ \hline
\end{tabular}
\end{table*}

==> Table/backup/table2.tex <==
%[Table2:与年份对应的表格]
 \begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
 \hline
 \textbf{}  & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline
\textbf{Chart}        & 9  & 2 & 2 & 1 & 3 & 7 & 5 & 5 & 6 & 9 & 5 & 8 & 6 & 68           \\ \hline
\textbf{Infographics} &     &   &   & 1  & 1  &   & 1 & 1 & 1 & 3 & 2 & 2 & 4 & 16           \\ \hline
\textbf{Data Comics}  &     &   &   &   &   &   & 1 &   & 1  & 1 & 5 & 2 & 3 & 13           \\ \hline
\textbf{Data Videos}  &    &   &  &   &   &    & 1 & 2 &   &  &   & 5 & 5 & 13          \\ \hline
\textbf{Dashboard}    & 3   & 1  &1   & 3 &  &  &  & 2 & 1 & 2 & 4 & 2 &  & 18           \\ \hline
\textbf{Scrollytelling}    &    &   &   &   &   &   &   &   &   & 1 &   &1  & 3 & 5           \\ \hline
\textbf{Glyph}        & 1   &  & 1 & 1 & 1 & 2 &  & 1 &   &  &  & 1 &2  & 10          \\ \hline
\textbf{Immersive}    &     &   &   &   &   &  &   &   &   & 2 &1   & 1 & 2 & 6           \\ \hline
\textbf{SUM}          & 13  & 3 & 4 & 6 & 5 & 9 & 8 & 11 & 9 & 17 & 17 & 22 & 25 & 149    \\ \hline
 \end{tabular}
 \end{table*}

==> Table/backup/table3-0228-edit.tex <==
\renewcommand\arraystretch{0.8}
\begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
\begin{tabular}{|cc|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \multicolumn{1}{c|} {\textbf{SUM}} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Chart}}}} 
%--------------------- Chart-------------------
& \textbf{Design Space} 
&% \cite{spence2005no}\cite{collins2009parallel}\cite{bateman2008seeing}\cite{rivadeneira2007getting}\cite{halvey2007assessment}\cite{schrammel2009visual}\cite{shaw2005utilizing}\cite{dubinko2007visualizing}\cite{bielenberg2005groups}\cite{seifert2008beauty}\cite{kaser2007tag}\cite{dent2008thematic}\cite{schulz2007interactive}\cite{balzer2005voronoi}\cite{wattenberg2005note}  \cite{harrower2001visualizing}\cite{harrower2003tips}\cite{ghoniem2004comparison}
&%\cite{cui2010context}\cite{lee2010sparkclouds}\cite{kong2010perceptual}\cite{schulz2010design} \cite{battersby2010considerations}\cite{duncan2010lombardi}
&%\cite{wu2011semantic}\cite{kim2011wordbridge}\cite{schulz2011treevis}
&%\cite{javed2012exploring}\cite{paulovich2012semantic} \cite{baudel2012capturing}
&%\cite{gansner2013interactive}\cite{abuthawabeh2013finding}\cite{dunne2013motif}\cite{schulz2013generative}
&%\cite{huron2014constructing}\cite{gramazio2014relation}\cite{rufiange2014animatrix}
&%\cite{chi2015morphable}\cite{marta2015story} 
&%\cite{wun2016comparing}\cite{denil2016storied}
&%\cite{sarikaya2017scatterplots}\cite{felix2017taking}
&%\cite{saket2018task}\cite{murakami2018depth} \cite{okoe2018node}\cite{romat2018animated}\cite{kopp2018temporal}\cite{soares2018visualizing}
&%\cite{luo2019enhancing}\cite{hearst2019evaluation}
&%\cite{wang2020cheat}\cite{lyi2020comparative}\cite{scheibel2020taxonomy} \cite{scheibel2020survey}
&%\cite{roth2021cartographic} \cite{biriukov2021storytelling}
&57  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} 
&%\cite{mackinlay2007show}\cite{viegas2009participatory}\cite{mapcreator2007}\cite{smith2009analyzing}  \cite{ellson2004graphviz} \cite{bastian2009gephi} \cite{auber2004tulip} \cite{dohleman2006exploratory}\cite{hagberg2008exploring}\cite{henry2007matlink} \cite{henry2007nodetrix}
&%\cite{koh2010maniwordle}
&%\cite{bostock2011d3}\cite{oesper2011wordcloud}\cite{gove2011netvisia}
&% \cite{strobelt2012rolled}\cite{arcgis2012} \cite{rufiange2012treematrix}
&%\cite{waldner2013facetclouds}\cite{rufiange2013diffani}
&%\cite{satyanarayan2014lyra}\cite{ren2014ivisdesigner}\cite{heimerl2014word}\cite{Peixoto2014graphtool}\cite{khomtchouk2014heatmapgenerator}
&%\cite{jo2015wordleplus}\cite{mapme2015}\cite{blanch2015dendrogramix}
&% \cite{mendez2016ivolver}\cite{satyanarayan2016vega}
&%\cite{mauri2017rawgraphs}\cite{linhares2017dynetvis}\cite{fernandez2017clustergrammer}
&%\cite{liu2018data}\cite{li2018echarts}\cite{mei2018viscomposer}
&%\cite{becker2019microsoft}\cite{romat2019expressive}\cite{aslak2019netwulf}\cite{angori2019chordlink}
&%\cite{zong2020lyra}\cite{scribblemaps2020}\cite{eaton2020toytree}
&
& 43  \\ \cline{2-16} 
 
\multicolumn{1}{|c|}{} & \textbf{AI-Supported}
&%  \cite{abello2006ask}
&%
&%
&%\cite{kong2012graphical}
&%
&%
&%\cite{lohmann2015concentri}
&%\cite{xu2016semantic}
&% \cite{wang2017edwordle}\cite{liu2017egocomp}
&%\cite{srinivasan2018augmenting} \cite{ren2018charticulator}\cite{moritz2018formalizing}
&%\cite{wang2019deepdrawing}
&%\cite{zhang2020viscode}\cite{fu2020chartem} \cite{li2020research}\cite{lin2020dziban} \cite{ge2020canis}\cite{hopkins2020visualint}
&%\cite{ge2021cast}\cite{chen2021vizlinter}\cite{chen2021augmenting}\cite{shu2021dancingwords}
& 20 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
&% \cite{heer2007voyagers}
&%
&%
&%
&%
&%\cite{cheng2014synonym}\cite{gao2014newsviews}  
&%\cite{wongsuphasawat2015voyager}\cite{vartak2015seedb}
&%\cite{wongsuphasawat2016towards}
&%\cite{jin2017development}
&%\cite{luo2018deepeye}
&%\cite{dibia2019data2vis}\cite{hu2019vizml} \cite{wang2019shapewordle}
&%\cite{zhao2020chartseer}\cite{zhou2020table2analysis}
&%\cite{zhou2021table2charts}
& 14 \\ \hline

%--------------------- Infograpics %20220228-搞定 -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Infograpics}}}}  &%
\textbf{Design Space} 
&% \cite{artacho2008influence}\cite{risch2008role}\cite{havre2002themeriver}  \cite{byron2008stacked}\cite{yost2005single} \cite{klippel2009colour}\cite{roberts2005haptic} \cite{ward2008multivariate}
&%
&%\cite{diakopoulos2011playable}\cite{moere2011role} \cite{aigner2011visualization}
&%\cite{smiciklas2012power}\cite{tanahashi2012design}\cite{kandogan2012just}
&%\cite{borkin2013makes}\cite{borgo2013glyph}
&%\cite{albers2014infographics}\cite{fuchs2014influence}
&%\cite{harrison2015infographic}\cite{otten2015infographics}\cite{albers2015infographics} \cite{jones2015information}\cite{tanahashi2015efficient}\cite{bach2015time}\cite{borkin2015beyond}
&%\cite{dunlap2016getting}\cite{lyra2016infographics}\cite{cmeciu2016beyond}\cite{kosara2016presentation}\cite{gronemann2016crossing}\cite{fuchs2016systematic}
&%\cite{hearst2017teaching}\cite{naparin2017infographics}\cite{kong2017internal}
&% \cite{santos2018influence}\cite{brath2018automated}
&%
&%\cite{di2020storyline}
&%\cite{lan2021smile}\cite{lan2021understanding}
&39   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} 
&% \cite{ribarsky1994glyphmaker}
&%\cite{Preceden2010}\cite{dukes2010dipity}
&%\cite{webalon2011tiki}\cite{TimelineSetter2011}
&%\cite{llc2012timeglider}
&%\cite{lee2013sketchstory}\cite{TimelineJS2013}
&%
&%\cite{wongsuphasawatlabella2015}
&%\cite{kim2016data}\cite{qiang2016storycake}\cite{brehmer2016timelines}\cite{swoopyDragjs2016}\cite{tong2016glyphlens}
&%\cite{kim2017visualizing}\cite{gomez2017ggplot2}\cite{ren2017chartaccent}
&%\cite{madan2018synthetically}\cite{xia2018dataink}  \cite{wang2018infonice}
&%\cite{kim2019dataselfie}\cite{brehmer2019timeline}
&%\cite{zhang2020dataquilt} \cite{coelho2020infomages}\cite{agarwal2020set}\cite{tsandilas2020structgraphics}
&%\cite{cui2021mixed}\cite{brehmer2021generative}
& 28 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Supported} 
&% 
&%\cite{chen2010click2annotate} \cite{chen2010touch2annotate}
&%
&%\cite{infogram2012}
&%\cite{visme2013}\cite{liu2013storyflow}\cite{hullman2013contextifier}
&%\cite{satyanarayan2014authoring}
&%\cite{fulda2015timelinecurator}
&%\cite{nguyen2016timesets}\cite{bryan2016temporal}
&% \cite{bylinskii2017understanding}
&%\cite{tang2018istoryline}
&%\cite{chen2019towards}
&%\cite{lu2020exploring}\cite{tang2020plotthread}\cite{zhao2020iconate}
&%\cite{tyagi2021user} \cite{yuan2021infocolorizer}\cite{latif2021kori}
&  19 \\ \cline{2-16} 
    
 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
& 
&
&
&
&
&
&
&
&
&%\cite{CANVA2018} \cite{park2018graphoto}
&%\cite{cui2019text}
&%\cite{qian2020retrieve}\cite{liu2020autocaption}
&%\cite{ying2021glyphcreator}
& 6 \\ \hline

%--------------------- Data Comics  %20220228-搞定   -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Data Comics}}}} 
& \textbf{Design Space}
& 
&
&
&
&
&
&\cite{zhao2015data}
&
&\cite{bach2017emerging}
&\cite{bach2018design}
&\cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding}
&\cite{wang2020data}
&
&  7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
& 
&
&
&
&
&
&
&
&
&
&\cite{kim2019datatoon}
&
&\cite{wang2021interactive}  \cite{kang2021toonnote}
&3   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
& 
&
&
&
&
&
&
&
&
&
&
&
&\cite{zhao2021chartstory}
& 1  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
& 
&
&
&
&
&
&
&
&
&
&\cite{wang2019datashot}
&\cite{shi2020calliope}
&
& 2 \\ \hline


%---------------------Data Videos %20220228-搞定 -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Data Videos}}}}  
& \textbf{Design Space}
& 
&
&
&
&
&
&\cite{amini2015understanding}
&\cite{wang2016animated}
&
&
&
&\cite{cao2020examining}\cite{thompson2020understanding}\cite{tang2020design}\cite{li2020improving}\cite{shu2020makes}
&\cite{shi2021communicating}\cite{lan2021kineticharts}
&7  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
& 
&
&
&
&
&
&
&\cite{amini2016authoring}
&
&
&
&
&\cite{chen2021augmenting}
& 2  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
& 
&
&
&
&
&
&
&
&
&
&
&
&\cite{thompson2021data} \cite{wang2021animated} 
& 2 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
& 
&
&
&
&
&
&
&
&
&
&
&
&\cite{shi2021autoclips}
&1  \\ \hline


%---------------------Dashboard %20220227-搞定 -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Dashboard}}}} 
& \textbf{Design Space}
& 
&
&
&
&
&
&
&\cite{froese2016lessons}
&\cite{laubheimer2017dashboards} \cite{qu2017keeping}
&\cite{sarikaya2018we}
&\cite{vazquez2019extending}\cite{vazquez2019information}
&\cite{chen2020composition}
&
&7  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
& \cite{tableau2003}\cite{ahlberg1996spotfire}\cite{cutroni2007google}
&
&\cite{elias2011exploration}
&\cite{choosel2012}
&\cite{filonik2013customisable} 
&
&
&
&
&
&
&
&
& 6   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Supported}
& 
&
&
&
&
&\cite{belo2014restructuring}
&
&
&\cite{dabbebi2017towards}\cite{santos2017data}
&
&
&\cite{elshehaly2020qualdash}\cite{ma2020ladv}
&
&5  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
& 
&\cite{QlikSense2010}
&
&\cite{datapine2012}\cite{thoughtspot2012}
&
&
&
&
&
&
&\cite{SisenseFusionAnalytics2019}
&
&
& 4  \\ \hline


%---------------------Scrollytelling %20220227-搞定 -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Scrollytelling}}}} 
& \textbf{Design Space}
&
&
&
&
&\cite{hullman2013deeper}
&
&
&
&
&\cite{seyser2018scrollytelling}\cite{elias2018towards}
&
&
&\cite{roth2021cartographic}
&4  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&
&
&\cite{conlen2018idyll}
&
&
&\cite{bocklandt2021sandslide}\cite{sultanum2021leveraging} 
&  3 \\ \cline{2-16} 


\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&
&\cite{winters2019automatically}
&
&
& 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
&
&
&
&
&
&
&
&
&
&
&
&
&\cite{lu2021automatic}
& 1 \\ \hline

%---------------------Immersive %20220227-搞定 -------------------
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Immersive}}}} & \textbf{Design Space}
& \cite{raja2004exploring}
&
&
&
&
&
&
&
&\cite{vierjahn2017towards}\cite{bach2017hologram}\cite{bach2017drawing}
&\cite{isenberg2018immersive}
&
& \cite{liu2020design}
&\cite{kraus2021value}
& 7 \\ \cline{2-16} 


\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
& 
&
&
&
&
&\cite{donalek2014immersive}
&
&\cite{cordeil2016immersive}\cite{filonik2016glance}
&
&\cite{butscher2018clusters}\cite{sicat2018dxr} 
&\cite{chen2019marvist}
&
&
&  6 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Supported}
& 
&
&
&
&
&
&
&
&
&
&
&
&
& \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Generator} 
& 
&
&
&
&
&
&
&
&
&
&
&
&
&  \\ \hline


\multicolumn{2}{|c|}{\textbf{SUM}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table*}

==> Table/backup/table3-0228.tex <==
\renewcommand\arraystretch{1.5}
\begin{table*}
\textbf{ \caption{Listed by year of publication of narrative visualization and tool type}}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \multicolumn{1}{c|} {\textbf{SUM}} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Chart}}}} 
& \textbf{Design Space} & 18 & 6 & 3 & 3 & 4 & 3 & 2 & 2 & 2 & 6 & 2 & 4 & 2 & 57  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 11 & 1 & 3 & 3 & 2 & 5 & 3 & 2 & 3 & 3 & 4 & 3 &  & 43 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai-Supported}& 1 &  &  & 1 &  &  & 1 & 1 & 2 & 3 & 1 & 6 & 4 & 20  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} & 1 &  &  &  &  & 2 & 2 & 1 & 1 & 1 & 3 & 2 & 1 & 14  \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Infograpics}}}}  
& \textbf{Design Space} & 8 &  & 3 & 3 & 2 & 2 & 7 & 6 & 2 & 2 &  & 1 & 2 & 38   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 1 & 2 & 2 & 1 & 2 &  & 1 & 5 & 3 & 3 & 2 & 4 & 2 & 28 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai Supported} &  & 2 &  & 1 & 3 & 1 & 1 & 2 & 1 & 1 & 1 & 3 & 3 & 19 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}  &  &  &  &  &  &  &  &  &  & 2 & 1 & 2 & 1 & 6 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Data Comics}}}} 
& \textbf{Design Space} &  &  &  &  &  &  & 1 &  & 1 & 1 & 3 & 1 &  & 7  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  &  & 1 &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai Supported} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  & 1 & 1 &  & 2 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Data Videos}}}}  
& \textbf{Design Space} &  &  &  &  &  &  & 1 & 1 &  &  &  & 5 & 2 & 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  & 1 &  &  &  &  & 1 & 2\\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai Supported}  &  &  &  &  &  &  &  &  &  &  &  &  & 2 & 2  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}  &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1  \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Dashboard}}}} 
& \textbf{Design Space}  &  &  &  &  &  &  &  & 1 & 2 & 1 & 2 & 1 &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 3 &  & 1 &  & 1 &  &  &  &  &  &  &  &  & 5 \\ \cline{2-16}
\multicolumn{1}{|c|}{} & \textbf{Ai Supported} &  &  &  &  &  & 1 &  &  & 2 &  &  & 2 &  & 5  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  & 1 &  & 2 &  &  &  &  &  &  & 1 &  &  & 4 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Scrollytelling}}}} 
& \textbf{Design Space} &  &  &  &  & 1 &  &  &  &  & 2 &  &  & 1 & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  & 1 &  &  & 2 & 3  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai Supported}  &  &  &  &  &  &  &  &  &  &  & 1 &  &  & 1  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Immersive}}}} 
& \textbf{Design Space} & 1 &  &  &  &  &  &  &  & 3 & 1 &  & 1 & 1 & 7  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  & 1 &  & 2 &  & 2 & 1 &  &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Ai Supported} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} & 44 & 12 & 12 & 14 & 15 & 15 & 19 & 24 & 22 & 29 & 24 & 36 & 29 & 295 \\ \hline 
\end{tabular}
\end{table*}









==> Table/backup/table3-0401-edit.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{1.5}
\begin{table*}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}

\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{2022} & \textbf{SUM} \\ \hline
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Statistical \\ Charts\end{tabular}}}}}& \textbf{Design Space} 
&
&
&
&
&
&\cite{huron2014constructing}
&
&\cite{wun2016comparing}
&
&\cite{saket2018task}
&\cite{luo2019enhancing}
&\cite{lyi2020comparative} \cite{wang2020cheat}
& 
& 6 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&\cite{satyanarayan2014lyra}
&
&\cite{mendez2016ivolver}
&\cite{mauri2017rawgraphs}
&
&
&\cite{zong2020lyra}
&\cite{chen2021augmenting}
& 5 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Supported}
 \cite{elshehaly2020qualdash} \cite{dabbebi2017towards}  \cite{ma2020ladv}

&
&
&
&
&
&\cite{belo2014restructuring}
&
&
&
& \cite{moritz2018formalizing}
&
&\cite{hopkins2020visualint}\cite{lin2020dziban} \cite{zhang2020viscode} \cite{fu2020chartem} \cite{ge2020canis}\cite{li2020research}
& \cite{chen2021vizlinter}\cite{ge2021cast}
& 9 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&\cite{vartak2015seedb}\cite{wongsuphasawat2015voyager}
&\cite{wongsuphasawat2016towards}
&
&\cite{luo2018deepeye}
&\cite{hu2019vizml}\cite{dibia2019data2vis}
&\cite{zhao2020chartseer}\cite{zhou2020table2analysis}
&  \cite{zhou2021table2charts}
&9 \\ \hline


\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Other \\ Charts\end{tabular}}}}} & \textbf{Design Space} 
&
&
&
&
&
&
&
&
&
&
&
&
& 
&  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&
&
&
&
&
& 
& \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&
&
&
& 
& \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&
&
& 
& \\ \hline

%&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&&

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Dashboard}}}} & 
\textbf{Design Space} 
&
&
&
&\cite{javed2012exploring}
&
&\cite{gramazio2014relation}
&
&\cite{froese2016lessons}
&\cite{qu2017keeping}
&\cite{sarikaya2018we}
&\cite{vazquez2019extending} \cite{suprata2019data} 
&\cite{chen2020composition}
& 
&\cite{fernandez2022beyond}
& 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&\cite{tableau2006}\cite{ahlberg1996spotfire} 
&
&\cite{elias2011exploration}
&\cite{elias2012annotating}
&
&
&
&
&
&
&
&
& 
&
& 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&\cite{belo2014restructuring}
&
&
&\cite{dabbebi2017towards}
&
&
&\cite{elshehaly2020qualdash}\cite{ma2020ladv}
& 
&4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&\cite{QlikSense2010}
&
&\cite{datapine2012}\cite{thoughtspot2012}
&
&
&
&
&
&
&\cite{SisenseFusionAnalytics2019}
&
& 
&4 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Glyphs}}}} & \textbf{Design Space} 
&\cite{yost2005single} \cite{ward2008multivariate} \cite{klippel2009colour}
&
&
&
&\cite{borgo2013glyph}
&\cite{fuchs2014influence}
&\cite{albo2015off}
&\cite{fuchs2016systematic}
&
&
&
&
& 
&7  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&\cite{ribarsky1994glyphmaker}
&
&
&
&
&
&
&\cite{tong2016glyphlens}
&
&\cite{ren2018charticulator}
&
&\cite{tsandilas2020structgraphics} 
& \cite{brehmer2021generative}
& 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&
&
&\cite{zhao2020iconate}
& 
& 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&
&
& \cite{ying2021glyphcreator}
&1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Infographic}}}} & \textbf{Design Space} 
&\cite{artacho2008influence}
&
&
&
&
&\cite{albers2014infographics}
&\cite{harrison2015infographic} 
&\cite{dunlap2016getting}\cite{lyra2016infographics}
&
&\cite{santos2018influence}
&
&
& \cite{lan2021smile}
& 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&\cite{lee2013sketchstory}
&
&
&\cite{kim2016data}
&
&\cite{wang2018infonice}\cite{xia2018dataink}
&\cite{kim2019dataselfie}
&\cite{zhang2020dataquilt} \cite{coelho2020infomages}
&\cite{cui2021mixed}
& 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&\cite{infogram2012}
&\cite{visme2013}
&
&
&
&
&
&\cite{chen2019towards}
&\cite{lu2020exploring}
& \cite{tyagi2021user}\cite{yuan2021infocolorizer}
& 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&\cite{CANVA2018}
&\cite{cui2019text}
&\cite{qian2020retrieve}
& 
&3 \\ \hline
  
\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Timeline}}}} & \textbf{Design Space} 
&
&
&
&\cite{tanahashi2012design}
&
&
&\cite{bach2015time}
&\cite{brehmer2016timelines}\cite{gronemann2016crossing}
&
&
&
&\cite{di2020storyline}
& \cite{lan2021understanding}
& 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&\cite{dukes2010dipity}
&\cite{webalon2011tiki}\cite{TimelineSetter2011}
&\cite{llc2012timeglider}
&\cite{TimelineJS2013}
&
&
&
&\cite{kim2017visualizing}
&
&\cite{brehmer2019timeline}
&
& 
&7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&\cite{liu2013storyflow}
&\cite{satyanarayan2014authoring}
&\cite{fulda2015timelinecurator}
&\cite{nguyen2016timesets}
&
&\cite{tang2018istoryline}
&
&\cite{tang2020plotthread} 
& 
& 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&
&
& 
& \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Annotated\\  Chart\end{tabular}}}}} & \textbf{Design Space} 
&
&
&
&
&\cite{borkin2013makes}
&
&\cite{borkin2015beyond}
&
&\cite{kong2017internal}
&
&
&
& 
&3  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&
&\cite{ren2017chartaccent}
&
&
&
& 
&1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&\cite{chen2010click2annotate} \cite{chen2010touch2annotate} 
&
&\cite{kandogan2012just}
&
&
&
&\cite{bryan2016temporal}
&
&
&
&
&\cite{latif2021kori}
&5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&\cite{hullman2013contextifier} 
&
&
&
&\cite{bylinskii2017understanding} 
&
&
&\cite{liu2020autocaption}
& 
&3 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\  Comics\end{tabular}}}}} & \textbf{Design Space} 
&
&
&
&
&
&
&\cite{zhao2015data} 
&
&\cite{bach2017emerging}
&\cite{bach2018design}
& \cite{zhao2019understanding}\cite{wang2019comparing} \cite{wang2019teaching}
&\cite{wang2020data}
& 
& 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&
&
&
&\cite{kim2019datatoon}
&
& \cite{wang2021interactive}  \cite{kang2021toonnote}
&3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&
&
&
& \cite{zhao2021chartstory}
&1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&\cite{wang2019datashot}
&\cite{shi2020calliope}
& 
&2 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Videos\end{tabular}}}}} & \textbf{Design Space} 
&
&
&
&
&
&
&\cite{amini2015understanding}
&\cite{wang2016animated} 
&
&
&
&\cite{li2020improving}\cite{cao2020examining}\cite{tang2020design} \cite{thompson2020understanding} \cite{shu2020makes}
& \cite{shi2021communicating}\cite{lan2021kineticharts} 
& 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&\cite{amini2016authoring}
&
&
&
&
& 
& 1\\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&\cite{liu2018data} 
&
&
& \cite{thompson2021data}\cite{wang2021animated}
&3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&
&
& \cite{shi2021autoclips}
&1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Scorllytelling}}}} & \textbf{Design Space} 
&
&    
&
&
&\cite{hullman2013deeper}
&
&
&
&
&\cite{seyser2018scrollytelling}\cite{elias2018towards}
&
&
& \cite{roth2021cartographic}
& 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool}
&
&
&
&
&
&
&
&
&
&\cite{conlen2018idyll} 
&
&
& \cite{bocklandt2021sandslide} \cite{sultanum2021leveraging}
& 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported}
&
&
&
&
&
&
&
&
&
&
&\cite{winters2019automatically}
&
& 
&1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator}
&
&
&
&
&
&
&
&
&
&
&
&
& \cite{lu2021automatic}
& 1 \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\end{tabular}
\end{table*}

==> Table/backup/table3-0401.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{1.5}
\begin{table*}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Statistical \\ Charts\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  &  & 1 &  & 1 &  & 1 & 1 & 2 &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  & 1 &  & 1 & 1 &  &  & 1 & 1 & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  & 1 &  & 6 & 2 & 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  & 2 & 1 &  & 1 & 2 & 2 & 1 & 9 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Other \\ Charts\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Dashboard}}}}
& \textbf{Design Space} &  &  &  & 1 &  &  &  & 1 & 1 & 1 & 1 & 1 &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 3 &  & 1 & 1 &  &  &  &  &  &  &  &  &  & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  & 1 &  &  & 2 &  &  & 2 &  & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  & 1 &  & 2 &  &  &  &  &  &  & 1 &  &  & 4 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Glyphs}}}}
& \textbf{Design Space} & 3 &  &  &  & 1 & 1 & 1 & 1 & \multicolumn{1}{l|}{} &  &  &  &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 1 &  &  &  &  &  &  & 1 &  & 1 &  & 1 & 1 & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  &  & 1 &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Infographic}}}}
& \textbf{Design Space} & 1 &  &  &  &  & 1 & 1 & 2 &  & 1 &  &  & 1 & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  & 1 &  &  & 1 &  & 2 & 1 & 2 & 1 & 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  & 1 & 1 &  &  &  &  &  & 1 & 1 & 2 & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  & 1 & 1 & 1 &  & 3 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Timeline}}}}
& \textbf{Design Space} &  &  &  & 1 &  &  & 1 & 2 &  &  &  & 1 & 1 & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  & 1 & 2 & 1 & 1 &  &  &  & 1 &  & 1 &  &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  & 1 & 1 & 1 & 1 &  & 1 &  & 1 &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Annotated\\  Chart\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  & 1 &  & 1 &  & 1 &  &  &  &  & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  & 1 &  &  &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  & 2 &  & 1 &  &  &  & 1 &  &  &  &  & 1 & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  & 1 &  &  &  & 1 &  &  & 1 &  & 3 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\  Comics\end{tabular}}}}}

& \textbf{Design Space} &  &  &  &  &  &  & 1 &  & 1 & 1 & 3 & 1 &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  &  & 1 &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  & 1 & 1 &  & 2 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Videos\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  &  &  & 1 & 1 &  &  &  & 5 & 2 & 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  & 1 &  &  &  &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  & 1 &  &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Scorllytelling}}}}
& \textbf{Design Space} &  &  &  &  & 1 &  &  &  &  & 2 &  &  & 1 & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  & 1 &  &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  & 1 &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}} & 8 & 4 & 3 & 8 & 8 & 6 & 9 & 15 & 9 & 15 & 15 & 30 & 24 & 154 \\ \hline

\end{tabular}
\end{table*}

==> Table/backup/table3.tex <==
\begin{table*}[]
\textbf{\caption{Narrative Visualization Genre Development Timeline}}
\begin{tabular}{|cc|c|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{Chart}} & Design Space & 2 & 1 &  & 1 & 1 &  & 3 & 1 & 2 & 1 & 2 & 2 & 1 & 17 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool & 6 & 1 & 2 & 1 & 1 & 3 & 1 &  & 1 & 3 & 1 & 5 & 4 & 29 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai-Supported & 1 &  &  &  & 1 & 2 &  & 4 & 1 & 3 &  &1  & 1 & 14 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  & 2 & 1 &  & 2 & 2 & 2 &  &  & 9 \\ \hline

\multicolumn{1}{|c|}{\multirow{Infographics}} & Design Space &  &  &  &  &  &  & 1 &  & 1 &  & 1 &  & 1 & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  & 1 &  & 2 &  & 2 & 3 & 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  & 1 & 1 &  &  &  &  &  &  &  &  & 2 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  & 1 & 1 &  &  & 2 \\ \hline

\multicolumn{1}{|c|}{\multirow{Data comic}} & Design Space &  &  &  &  &  &  & 1 &  & 1 & 1 & 3 & 1 &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  &  & 1 &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  & 1 & 1 &  & 2 \\ \hline

\multicolumn{1}{|c|}{\multirow{Data video}} & Design Space &  &  &  &  &  &  & 1 &  &  &  &  & 5 & 2 & 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  & 2 &  &  &  &  & 1 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{Dashboard}} & Design Space & 1 &  &  &1  &  &  &  & 2 & 1 & 2 & 2 & 1 &  & 10 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool & 1 &  & 1 &  &  &  &  &  &  &  & 1 & 1 &  & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator & 1 & 1 &  & 2 &  &  &  &  &  &  & 1 &  &  & 5 \\ \hline

\multicolumn{1}{|c|}{\multirow{Scrollytelling}} & Design Space &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  & 1 &  & & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &1  &  & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{Glyph}} & Design Space & 1 &  & 1 & 1 & 1 & 2 &  & 1 &  &  &  &  &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  & 1 &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{Immersive}} & Design Space &  &  &  &  &  &  &  &  &  & 1 &  & 1 & 1 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  & 1 & 1 &  &  & 2 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Ai Supported &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 \\ \hline
\multicolumn{2}{|c|}{SUM} & 13 & 3 & 4 & 6 & 5 & 9 & 8 & 11 & 9 & 17 & 17 & 22 & 25 & 149 \\ \hline
\end{tabular}
\end{table*}








==> Table/backup/table4-edit.tex <==
%[Table2:与年份对应的表格]
 \begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
 \begin{tabular}{|c|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|}
 \hline
 \textbf{}  & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

%上面不要动

%下面是chart
\textbf{Chart}     
&\cite{kosslyn1989understanding} \cite{ahlberg1996spotfire} \cite{stolte2002polaris} \cite{fekete2004infovis} \cite{spence2005no} \cite{heer2005prefuse} \cite{abello2006ask} \cite{henry2007nodetrix}  \cite{bostock2009protovis}
&\cite{grammel2010information} \cite{cui2010context}
& \cite{oesper2011wordcloud} \cite{bostock2011d3} % \cite{TimelineJS} 
&\cite{kong2012graphical} 
& \cite{borkin2013makes}   \cite{hullman2013contextifier} \cite{dunne2013motif} %\cite{TimelineSetter} 
&\cite{ren2014ivisdesigner} \cite{ren2014weiboevents}\cite{satyanarayan2014lyra} \cite{heimerl2014word} \cite{cheng2014synonym} \cite{satyanarayan2014authoring} \cite{gao2014newsviews}
&\cite{wongsuphasawat2015voyager} \cite{bach2015time}  \cite{fulda2015timelinecurator} \cite{borkin2015beyond} \cite{albo2015off}
&\cite{felix2016texttile} \cite{satyanarayan2016vega} \cite{brehmer2016timelines} \cite{nguyen2016timesets} \cite{xu2016semantic}
&\cite{mauri2017rawgraphs} \cite{kim2017visualizing} \cite{felix2017taking} \cite{wang2017edwordle} \cite{jin2017development} \cite{ren2017chartaccent}
& \cite{liu2018data} \cite{sarvghad2018embedded}  \cite{srinivasan2018augmenting} \cite{ren2018charticulator} \cite{luo2018deepeye}  \cite{brath2018automated} \cite{hoelscher2018using} \cite{tang2018istoryline} \cite{moritz2018formalizing}
&\cite{luo2019enhancing} \cite{dibia2019data2vis} \cite{hu2019vizml} \cite{chen2019towards}  \cite{hearst2019evaluation}
&\cite{wang2020cheat} \cite{lyi2020comparative}  \cite{fu2020chartem} \cite{zong2020lyra} \cite{liu2020autocaption} \cite{hopkins2020visualint} \cite{tsandilas2020structgraphics} \cite{tang2020plotthread}
&\cite{cui2021mixed} \cite{ge2021cast} \cite{lan2021understanding} \cite{shu2021dancingwords}\cite{latif2021kori} \cite{roth2021cartographic}
& 68\\ \hline 

%-----------------------
%infographics
%-----------------------


%下面是Infographics
\textbf{Infographics} 
&
&
&  
& \cite{infogram2012}
&  \cite{visme2013}
&
& \cite{otten2015infographics}
& \cite{kim2016data}
& \cite{hearst2017teaching} 
& \cite{xia2018dataink} \cite{wang2018infonice} \cite{CANVA2018}
& \cite{lalle2019gaze} \cite{cui2019text}
& \cite{coelho2020infomages}  \cite{lu2020exploring}
& \cite{lan2021smile} \cite{yuan2021infocolorizer} \cite{wang2021animated}  \cite{tyagi2021user}
&  16        \\ \hline


%-----------------------
%data comics
%-----------------------

\textbf{Data Comics}
&
&
&
&
&
&
& \cite{zhao2015data}
&
& \cite{bach2017emerging}
& \cite{bach2018design}
& \cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding} \cite{wang2019datashot} \cite{kim2019datatoon}
& \cite{wang2020data} \cite{shi2020calliope}
& \cite{wang2021interactive}  \cite{kang2021toonnote} \cite{zhao2021chartstory}
&  13         \\ \hline

%-----------------------
%data videos
%-----------------------

\textbf{Data Videos}&
& 
& 
& 
& 
&
& \cite{amini2015understanding}
&  \cite{wang2016animated} \cite{amini2016authoring}
&
& 
&
& \cite{thompson2020understanding} \cite{li2020improving} \cite{shu2020makes} \cite{tang2020design} \cite{cao2020examining}  
& \cite{shi2021communicating} \cite{lan2021kineticharts} \cite{chen2021augmenting}  \cite{thompson2021data}  \cite{shi2021autoclips}
&  13   \\ \hline

%-----------------------
% dashboard
%-----------------------


\textbf{Dashboard}
& \cite{few2007dashboard}   \cite{bajzek2007inventing} \cite{IBMCognosAnalytics}%cogno公司在2008年被IBM公司收购，后续版本迭代中增加了AI功能，但是不确实具体合适增加的AI
& \cite{QlikSense2010}
&\cite{elias2011exploration}
&\cite{elias2012annotating}  \cite{datapine2012} \cite{thoughtspot2012}%这两款工具都是开发于2012年，在后续的版本迭代中逐渐增加了AI功能
& 
&
& 
& \cite{schwendimann2016perceiving} \cite{froese2016lessons}
& \cite{qu2017keeping}
&  \cite{sarikaya2018we} \cite{molenaar2018teachers}
&  \cite{sedrakyan2019guiding} \cite{cha2019applying} \cite{becker2019microsoft} \cite{SisenseFusionAnalytics2019}
&  \cite{chen2020composition}  \cite{ma2020ladv} 
& 
&   19     \\ \hline

%Slideshow
\textbf{Slideshow}
&
&
&
&
&
&
& 
&
& 
& \cite{wang2018narvis}
&
& \cite{leake2020generating}
& \cite{joshi2021learning} \cite{sultanum2021leveraging} \cite{lu2021automatic} 
& 4      \\ \hline

%Glyph
\textbf{Glyph}
&  \cite{roberts2005haptic}
&
& \cite{ropinski2011survey}
& \cite{maguire2012taxonomy} 
& \cite{borgo2013glyph}
& \cite{fuchs2014influence} \cite{chung2014glyph}
&
&\cite{fuchs2016systematic} 
&
&
& 
& \cite{zhao2020iconate}
&  \cite{brehmer2021generative} \cite{ying2021glyphcreator}
&  10      \\ \hline

%Immersive
\textbf{Immersive}
&
&
&
&
&
&
&
&
& 
& \cite{isenberg2018immersive} \cite{sicat2018dxr}
&\cite{chen2019marvist}
& \cite{zikas2020immersive} 
& \cite{kraus2021value} \cite{dang2021gesturemap}
&   6     \\ \hline

\textbf{SUM}
&13 &3 &4 &6 &5 &9 &8 &11 &10 &17 &17 &22 &25 &149       \\ \hline
 \end{tabular}
 \end{table*}


==> Table/backup/table4.tex <==
%[Table2:与年份对应的表格]
 \begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
 \begin{tabular}{|c|m{0.7cm}<{\centering}|c|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|m{0.7cm}<{\centering}|}
 \hline
 \textbf{}  & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline
%上面不要动

%下面是chart
\textbf{Chart}     
& \cite{spence2005no} \cite{kosslyn1989understanding}\cite{heer2007voyagers}\cite{fekete2004infovis}\cite{stolte2002polaris}\cite{bostock2009protovis}\cite{heer2005prefuse}\cite{mackinlay2007show}\cite{ahlberg1996spotfire}\cite{abello2006ask}\cite{bastian2009gephi} \cite{henry2007nodetrix}
%\cite{bavoil2005vistrails} \cite{bazeley2002evolution} 
& \cite{grammel2010information} \cite{cui2010context} 
& \cite{oesper2011wordcloud} \cite{bostock2011d3} %\cite{TimelineSetter2011} \cite{smoot2011cytoscape}
& \cite{kong2012graphical}\cite{kandel2012profiler} \cite{kolman2012infomaps} %\cite{nadhani2012fusioncharts}
& \cite{gratzl2013lineup}\cite{borkin2013evaluation} \cite{borkin2013makes} %\cite{TimelineJS2013} \cite{murphy2013data} \cite{morisette2013vistrails} \cite{hullman2013contextifier}
& \cite{ren2014ivisdesigner} \cite{heimerl2014word} \cite{satyanarayan2014authoring} \cite{ren2014weiboevents} \cite{satyanarayan2014lyra}\cite{gao2014newsviews}
& \cite{bach2015time} \cite{wongsuphasawat2015voyager} \cite{fulda2015timelinecurator}\cite{felix2015revex}\cite{vartak2015seedb} \cite{borkin2015beyond}
& \cite{brehmer2016timelines}\cite{felix2016texttile}\cite{saket2016visualization}\cite{satyanarayan2016vega}\cite{nguyen2016timesets} %\cite{bigelow2016iterating}
&\cite{kim2017visualizing}   \cite{felix2017taking}  \cite{wang2017edwordle}\cite{harrison2017petminer}\cite{mauri2017rawgraphs}\cite{jin2017development} \cite{ren2017chartaccent} %\cite{caldarola2017big}
& \cite{ren2018charticulator}  \cite{liu2018data}  \cite{sarvghad2018embedded} \cite{hoelscher2018using}\cite{coene2018sigmajs}\cite{luo2018deepeye}\cite{srinivasan2018augmenting} \cite{brath2018automated} % \cite{li2018bdviewer}
& \cite{luo2019enhancing}  \cite{chen2019towards}\cite{dibia2019data2vis}
& \cite{wang2020cheat} \cite{lyi2020comparative} \cite{zong2020lyra} \cite{fu2020chartem} \cite{tsandilas2020structgraphics} \cite{ge2020canis} \cite{liu2020autocaption} \cite{hopkins2020visualint}  % \cite{sievert2020interactive}
& \cite{lan2021understanding} \cite{roth2021cartographic}  \cite{cui2021mixed} \cite{shu2021dancingwords}  \cite{eirich2021irvine}    \cite{latif2021kori}
&71 \\ \hline

%-----------------------

%-----------------------


%下面是Infographics
\textbf{Infographics} 
&
&
&  
&
& 
&
& \cite{otten2015infographics}
& \cite{kim2016data}
& \cite{hearst2017teaching}
& \cite{wang2018infonice}  \cite{xia2018dataink}
& \cite{cui2019text} \cite{lalle2019gaze}
& \cite{coelho2020infomages}  \cite{lu2020exploring}
&\cite{yuan2021infocolorizer} \cite{lan2021smile} \cite{tyagi2021user}
&  12         \\ \hline


\textbf{Data Comics}
&
&
&
&
&
&
&\cite{tobita2015comic}
&
&
& \cite{bach2018design}
& \cite{wang2019teaching} \cite{wang2019comparing} \cite{zhao2019understanding} \cite{wang2019datashot}\cite{kim2019datatoon}
& \cite{wang2020data} \cite{shi2020calliope}
&\cite{wang2021interactive} \cite{zhao2021chartstory} \cite{kang2021toonnote}
&   12        \\ \hline


\textbf{Data Videos}&
& 
& 
& 
& 
&
& \cite{amini2015understanding}
&\cite{wang2016animated} \cite{amini2016authoring}
&
& 
&
& \cite{thompson2020understanding}  \cite{li2020improving}  \cite{shu2020makes} \cite{tang2020design}  \cite{cao2020examining} 
&\cite{shi2021communicating}  \cite{lan2021kineticharts} \cite{shi2021autoclips} \cite{chen2021augmenting}  \cite{wang2021animated}\cite{thompson2021data}
&   14        \\ \hline



%dashboard
\textbf{Dashboard}
& \cite{few2007dashboard}  \cite{bajzek2007inventing}
&
& \cite{elias2011exploration}
& \cite{nadhani2012fusioncharts} \cite{elias2012annotating}
& \cite{hullman2013contextifier}
& %\cite{bhardwaj2014datahub}%这一篇多了
& \cite{loorak2015timespan} \cite{ai2015neuroblocks}
& \cite{schwendimann2016perceiving}  \cite{froese2016lessons}
& \cite{qu2017keeping}  \cite{siddiqui2017fast}
& \cite{sarikaya2018we}  \cite{molenaar2018teachers}
& \cite{sedrakyan2019guiding}  \cite{cha2019applying} \cite{becker2019microsoft} %\cite{lousa2019evaluation}\cite{munz2019visme} 
& \cite{chen2020composition} \cite{ma2020ladv}
& 
&  19       \\ \hline





%Slideshow
\textbf{Slideshow}
&\cite{hinrichs2008emdialog}
&
&
&
&
&
& 
&
& 
&\cite{wang2018narvis}
&
&\cite{tang2020plotthread}
& \cite{lu2021automatic} \cite{sultanum2021leveraging} \cite{joshilearning} %\cite{Flourish}
& 6        \\ \hline

%Glyph
\textbf{Glyph}
& \cite{roberts2005haptic} 
& \cite{sanyal2010noodles} 
& \cite{ropinski2011survey} 
& \cite{maguire2012taxonomy}
& \cite{borgo2013glyph} \cite{dunne2013motif}
& \cite{fuchs2014influence} \cite{chung2014glyph}
&   \cite{albo2015off} 
& \cite{fuchs2016systematic} 
&
&\cite{chevalier2018using}
& 
& \cite{zhao2020iconate}
& \cite{brehmer2021generative}
&    13       \\ \hline

%Immersive
\textbf{Immersive}
&
&
&
&
& \cite{spaulding2013design}
& \cite{palmas2014movexp}
&
&
& \cite{chen2017exploring}
& \cite{sicat2018dxr} \cite{isenberg2018immersive}
& \cite{chen2019marvist}
&\cite{nebeling2020mrat}
&\cite{dang2021gesturemap}\cite{jing2021eyemr}\cite{kraus2021value}
&   10        \\ \hline

\textbf{SUM}
&15 &4 &4 &6 &7 &9 &12 &10 &11 &17 &14 &22 &25 & 157       \\ \hline
 \end{tabular}
 \end{table*}


==> Table/backup/table5-edit.tex <==
%%%%%
% Please add the following required packages to your document preamble:

\renewcommand\arraystretch{0.5}
\begin{table*}[]
\begin{tabular}{|cc|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \multicolumn{1}{c|} {\textbf{SUM}} \\ \hline

% chart的内容

%下面不能动

\multicolumn{1}{|c|}{\multirow {\textbf{Chart}}}
& Design Space 
& \cite{spence2005no}\cite{kosslyn1989understanding}   &\cite{grammel2010information}  &  &   &\cite{borkin2013makes}  &  &\cite{bach2015time}  \cite{borkin2015beyond}\cite{albo2015off} &\cite{brehmer2016timelines}  &  \cite{kim2017visualizing}\cite{felix2017taking} &\cite{brath2018automated}  &\cite{luo2019enhancing}  \cite{hearst2019evaluation} &\cite{wang2020cheat}\cite{lyi2020comparative}  &\cite{lan2021understanding}   &   \\ \cline{2-16} 
 
\multicolumn{1}{|c|}{} & Authoring Tool  
&\cite{ahlberg1996spotfire} \cite{stolte2002polaris} \cite{heer2005prefuse}\cite{fekete2004infovis} \cite{bostock2009protovis}\cite{henry2007nodetrix} &\cite{cui2010context}    &  \cite{oesper2011wordcloud} \cite{bostock2011d3} &\cite{kong2012graphical}  &\cite{dunne2013motif}  &\cite{ren2014ivisdesigner} \cite{heimerl2014word} \cite{satyanarayan2014authoring} &\cite{fulda2015timelinecurator}  &  & \cite{ren2017chartaccent}  &\cite{liu2018data}\cite{sarvghad2018embedded}\cite{hoelscher2018using}  & \cite{chen2019towards} &\cite{fu2020chartem}\cite{zong2020lyra}\cite{liu2020autocaption} \cite{hopkins2020visualint} \cite{tsandilas2020structgraphics} &\cite{cui2021mixed} \cite{shu2021dancingwords} \cite{latif2021kori} \cite{roth2021cartographic}&   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools 
& \cite{abello2006ask} &  &  &  & \cite{hullman2013contextifier} &\cite{ren2014weiboevents}\cite{satyanarayan2014lyra}   &  &\cite{felix2016texttile} \cite{satyanarayan2016vega} \cite{nguyen2016timesets} \cite{xu2016semantic} &\cite{mauri2017rawgraphs}  &\cite{srinivasan2018augmenting}  \cite{ren2018charticulator} \cite{tang2018istoryline} &  &\cite{tang2020plotthread}  &\cite{ge2021cast}  &  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator 
&  &  &  &  &  &\cite{cheng2014synonym}\cite{gao2014newsviews}   &\cite{wongsuphasawat2015voyager}  &  &\cite{jin2017development} \cite{wang2017edwordle} &\cite{luo2018deepeye} \cite{moritz2018formalizing}  &\cite{dibia2019data2vis} \cite{hu2019vizml}  &  &  &  \\ \hline


%Infographics的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Infographics}}} & Design Space &  &  &  &  &  &   &\cite{otten2015infographics}  &  &\cite{hearst2017teaching}  &  & \cite{lalle2019gaze}  &  &\cite{lan2021smile}  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool&  &  &  &  &  &   &  &\cite{kim2016data}  &  & \cite{xia2018dataink}\cite{wang2018infonice} &  & \cite{coelho2020infomages}\cite{lu2020exploring}  &\cite{yuan2021infocolorizer}\cite{wang2021animated} \cite{tyagi2021user}   &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  & \cite{infogram2012}  &\cite{visme2013}  &   &  &  &  &  &  &  &  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &   &  &  &  &\cite{CANVA2018}  &\cite{cui2019text}  &  &  &  \\ \hline

%data comic的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Data comic}}} 
& Design Space &  &  &  &  &  &   & \cite{zhao2015data} &  &\cite{bach2017emerging}  &\cite{bach2018design}  &\cite{wang2019teaching} \cite{wang2019comparing} \cite{zhao2019understanding}   &\cite{wang2020data}  &  &    \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &   &  &  &  &  & \cite{kim2019datatoon}  &  & \cite{wang2021interactive}\cite{kang2021toonnote}  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &   &  &  &  &  &  &  & \cite{zhao2021chartstory} &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &   &  &  &  &  & \cite{wang2019datashot} &\cite{shi2020calliope}  &  &   \\ \hline

%data video的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Data video}}} 
& Design Space &  &  &  &  &  &   & \cite{amini2015understanding}  &  &  &  &  &\cite{thompson2020understanding}  \cite{li2020improving} \cite{shu2020makes} \cite{tang2020design} \cite{cao2020examining}   &\cite{shi2021communicating}\cite{lan2021kineticharts}  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &   &  &\cite{wang2016animated} \cite{amini2016authoring}   &  &  &  &  &\cite{chen2021augmenting}   &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &   &  &  &  &  &  &  & \cite{thompson2021data} &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator&  &  &  &  &  &   &  &  &  &  &  &  &\cite{shi2021autoclips}  &  \\ \hline



%Dashboard的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Dashboard}}}
& Design Space &\cite{few2007dashboard}  &  &  &\cite{elias2012annotating}  &  &   &  &\cite{schwendimann2016perceiving} \cite{froese2016lessons}  &\cite{qu2017keeping}  &  \cite{sarikaya2018we}\cite{molenaar2018teachers} & \cite{sedrakyan2019guiding}  \cite{cha2019applying}  & \cite{chen2020composition} &  &   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & Authoring Tool &\cite{bajzek2007inventing}   &  & \cite{elias2011exploration} &  &  &   &  &  &  &  & \cite{becker2019microsoft} &\cite{ma2020ladv}  &  &  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools&  &  &  &  &  &   &  &  &  &  &  &  &  &   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator &\cite{IBMCognosAnalytics}  & \cite{QlikSense2010} &  &\cite{datapine2012} \cite{thoughtspot2012} &  &   &  &  &  &  &\cite{SisenseFusionAnalytics2019}  &  &  &  \\ \hline


%Slideshow的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Slideshow}}}
& Design Space &  &  &  &  &  &   &  &  &  &  &  &  &\cite{joshi2021learning}  &  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  & &   &  &  &  &\cite{wang2018narvis}  &  &  &\cite{sultanum2021leveraging} \cite{lu2021automatic}   &  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &   &  &  &  &  &  &  &  &   \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &   &  &  &  &  &  & \cite{leake2020generating} &  &  \\ \hline

%Glyph的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Glyph}}} 
& Design Space &\cite{roberts2005haptic}  &  &\cite{ropinski2011survey}   &\cite{maguire2012taxonomy}  &\cite{borgo2013glyph}  &\cite{fuchs2014influence} \cite{chung2014glyph}     &  &  \cite{fuchs2016systematic}  &  &  &  &  &  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &   &  &  &  &  &  &  & \cite{brehmer2021generative}  &  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &   &  &  &  &  &  &\cite{zhao2020iconate}  &  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &  &\cite{ying2021glyphcreator}  &  \\ \hline


%Immersive的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Immersive}}} 
& Design Space &  &  &  &  &  &   &  &  &  & \cite{isenberg2018immersive} &  &\cite{zikas2020immersive}  &\cite{kraus2021value}  &    \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &   &  &  &  &\cite{sicat2018dxr}  &\cite{chen2019marvist}  &  &  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &   &  &  &  &  &  &  &\cite{dang2021gesturemap}  &   \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &   &  &  &  &  &  &  &  &   \\ \hline


\multicolumn{2}{|c|}{\textbf{SUM}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

\end{tabular}
\end{table*}

==> Table/backup/table5.tex <==
%%%%%
% Please add the following required packages to your document preamble:

\renewcommand\arraystretch{0.8}
\begin{table*}[]
\begin{tabular}{|cc|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|m{0.5cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \multicolumn{1}{c|} {\textbf{SUM}} \\ \hline

% chart的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Chart}}}
& Design Space &\cite{kosslyn1989understanding} \cite{spence2005no}   &\cite{grammel2010information}  &  &  &\cite{borkin2013makes}  &  &\cite{bach2015time} \cite{borkin2015beyond} &\cite{brehmer2016timelines}  & \cite{kim2017visualizing} \cite{felix2017taking}   & \cite{brath2018automated}  &\cite{luo2019enhancing}  &\cite{wang2020cheat} \cite{lyi2020comparative}  &\cite{lan2021understanding}\cite{roth2021cartographic}  &15  \\ \cline{2-16} 
 
\multicolumn{1}{|c|}{} & Authoring Tool &\cite{ahlberg1996spotfire} \cite{stolte2002polaris} \cite{fekete2004infovis} \cite{heer2005prefuse} \cite{henry2007nodetrix} \cite{bostock2009protovis} &\cite{cui2010context}  & \cite{oesper2011wordcloud} \cite{bostock2011d3} %\cite{TimelineJS}
&\cite{kong2012graphical}  & %\cite{TimelineSetter}  
& \cite{heimerl2014word} \cite{satyanarayan2014authoring}&\cite{fulda2015timelinecurator}  &  &\cite{wang2017edwordle}  \cite{ren2017chartaccent}  &\cite{ren2018charticulator} \cite{liu2018data} \cite{sarvghad2018embedded}  \cite{hoelscher2018using} &\cite{chen2019towards} &\cite{ge2020canis} \cite{fu2020chartem} \cite{zong2020lyra}   \cite{tsandilas2020structgraphics} \cite{liu2020autocaption} \cite{hopkins2020visualint} &\cite{cui2021mixed}\cite{shu2021dancingwords} \cite{latif2021kori}  & 29  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools &\cite{bastian2009gephi}  &  &  &%\cite{TouchGraph}  
&  &\cite{ren2014weiboevents} \cite{ren2014ivisdesigner}\cite{satyanarayan2014lyra} &\cite{vartak2015seedb} \cite{felix2015revex} &\cite{saket2016visualization} \cite{felix2016texttile}\cite{satyanarayan2016vega} &\cite{harrison2017petminer} \cite{mauri2017rawgraphs} \cite{jin2017development} &\cite{coene2018sigmajs} \cite{srinivasan2018augmenting} &  &  &\cite{eirich2021irvine}  &16  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator &\cite{abello2006ask} \cite{heer2007voyagers} \cite{mackinlay2007show} &  &  & \cite{kandel2012profiler} \cite{kolman2012infomaps} &  \cite{borkin2013evaluation} \cite{hullman2013contextifier} &\cite{gao2014newsviews}  &\cite{wongsuphasawat2015voyager}  &\cite{nguyen2016timesets}  &  &\cite{luo2018deepeye}  &\cite{dibia2019data2vis}  &  &  & 13 \\ \hline


%Infographics的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Infographics}}} & Design Space &  &  &  &  &  &  &\cite{otten2015infographics}  &  &\cite{hearst2017teaching}  &  &\cite{lalle2019gaze}  &  &\cite{lan2021smile}  & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &\cite{kim2016data}  &  &\cite{xia2018dataink}  &  &\cite{coelho2020infomages}\cite{lu2020exploring}  &\cite{yuan2021infocolorizer} \cite{tyagi2021user} &6  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &  &  &  &\cite{wang2018infonice}  &  &  &  &1  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &\cite{cui2019text}  &  &  &1  \\ \hline


%data comic的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Data comic}}} 
& Design Space &  &  &  &  &  &  &  &  &  &\cite{bach2018design}  & \cite{wang2019teaching}\cite{wang2019comparing} \cite{zhao2019understanding} &\cite{wang2020data}  &  &5  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  &  &\cite{wang2019datashot}  &  & \cite{wang2021interactive}  \cite{kang2021toonnote}  & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &  &  &  &  &\cite{kim2019datatoon}  &  &\cite{zhao2021chartstory}  & 2 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &\cite{tobita2015comic}  &  &  &  &  &\cite{shi2020calliope}  &  & 2 \\ \hline


%data video的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Data video}}} 
& Design Space &  &  &  &  &  &  &\cite{amini2015understanding}  &  &  &  &  &\cite{thompson2020understanding}  \cite{li2020improving} \cite{shu2020makes} \cite{tang2020design} &\cite{shi2021communicating} \cite{lan2021kineticharts}  &7  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &\cite{wang2016animated} \cite{amini2016authoring}  &  &  &  &\cite{cao2020examining}  & \cite{chen2021augmenting}  \cite{wang2021animated} & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &  &  &  &  &  &  &\cite{thompson2021data}  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  & \cite{shi2021autoclips}   &  & 1 \\ \hline



%Dashboard的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Dashboard}}}
& Design Space &\cite{few2007dashboard}   &  &  &\cite{elias2012annotating}  &  &  &  &\cite{schwendimann2016perceiving} \cite{froese2016lessons}   &\cite{qu2017keeping}  &\cite{sarikaya2018we} \cite{molenaar2018teachers} &\cite{sedrakyan2019guiding} \cite{cha2019applying} & \cite{chen2020composition} &  &10  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & Authoring Tool &\cite{bajzek2007inventing}  &  & \cite{elias2011exploration} &  &  &  &  &  &  &  &  & \cite{ma2020ladv}  &    &3  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &\cite{loorak2015timespan}  &  &  &  &\cite{becker2019microsoft}  &  &  &2  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator &  &  &  &\cite{nadhani2012fusioncharts} &\cite{hullman2013contextifier}  &  &\cite{ai2015neuroblocks}  &  &\cite{siddiqui2017fast}  &  &  &  &  & 3 \\ \hline


%Slideshow的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Slideshow}}}
& Design Space &  &  &  &  &  &  &  &  &  &  &  &  &\cite{joshilearning}  & 1 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  &\cite{wang2018narvis}  &  &  
&\cite{sultanum2021leveraging}  & 2 \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &  &  &  &  &  
&\cite{tang2020plotthread}  &\cite{lu2021automatic}  &2  \\ \cline{2-16} 

\multicolumn{1}{|c|}{} & AI Generator &\cite{hinrichs2008emdialog}  &  &  &  &  &  &  &  &  &  &  &  &  &1  \\ \hline



%Glyph的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Glyph}}} 
& Design Space &\cite{roberts2005haptic}  &  & \cite{ropinski2011survey} & \cite{maguire2012taxonomy}  &\cite{borgo2013glyph}  &\cite{fuchs2014influence} \cite{chung2014glyph} &\cite{albo2015off}  & \cite{fuchs2016systematic} &  &  &  &  &  & 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &\cite{dunne2013motif}  &  &  &  &  &  &  &  &\cite{brehmer2021generative}  & 2 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &\cite{sanyal2010noodles}  &  &  &  &  &  &  &  &\cite{chevalier2018using}  &  &\cite{zhao2020iconate}  &  & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

%Immersive的内容
\multicolumn{1}{|c|}{\multirow {\textbf{Immersive}}} 
& Design Space &  &  &  &  &\cite{spaulding2013design}  &  &  &  &\cite{chen2017exploring}  &\cite{isenberg2018immersive}  &  &  &\cite{kraus2021value}  &4  \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & Authoring Tool &  &  &  &  &  &  &  &  &  &  &\cite{chen2019marvist}   &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI-Supported Tools &  &  &  &  &  &  &  &  &  &\cite{sicat2018dxr}  &  &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & AI Generator &  &  &  &  &  &\cite{palmas2014movexp}  &  &  &  &  &  &\cite{nebeling2020mrat}  &\cite{dang2021gesturemap} \cite{jing2021eyemr}  & 4 \\ \hline


\multicolumn{2}{|c|}{\textbf{SUM}} &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline

\end{tabular}
\end{table*}

==> Table/table2-0413.tex <==
\renewcommand\arraystretch{1.5}

\begin{table*}[]
\textbf{ \caption{Listed by year of narrative visualization publication}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
 & \multicolumn{1}{c|}{\textbf{Before}} & \multicolumn{1}{c|}{\textbf{2010}} & \multicolumn{1}{c|}{\textbf{2011}} & \multicolumn{1}{c|}{\textbf{2012}} & \multicolumn{1}{c|}{\textbf{2013}} & \multicolumn{1}{c|}{\textbf{2014}} & \multicolumn{1}{c|}{\textbf{2015}} & \multicolumn{1}{c|}{\textbf{2016}} & \multicolumn{1}{c|}{\textbf{2017}} & \multicolumn{1}{c|}{\textbf{2018}} & \multicolumn{1}{c|}{\textbf{2019}} & \multicolumn{1}{c|}{\textbf{2020}} & \multicolumn{1}{c|}{\textbf{2021}} & \multicolumn{1}{c|}{\textbf{SUM}} \\ \hline
\textbf{Dashboard} & 3 & 1 & 1 & 4 &   & 1 &   & 1  & 3 & 1  & 2  & 3  &    & 20  \\ \hline
\textbf{Infographic}& 1 &   &   & 1 & 2 & 1 & 1 & 3  &   & 4  & 3  & 4  & 4  & 24 \\ \hline
\textbf{Timeline}  &   & 1 & 2 & 2 & 2 & 1 & 2 & 3  & 1 & 1  & 1  & 2  & 1  & 19   \\ \hline
\textbf{Annotated chart} &   & 2 &   & 1 & 2 &   & 1 &   & 3 &    &    & 1  & 1  & 12  \\ \hline
\textbf{Data Comics}  &   &   &   &   &   &   & 1 &    & 1 & 1  & 5  & 2  & 3  & 13   \\ \hline
\textbf{Data videos} &   &   &   &   &   &   & 1 & 2  &   & 1  &    & 5  & 5  & 14  \\ \hline
\textbf{Scrollytelling} &   &   &   &   & 1 &   &   &    &   & 3  & 1  &    & 4  & 9  \\ \hline
\textbf{SUM} & 4 & 4 & 3 & 8 & 7 & 3 & 6 & 10 & 7 & 11 & 12 & 17 & 18 & 110\\ \hline
\end{tabular}
\end{table*}

==> Table/table3-0413.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand\arraystretch{1.5}
\begin{table*}
\begin{tabular}{|cc|c|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|m{0.6cm}<{\centering}|c|}
\hline
\multicolumn{2}{|c|}{} & \textbf{Before} & \textbf{2010} & \textbf{2011} & \textbf{2012} & \textbf{2013} & \textbf{2014} & \textbf{2015} & \textbf{2016} & \textbf{2017} & \textbf{2018} & \textbf{2019} & \textbf{2020} & \textbf{2021} & \textbf{SUM} \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Dashboard}}}}
& \textbf{Design Space} &  &  &  & 1 &  &  &  & 1 & 1 & 1 & 1 & 1 &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} & 3 &  & 1 & 1 &  &  &  &  &  &  &  &  &  & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  & 1 &  &  & 2 &  &  & 2 &  & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  & 1 &  & 2 &  &  &  &  &  &  & 1 &  &  & 4 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Infographic}}}}
& \textbf{Design Space} & 1 &  &  &  &  & 1 & 1 & 2 &  & 1 &  &  & 1 & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  & 1 &  &  & 1 &  & 2 & 1 & 2 & 1 & 8 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  & 1 & 1 &  &  &  &  &  & 1 & 1 & 2 & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  & 1 & 1 & 1 &  & 3 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Timeline}}}}
& \textbf{Design Space} &  &  &  & 1 &  &  & 1 & 2 &  &  &  & 1 & 1 & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  & 1 & 2 & 1 & 1 &  &  &  & 1 &  & 1 &  &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  & 1 & 1 & 1 & 1 &  & 1 &  & 1 &  & 6 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  &  & 0 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Annotated\\  Chart\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  & 1 &  & 1 &  & 1 &  &  &  &  & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  & 1 &  &  &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  & 2 &  & 1 &  &  &  & 1 &  &  &  &  & 1 & 5 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  & 1 &  &  &  & 1 &  &  & 1 &  & 3 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\  Comics\end{tabular}}}}}

& \textbf{Design Space} &  &  &  &  &  &  & 1 &  & 1 & 1 & 3 & 1 &  & 7 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  &  & 1 &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  & 1 & 1 &  & 2 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Videos\end{tabular}}}}}
& \textbf{Design Space} &  &  &  &  &  &  & 1 & 1 &  &  &  & 5 & 2 & 9 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  & 1 &  &  &  &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  & 1 &  &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{1}{|c|}{\multirow{4}{*}{\rotatebox{90}{\textbf{Scorllytelling}}}}
& \textbf{Design Space} &  &  &  &  & 1 &  &  &  &  & 2 &  &  & 1 & 4 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{Authoring Tool} &  &  &  &  &  &  &  &  &  & 1 &  &  & 2 & 3 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Supported} &  &  &  &  &  &  &  &  &  &  & 1 &  &  & 1 \\ \cline{2-16} 
\multicolumn{1}{|c|}{} & \textbf{AI Generator} &  &  &  &  &  &  &  &  &  &  &  &  & 1 & 1 \\ \hline

\multicolumn{2}{|c|}{\textbf{SUM}}& 4 & 4 & 3 & 8 & 7 & 3 & 6 & 10 & 8 & 11 & 12 & 17 & 18 & 111 \\ \hline

\end{tabular}
\end{table*}

==> archive-authoringtlool.tex <==
\section{Authoring Tools}
Authoring tools are software applications used to develop e-learning products. Authoring tools reduce the effort involved in writing code or scripts directly in a programming editor, and they often use a "what you see is what you get" ("what you see is what you get") interface, allowing users to easily manipulate and configure their content using intuitive visual icons. Authoring tools reduce the skills required for the authoring process, and in some cases, the average user can use them to author in a short period of time. And most Authoring tools are designed to automate some of the more time-consuming tasks, optimize workflow, and generally provide a more streamlined and efficient approach to the creative process.

\subsection{Universal Visualization Authoring tools}
Authoring tools also play an important role in the field of visualization. Researchers have combined programming techniques to make various improvements to address problems in the visualization field. In this section, we explore authoring tools in the visualization field that not only provide novice visualizers with the opportunity to get started quickly and easily but also save visualizers a lot of time in repetitive tasks and optimize their workflow. Researchers have explored various aspects of the visualization process.\cite{berking2016choosing}

\textbf{[Data Processing Stage - Data Grouping]}
Before practitioners can visualize data, they first need to process the data, group them, collect, simplify and represent the relevant information in a generalized form, which is a routine operational step in data visualization, and although data grouping plays an important role for data exploration, it is not easy to further define the automatically generated grouping criteria. Sarvghad, A. et al (2019) address this type of problem by introducing an Embedded Merge \& Split (EMS) interaction technique that allows direct adjustment of data grouping criteria. This technique allows the user to adjust the data grouping criteria by directly manipulating the codes used to present the groups, thus reducing the amount of time and steps spent on data exploration. The researcher also provides a set of design guidelines to guide how to apply EMS techniques to other visualization types.\cite{sarvghad2018embedded} \textbf{[Pre-visualization]} Even for experts in the visualization field, the selection of graphics is not an easy task in the early stages of visualization creation. To facilitate visualization practitioners to retrieve various visualization design graphics more efficiently, Hoque, E (2020) built the D3 visualization search engine, which can index D3 visualizations based on visual style and infrastructure.\cite{hoque2019searching}

\textbf{[Create visualization]} To facilitate faster and more efficient data visualization design for practitioners and general users, researchers have developed a large number of tools that require no programming and have a graphical user interface for visual creation. Users can embed designed visualizations into existing websites or web-based applications by inserting a piece of Javascript provided by iVisDesigner, and users can Interactively arrange visualization elements using different ways to combine and link different types of visualizations.\cite{ren2014ivisdesigner} It is also possible to perform interactive operations (e.g., clicking buttons, dragging or pressing keys) directly on the visualization that the user is editing in the Lyra2 system. The system also provides a variety of interaction design suggestions that allow the user to quickly implement a variety of visualizations through demonstrated interaction designs.\cite{zong2020lyra}
Secondly, building graphical user interfaces for visual authoring is a challenge, as it is necessary to reconcile the tension between flexible graphical manipulation and the generation of process-visualizations based on graphical syntax or declarative languages. To better support designers' workflows and practices, Liu, Z. et al. (2018) proposed a framework for visual authoring based on inert data coding. The framework uses graphic design concepts (e.g., shapes, locus points, line segments, and groups) to describe components in a visualization. Based on this framework, the researchers designed and developed the Data Illustrator system, which adds inert data binding to vector design tools for visualization authoring. The generated visualization components each have a data range and are considered as peers of each other in the set. Sets use layout to arrange shapes and can be nested to create more complex organizations. When bound to a visual property, the data acts as a constraint and unbound properties can be manipulated freely. These components and operators can describe the structure and generation of various visualizations.\cite{liu2018data}
 
\textbf{[Visual layout]}
In addition, there are also researchers who have explored many aspects of visual layout. Henry, N.et al.(2007) proposed the NodeTrix technique, a hybrid representation of the network, which uses a node link graph to show the global structure of the network and any part of the network that shows the adjacency matrix.\cite{henry2007nodetrix} Dunne, C., \& Shneiderman, B. (2013) proposed the technique of pattern simplification, this technique is mainly designed to improve the problem of complex node-link graphs and taking too much screen space.\cite{dunne2013motif} Tsandilas, T. (2020) proposed StructGraphics, a tool that helps users to explore visual layouts without the constraints of data encoding. With this software, designers can first draw graphs on a canvas and then structure visual attributes to build visual designs without using specific datasets or data architectures.\cite{tsandilas2020structgraphics}

\subsection{Specific Visualization Authoring tools}
In addition to the general Authoring tools for visual design, we can also see that many researchers have been developing and designing a lot of specific Authoring tools for visual design. This chapter investigates different types of Authoring tools according to the visualization design categories mentioned in Chapter 4.

\subsubsection{Chart}
General visualization tools typically require manual specification of views: analysts must choose which transformations and visualization codes to apply based on data variables. These decisions usually involve some domain knowledge as well as visualization design expertise, which is a lengthy specification process that can hinder the exploration of the data. \textbf{[Chart analysis phase]} Wongsuphasawat et al. (2016) developed the voyager system, which will recommend charts based on statistical and perceptual measures of data and perform faceted browsing, as well as integrate with visualization systems to support the exploration of multivariate tabular data. In the early stages of data analysis, Voyager prioritizes data variation (different variable choices and transformations) over design variation (different visual coding of the same data). Helps developers explore breadth-oriented data to discover previously unseen information about the data and increase the variable coverage of the data.\cite{wongsuphasawat2015voyager}
 
\textbf{[Chart Creation Stage]}Ren, D (2017) describes how to help presenters quickly and easily refine their charts with a variety of annotations. A design space for chart annotations is described and using this design space, Chart Accent, an interactive tool that allows one to manually generate data annotations, was developed. This tool provides a new way to define and use data-driven annotations.\cite{ren2017chartaccent} It is very helpful in improving the readability and comprehensibility of charts. And Ren, D (2019) in another study presented the Charticulator tool, a framework that can be used to create a wide range of charts. This is an interactive chart creation tool for specifying custom and reusable chart layouts. Charticulator translates chart specifications into mathematical layout constraints and uses a constraint resolution algorithm to automatically compute a set of layout properties to implement the chart. Thanks to the constraint-based layout approach, it is possible to export chart designs as reusable templates or to import them to other visualization tools for re-editing.\cite{ren2018charticulator}  However, the software has an obvious limitation in that it only supports the repetition of a portion of a chart segment, so the granularity of the data must be predetermined by the chart creator. To address this limitation, the researcher also noted a desire to extend the framework in two ways. First, data transformation channels could be added to the segment level; by specifying a set of data transformations, the chart creator would be able to aggregate the data to the desired granularity. Second, and more importantly, a Glyph could be allowed to be designed as a nested chart. Thus, an important direction for future research is to envision new forms of interactive tutorials to facilitate self-learning for highly definable user interfaces like Charticulator.
 
\textbf{[Comparison of the two tools]}
The most common method of generating visualizations today is to use template-based software to quickly and automatically generate visualizations. However, it has also been suggested that building visualizations with touchable mapping may be a more achievable method for people without visualization expertise. People can quickly implement their own creations without any help when creating visualizations using touchable mapping. Wun, T. (2016) conducted a comparison for both methods and showed that when generating visualizations using Microsoft Excel, participants spent more time exploring the tool. Whereas, when using touchable mapping, participants spent more time on operations directly related to the data, such as visual mapping operations.\cite{wun2016comparing} Therefore, if a novice is just doing some simple visualization creation, he or she can focus more on using touchable mapping, which can lead to faster chart creation groundwork.
 
\textbf{[Chart Animation]}
Diagram animation is an effective means of attracting people's attention and keeping them engaged. Ge, T. et al. (2020) proposed Canis, the first fully supported domain-specific language (DSL) for constructing diagram animations that can be rendered across multiple platforms. Canis requires the use of a data-rich SVG icon as the input format. By adding three attributes "id" (index), "class" (SVG element type), and "datum" (associated data) to each marker, designers can Select all visual tags to generate data-driven animations. This means that Canis can be applied to any chart created by any existing chart-building tool, as long as sufficient data is available.\cite{ge2020canis} Although the specification of Canis is simpler than the D3 code, it still requires basic programming knowledge. Based on Canis, researchers have come up with Cast, a tool for interactive chart creation, a visual specification for chart animation consisting of keyframes, which supports automatic complementary construction of keyframes and keyframe sequences. It also allows the user to refine the animation specification (e.g., adjusting keyframes to play together across tracks, adjusting delays) by changing other parameters of the animation effect through direct manipulation via the control panel.\cite{ge2021cast} Researchers have also designed and developed systems to create animated data graphics with no programming at all. Data Animator uses the Data Illustrator framework to analyze and match two static visual objects and automatically generate transitions by default. Designers have the flexibility to interpret and adjust the matching results through a visual interface. Data Animator also supports dividing complex animations into segments by layering keyframes and using data attributes to stagger the start time and change the speed of animated objects through a timeline view.\cite{thompson2021data}
 
\textbf{[Chart Export Phase]} In practice, charts are widely stored as bitmap images. Although it can be easily propagated for use, operations such as re-editing the chart to change the chart style or the data values in the chart is equivalent to redrawing a new chart, a process that is very time-consuming and error-prone. Therefore, Fu, J. et al. (2021) proposed a data embedding model, Chartem, which encodes a large amount of information into the background of the chart image without affecting the human perception of the chart itself. The embedded information, then, becomes an intrinsic part of the chart image, and the information of the chart image can be extracted by software for the purpose of reprocessing.\cite{fu2020chartem}
 
\textbf{[Dashboard]} Despite the growing interest and demand for visualization-driven analytics, these difficulties in terms of expertise or workload continue to hinder the creation and utilization of dashboards for a wide audience.\cite{ma2020ladv} In addition to the design and development of Authoring Tools for single charts, there has been considerable research on visualization systems for multiple charts in the same space, such as dashboards. Micheline Elias (2011) built a fully functional Exploration Views dashboard visualization system for novice users, which allows novice visualization users to easily build and customize business intelligence information dashboards, which provides an intuitive environment to dynamically create, rearrange, search, and explore multiple visual data representations from different data sources.\cite{elias2011exploration} Ma, R. (2021) proposed a method called LADV for efficient creation of visualization prototypes from dashboards or sketches. It is a web-based authoring tool for learning, combining and customizing dashboard visualizations in a cloud computing environment. It is not designed to generate a final product, but to propose a lightweight approach to rapid prototyping. The core idea of LADV is to automatically learn designs from examples, a new deep learning-based model that identifies and locates various categories of charts and extracts colors from the input image or sketch. Using LADV, novices can import dashboards for design by selecting an example from a collection to generate a dashboard template that can be applied and further customized interactively.LADV quickly converts the designer's concepts from sketches into usable dashboard presentations for rapid prototyping and evaluation. Thus reducing the burden of designing, implementing and evaluating dashboard visualizations.\cite{ma2020ladv}

\subsubsection{Glyph}
Chen, Z. et al. (2020) proposed MARVisT, a mobile AR visualization tool that uses information from reality to help non-experts deal with relationships between data and virtual symbols, real objects and virtual symbols, and real objects and data. Using MARVisT, users without visualization expertise can bind data to real-world objects to quickly and easily create expressive AR Glyph-based visualizations that redefine real-world representations with data.\cite{chen2019marvist}
Brehmer, M. et al. (2021) proposed the diatom technique, a technique for generating symbol design inspiration by sampling from a palette of marker shapes, coded channels, and symbol holder shapes, which the authors used as a Tableau plug-in to facilitate the creation of Glyph visual diagrams by practitioners.\cite{brehmer2021generative}

\subsubsection{Timeline}
Creating timeline infographics is a time-consuming task for novices, and users usually borrow Timelines that have already been designed online and apply them to their data. , Z. et al. (2020) address this problem by stating that there are two main challenges in this research, the first is how to make the computer understand the information in the Timeline, and the second is how to transform the images into editable templates based on the understood information. To solve the above challenges, the researchers propose two parts of deconstruction and reconstruction. The innovation combines a combination of more mature technical solutions from the industry. The current technology still relies on template-based creation, and future research directions can be improved towards a more liberal creation model.\cite{chen2019towards}
TimelineJS\cite{TimelineJS} and TimelineSetter\cite{TimelineSetter}, two common tools for creating Timelines, go a step further and generate slide presentations with a timeline with full descriptions of each event; using TimelineJS, the peripheral linear timeline serves as an interactive navigation aid, using panning transitions between successive narrative points.\cite{brehmer2016timelines} Fulda, J. et al. (2016) introduced TimeLineCurator, a browser-based authoring tool that allows processing unstructured text documents with temporal texts using natural language and extracting temporal texts from them and encoding them along a visual timeline. System administration features provide controls for managing and editing events on the timeline, the ability to combine timelines from multiple source documents, and export managed timelines for online deployment. The tool provides journalists and others who tell time stories with the process of creating timelines, greatly facilitating the management and processing of documents containing timelines.\cite{fulda2015timelinecurator}

\subsubsection{infographic}
Designing Infographics can be a tedious process for non-professionals and a time-consuming one even for professional designers. In the field of infographics, researchers have focused on how to combine Infographic and automation technologies. This is to reduce the difficulty of creating visual diagrams for non-specialists and to increase the speed and efficiency of diagrams for professionals.

\textbf{[Infographic Creation Tool]}Kim, N. W. et al. (2017) proposed Data-Driven Guidelines (DDG), a technique for designing expressive information graphics in a graphic design environment. It is mainly used to address the current design practice where designers manually encode data into custom graphics. Data guides are generated from data and can be manipulated directly for intuitive interaction. Free from being constrained by pre-defined templates or markers, designers can generate guides from data and use them to draw, place and measure custom shapes.\cite{kim2016data}
Sun, X. et al. proposed the Smart Pick-Paste tool, which utilizes existing infographics and can extract elements from the diagram into reusable templates that can be intelligently extracted and pasted into new infographics, reducing the difficulty of infographic redesign.\cite{sunsmart} Tyagi, A. (2021) proposed a flexible framework for automated and semi-automated infographic design. Based on this framework, the researchers developed Infographics Wizard to help novice designers create high-quality infographics by providing infographic suggestions for different design components.\cite{tyagi2021user} Lu et al. (2020) extracted the visual information flow of these images by analyzing a large number of infographics and used semi-automated techniques to extract design patterns of visual information flow from the dataset. Based on this, an infographic visual flow search tool, VIF-Explorer, was established. (Advantage) Using this tool, infographics can be searched based on selected or drawn VIF patterns, which both improves the efficiency of infographic search and facilitates the creation of narrative infographics. (Disadvantage) However, this software can only analyze simple infographics, and it is difficult to identify the flow of information in infographics that use many creative techniques and are too rich in content.\cite{lu2020exploring}
 
\textbf{[Tools for integration with PPT]}
In addition to designing in specialized visual authoring software, researchers have also developed tools that integrate with commonly used office software in the form of plug-ins to improve the problem of frequent software switching for practitioners. wang, Y. et al. (2018) proposed the InfoNice visual design tool that allows users to easily create data-driven infographics. InfoNice allows users to transform unmodified charts into infographics with multiple visual elements through custom markup. Researchers have integrated InfoNice into Microsoft Power BI, reducing the cost for designers to switch between data exploration and presentation.\cite{wang2018infonice} Cui, W. (2021) proposed Chartreuse, a hybrid active method for reusing infographics. chartreuse takes vectorized infographics as input and extracts chart models from them to help users quickly match new data sets. And the technology is integrated into PowerPoint and used to seamlessly reuse existing PowerPoint infographics templates. But Chartreuse is only suitable for creating bar charts and has significant limitations in the selection of charts.\cite{cui2021mixed}
By investigating a series of dynamic infographics, Yun Wang et al. (2021) pointed out that dynamic infographics mainly contain three aspects, which are infographic design elements (title, body, footnote, repeating unit, connector, unit title, unit description, unit index, unit icon, unit background), layout form (linear layout, radial layout, segmented layout, free layout ) and animation mode (simultaneous display, repeating unit by the unit display, similar element by element display). A reconstructed information structure algorithm is further proposed to follow the convention of animated infographic design, and infomation technique is proposed. And the infomation technique is applied to PowerPoint to transform a static infographic into a dynamic version through two steps of information structure extraction and animation choreography.\cite{wang2021animated}
Wang, Q. (2019) developed Narvis, an efficient, expressive, and user-friendly slide creation tool for introducing data visualization design, from a pedagogical perspective with teachers and students as the primary target groups. Teachers use Narvis to create tutorials explaining data visualization, and students use the tutorials to understand visualization design.\cite{wang2018narvis}
 
\textbf{[graphic combination]}
The combination of graphical and textual information can be applied in various domains, but there are difficulties in how to synthesize the two forms because they are spatially separated and the reader must switch back and forth in order to find a reference between the text and the visual markers on the graph encoding the data values. It imposes a significant cognitive burden on the reader's working memory and negatively affects learning. In response to this problem, Latif, S et al. (2021) investigated how to make a tight combination between text and graphs, and therefore developed Kori, a hybrid active system that enables the combination of text and graphs in an interactive way.\cite{latif2021kori} Cui, W. (2020) proposed the Text-to-Viz technique to generate corresponding infographics through textual descriptions in natural language, which can be divided into two core steps, the semantic parsing phase (for understanding how such information is described in people's everyday language) and the visual generation phase (layout, description, graphics, colors). Using this method it is possible to distill the right information for visualization and to ensure that the elements in the final infographic match harmoniously.\cite{cui2019text}
 
\textbf{[Creative Tools]}
Although these tools and applications can help designers generate data visualizations, the integration of custom symbols and layouts is usually somewhat limited due to the limitations of the tools themselves, and thus the resulting mostly common visual infographics hinder creative exploration and expression. Xia, H. et al. (2018) proposed DataInk, a pen and touch-enabled user interface that By using this system, designers can express their creative thinking by drawing on a digital canvas and bind their drawn graphics to data. This tool makes data visualization more creative by associating creative expression with data.\cite{xia2018dataink}
 
\textbf{[Infographic color]}
Yuan, L.P. et al. (2021) used deep learning techniques to build a recommendation engine to extract good color design practices from data and further developed the InfoColorizer tool, which allows ordinary users to design color palettes effectively using a data-driven approach in the infographics creation process. InfoColorizer also supports Some basic editing features that allow users to experiment with different infographics layouts, get corresponding palette recommendations, and iteratively refine their designs.\cite{yuan2021infocolorizer}
 
\textbf{[Summary]}
Creating an effective and aesthetically pleasing data visualization often requires cross-disciplinary skills, especially the ability to analyze data and graphic design at the same time, which is difficult for an average user without professional training. These cutting-edge technical studies help users generate visualizations through automated approaches to both data insights and design aesthetics, lowering the threshold for users to create visualizations and effectively improving productivity.

\subsubsection{Data Comic}
Data cartoons are a static form of visual narrative for storytelling, and researchers have conducted research to enhance the level of detail and potential user experience of data cartoons in conjunction with automation techniques.
Wang, Z., (2021) proposed a lightweight specification language, Comic Script, for designers to add interactivity to static comics, where users can add and remove panels in predefined panel layouts to support branching, change perspective, or get details on-demand, as well as provide the ability to modify data or interact with the data.\cite{wang2021interactive} Zhao, J. et al.(2021) proposed the ChartStory tool to produce data stories from a collection of user-created charts, using a comic panel-like style to suggest the underlying order and logic of the data-driven narrative. Data cartoon format, which can also be further refined and stylized through tools.\cite{zhao2021chartstory} Kang, D (2021) explored how to design computational notebooks to create more intuitive visual communication by integrating comic formats. ToonNote, an extension of JupyterLab notebooks, was developed with this purpose in mind, enabling readers to switch between notebook views and comic layout views.ToonNote integrates directly with notebooks and allows for linear or visually oriented narratives.\cite{kang2021toonnote} However, the software currently only allows the author to manually mark each cell to indicate which cells need to be converted to comic frames, thus potentially adding to the workload by causing a certain amount of repetition, which could be combined with automation technology on this program to ease the author's burden in creating an effective Data comic.
 
\subsubsection{Data Video}
With the diversification of media forms, Data Video becomes an effective form of narrative and becomes increasingly important in visualization efforts. Wang, Y. et al. (2016) proposed an animated narrative visualization system to present clickstream data of temporal videos. Clickstream data is important for understanding user behavior and improving online video services, and researchers refer to nonlinear temporal mapping methods and foreshadowing techniques. The nonlinear temporal mapping approach focuses on the interesting parts of the animation and compresses the uninteresting parts of the user into the background; the foreshadowing technique can attract viewers and remind them of the events in the animation, which are very helpful for improving the appeal of data videos.\cite{wang2016animated}
Amini, F. et al. (2017) developed DataClips, a web-based tool that allows data enthusiasts to write, edit, and assemble data clips to create data videos without programming skills, in order to reduce the difficulty of making data videos. Data-driven "clips" can be assembled together to form longer sequences. It has been experimentally demonstrated that non-expert users can learn and use DataClips in a short training time.\cite{amini2016authoring} D. Shi et al. (2021) designed and developed AutoClips, which can automatically generate data videos after entering a sequence of data facts.\cite{shi2021autoclips} Chen, Z. et al. (2021) focused on data visualization of ball videos in sports and derived a design space for enhanced sports videos featuring elements and clips through an extensive analysis of sports videos, and the four design dimensions of the design space (i.e., data type, visual type, data hierarchy, and narrative order) and their combined frequency provide data insights for various purposes (e.g., entertainment or education) to select and visuals provide guidance. Based on the requirements of the design space, the researcher designed and implemented Viscommentary, a proof-of-concept system that facilitates the creation of sphere-enhanced videos through data insights and visualization suggestions.\cite{chen2021augmenting}

\subsubsection{Storytelling}
Current visualization tools either lack support for storytelling or require significant technical expertise. Satyanarayan, A., \& Heer, J. (2014) Based on interviews with journalists, a model for writing linear and nonlinear data stories was proposed, on the basis of which Ellipsis was designed and developed, a system that combines a domain-specific language (DSL) for storytelling and a graphical interface for story creation. Users can tell stories without programming, and the system lowers the threshold for writing narrative visualizations.\cite{satyanarayan2014authoring} Sultanum, N. et al. (2021) explored a storytelling authoring approach for data-driven articles that separates semantics, textual graphical links, and the form of storytelling layouts. Based on this approach, the researchers constructed VizFlow, a concept creation tool for creating dynamic data-driven articles. Using Text-Chart Links to guide different storytelling layouts, static data-driven articles (with text and supporting charts) can be transformed into dynamic articles.\cite{sultanum2021leveraging} Wang, Y et al. (2019) proposed DataShot, a complete system for automatically generating visual information briefs, which can transform input tabular data into infographics through a 3-step process of fact extraction, fact combination, and visual synthesis.DataShot can effectively reduce the difficulty of data exploration and production of information briefs, and through expressive visual design to DataShot can reduce the difficulty of data exploration and information presentation, and enhance the readability of data through expressive visual design.\cite{wang2019datashot} Shi, D. et al. (2021) proposed the Calliope tool, a tool for automatically generating visual data stories from spreadsheets, which consists of two parts, a story generation engine, and a story editor. This tool lowers the threshold of Data Story creation by automatically generating usable data stories after users enter a table data. Unlike DataShot, which is randomly assembled, Calliope requires the entire story to be a coherent whole, with logical connections between the preceding and following pieces.\cite{shi2020calliope}
 
\textbf{[Word cloud]}
In addition, there are researchers who have improved word clouds to address the problematic points that they have. Word clouds are a form of visualization in which text words that occur with different frequencies in text data are size-coded and the coded words are arranged spatially on a canvas to achieve a quick understanding of the core points in the data for the viewer. Although widely used, word clouds suffer from two significant problems leading to the inability to effectively communicate stories. The first aspect is the inability to simultaneously illustrate the complex relationships between words, and the second is that as the narrative content evolves and a series of events drives the story in time and cause and effect, the word cloud loses temporal information for the story as a whole.
Through exploratory research, Cui, W. et al. (2020) proposed an initial design space for animated word clouds to tell potential stories, and the researchers identified key narrative elements, proposed a set of design factors, and summarized design goals. Based on the design space, the DancingWords authoring tool was developed to allow users to explore the narrative and generate interactive animations with the automatic layout.\cite{cui2019text}

\subsection{Summary}
In the field of visual design in the digital age, graphic design is not only characterized by visual interactivity and semantic versatility, but also has new developments in the form of graphic design creation tools, creation process, presentation, and design expressions. In order to lower the design and use threshold of visualization, promote the popularity of visualization, and integrate visual creation into daily life, researchers have proposed many visual creation tools. In this section, we investigate Authoring tools in the field of visualization and see that researchers have made efforts to optimize various aspects of the visualization design process, starting from the processing of data after obtaining them, to how to create visualizations easily, and how to optimize the layout of visualizations.

The development of digital technology has greatly reduced the cost of authoring tools, and the Internet provides the most convenient distribution channel for this purpose. The combination of the three has significantly lowered the threshold of creation. We also find that static types of visualization, whether charts, infographics, or data cartoons, are evolving to the interactive level, and are mostly focused on narrative research. Secondly, most of the authoring tools can only create some common visual infographics, and there is less research on tools for creative thinking expression. Therefore, in future work, in addition to strengthening research on narrative visualization to present visualization charts in the form of stories, research on how to combine data visualization with creative thinking needs to be strengthened to support more art designers to jointly participate in visualization scenarios development.


==> archive.tex <==
\subsection{Visualization tools}
Researchers have combined programming techniques to make various improvements to address some of the problems in the field of visualization. Henry, N., et al. (2007) addressed the inability of visualization systems to display both the readability of the global structure of the network and the local information in detail by proposing the \textit{NodeTrix technique}, a hybrid representation of the network that uses a node connectivity graph to display the global structure of the network and Any part of the network shows the adjacency matrix.\cite{henry2007nodetrix} Dunne, C., & Shneiderman, B. (2013) proposed a \textit{pattern simplification technique}, which is mainly designed to improve the problem of complex node connectivity graphs that take up too much screen space.\cite{dunne2013motif} To facilitate visual design practitioners to retrieve various visual design graphics more efficiently, Hoque, E (2020) proposed a \textit{D3 visualization search engine} that can index D3 visualizations based on visual style and underlying structure.\cite{hoque2019searching}
To facilitate faster and more efficient data visualization design for practitioners and general users, researchers have developed visualization design tools for different forms of visualization.

\subsubsection{Charts}
Micheline Elias (2011) built a fully functional Exploration Views dashboard visualization system for\cite{elias2011exploration} novice users that allows novice visualization users to easily build and customize business intelligence information dashboards by providing an intuitive environment for dynamically creating, rearranging, searching, and exploring multiple visual data representations from different data sources. visual data representations. Ren, D (2017) describes how to help presenters quickly and easily refine their charts with a variety of annotations. A design space for chart annotation is described, and using this design space, \textit{Chart Accent,} an interactive tool that allows one to manually generate data annotations, was developed. This tool provides a new way to define and use data-driven annotations.\cite{ren2017chartaccent} It is very helpful in improving the readability and comprehensibility of charts. And Ren, D (2019) in another study presented the Charticulator tool (with actual software), a framework that can be used to create a wide range of charts. This is an interactive chart creation tool for specifying custom and reusable chart layouts.Charticulator translates chart specifications into mathematical layout constraints and uses a constraint resolution algorithm to automatically compute a set of layout properties to implement the chart. Thanks to the constraint-based layout approach, it is possible to export chart designs as reusable templates or to import them to other visualization tools for re-editing.\cite{ren2018charticulator} However, the software has an obvious limitation in that it only supports first-level repetition in chart segments, so the granularity of the data must be predetermined by the chart creator. To address this limitation, the researcher also noted a desire to extend our framework in two ways. First, a data transformation pipeline could be added to the segment level; by specifying a set of data transformations, the chart creator would be able to aggregate the data to the desired granularity. Second, and more importantly, a Glyph can be allowed to be designed as a nested diagram. Thus, an important direction for future research is to envision new forms of interactive tutorials to facilitate self-learning for highly definable user interfaces like Charticulator.

\subsubsection{Glyph}
Brehmer, M. et al. (2021) proposed the diatom technique, a technique for generating symbol design inspiration by sampling from a palette of marker shapes, coded channels, and symbol holder shapes, which the authors used as a Tableau plug-in to facilitate the creation of Glyph visual diagrams by practitioners.\cite{brehmer2021generative}

\subsubsection{infographic}
In the field of infographics, researchers have focused on how to combine Infographic with automation techniques. Cui, W. (2020) proposed the Text-to-Viz technique to generate corresponding infographics through textual descriptions in natural language, which requires understanding the user input text, extracting the correct information for visualization, and ensuring that the elements in the final infographic match harmoniously. The method can be divided into two core steps, the semantic parsing phase (for understanding how such information is described in people's everyday language) and the visual generation phase (layout, descriptions, graphics, colors). The method generates high-quality infographics that are suitable for practical business and personal applications.\cite{cui2019text} Lu et al. (2020) extracted the visual information flow of these images by analyzing a large number of infographics and used a semi-automated technique to extract the design patterns of visual information flow from the dataset. Based on this, an infographic visual flow search tool, VIF-Explorer, was established. (Advantage) Using this tool, infographics can be searched based on selected or drawn VIF patterns, which both improves the efficiency of infographic search and facilitates the creation of narrative infographics. (Disadvantage) However, this software can only analyze infographics with simple content, and it is difficult to determine the information flow characteristics of infographics that use many creative techniques and are too rich in content.\cite{lu2020exploring} Yun Wang et al. (2021), by investigating a series of dynamic infographics, pointed out that dynamic infographics mainly contain three aspects, which are infographic design elements (title, body, footnote, repeating unit, connector, unit title, unit description, unit index, unit icon, unit background), layout form (linear layout, radial layout, segmented layout, free layout ) and animation mode (simultaneous display, repeating unit by unit display, similar element by element display). A reconstructed information structure algorithm is further proposed to follow the convention of animated infographic design, and infomotion technique is proposed. And the infomation technique is applied to PowerPoint to transform a static infographic into a dynamic version through two steps of information structure extraction and animation choreography.\cite{wang2016animated}
\textbf{[Summary]}
Creating an effective and aesthetically pleasing data visualization often requires cross-disciplinary skills, especially the ability to analyze data and graphic design at the same time, which is difficult for an average user without professional training. These cutting-edge technical studies help users generate visualizations through automated approaches to both data insights and design aesthetics, lowering the threshold for users to create visualizations and effectively improving productivity.

\subsubsection{Data Comics}
Data Comics are a static form of storytelling visual narrative, often presented in paper form, that researchers have studied in order to enhance the level of detail and potential user experience of data comics in conjunction with automation technologies. Wang, Z., (2021) proposed a lightweight specification language - Comic Script - for designers to add interactivity to static comics, often in paper form, and for users to add and remove panels in predefined panel layouts to support branching, changing perspectives, or getting details on demand, as well as providing the ability to modify data or interact with data. -Comic Script, for designers to add interactivity to static comics, where users can add and remove panels from a predefined panel layout to support branching, change perspective, or get details on demand, as well as provide the ability to modify or interact with the data.\cite{wang2021interactive}
Kang, D (2021) explores how computational notebooks can be designed to encourage clearer communication by integrating a comic format. ToonNote, an extension of JupyterLab notebooks, was developed with this purpose in mind, enabling readers to switch between typical notebook views and comic layouts. Using ToonNote enables a higher degree of certainty about the author's ideas and insights than reading computational notebooks alone.ToonNote offers some inherent benefits that other formats do not have or lack, such as direct integration with notebooks or a linear, visually oriented narrative. However, the software currently only allows authors to manually mark each cell to indicate which cells need to be converted to comic frames, which can create a certain workload, so it is possible to combine this program on with automation techniques to ease the burden on authors in creating an effective data comic.\cite{kang2021toonnote}

\subsubsection{Data Video}
With the diversification of media forms, Data Video becomes an effective form of narrative and becomes increasingly important in visualization efforts. Wang, Y. et al. (2016) proposed an animated narrative visualization system to present clickstream data of temporal videos. Clickstream data is important for understanding user behavior and improving online video services, and researchers refer to nonlinear temporal mapping methods and foreshadowing techniques. The nonlinear temporal mapping approach focuses the interesting parts of the animation and compresses the uninteresting parts of the user into the background; the foreshadowing technique can attract viewers and remind them of the events in the animation, which are very helpful to improve the appeal of data videos.\cite{wang2016animated} D. Shi et al. (2021) introduced a new method, AutoClips, in order to lower the threshold for creating data videos, which automatically generates data videos after entering a sequence of data facts.\cite{shi2021autoclips}

\subsubsection{Timeline}
Creating timeline infographics is a time-consuming task for novices, and users usually borrow Timelines already designed online and apply them to their own data, so researchers have addressed this need to extract editable templates from existing Timeline images for their own creation. Chen, Z. et al. (2020) address this problem by stating that there are two main challenges in this research, the first is how to make the computer understand the information in the Timeline, and the second is how to transform the images into editable templates based on the understood information. To address these challenges, the researchers propose two parts: deconstruction and reconstruction. The innovation that combines a combination of more mature technical solutions from the industry. The current technology still relies on template-based authoring, and future research directions could be improved towards a more free-form authoring model.\cite{chen2019towards}
TimelineJS(Northwestern University Knight Lab,2013) And TimelineSetter[A. Shaw.et al , 2011] are two of the tools that go a step further and generate slide presentations with a timeline with full text descriptions of each event; using TimelineJS, the peripheral linear timeline acts as an interactive navigation aid, using panning transitions between successive narrative points.

\subsubsection{storytelling}
Wang, Y et al. (2019) proposed DataShot, a complete system for automatically generating visual information briefs that can transform input tabular data into infographics through a 3-step process of fact extraction, fact combination, and visual synthesis.DataShot can effectively reduce the difficulty of data exploration and production of information briefs, and through expressive visual design to DataShot can reduce the difficulty of data exploration and information presentation, and enhance the readability of data through expressive visual design.\cite{wang2019datashot} Shi, D. et al. (2021) proposed the Calliope tool, a tool for automatically generating visual data stories from spreadsheets, which consists of two parts, a story generation engine and a story editor. This tool lowers the threshold of Data Story creation by automatically generating usable data stories after users enter a table data. Unlike DataShot, which is randomly assembled, Calliope requires the entire story to be a coherent whole, with logical connections between the preceding and following pieces.\cite{shi2020calliope}

\subsection{Summary}
\textbf{[Problem points of existing studies]} Through the systematic analysis of visualization cognitive level, visualization design guidelines, and design practices, we found that the current visualization design guidelines still have some disadvantages. Firstly, there are \textit{too many design guidelines, which makes it difficult to choose}, and the complexity of design guidelines increases the cost of learning and reduces the efficiency of retrieval; secondly, \textit{some guidelines do not further explain under what circumstances it is more appropriate to use, but only present ideas and provide validation.} Visual coding methods should be carefully designed to achieve a trade-off between interpretability and simplicity.\cite{tang2020design}
\textbf{[Future Work]}
For example, the \textit{guidelines should be categorized} to reduce the search time and improve the search efficiency; the \textit{design guidelines should be integrated with specific design problems and combined with the design purpose,} so that novices can search the design guidelines directly through the design problems.\cite{tang2020design}
From the study of literature such as visualization design guidelines, we can see that visualization design guidelines are only a guideline, not a rule. We can use visualization design guidelines to design according to the actual situation, but we cannot use the design guidelines as a standard to measure the design. Visualization design guidelines are a starting point for designers, not an end point, that is, if one lacks sufficient experience in the visualization field, then using visualization design guidelines will make the design better in most cases, and as a mature visualization designer, one does not need to follow the visualization guidelines dogmatically, but should focus more on the subtle aspects of visualization design that can improve It is more important to focus on the subtle design that can improve user experience and user perception.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/03-Dashboard.tex <==
\section{Dashboard} %20220322版本
\begin{figure*}[htp]%[hbt!]
%\setlength{\abovecaptionskip}{-0.01cm}
\setlength{\belowcaptionskip}{-0.1cm}
    \centering
    \includegraphics[width=16.5cm]{Figure/01-dashboard.png}
    \caption{Selected examples of dashboard's design spaces and tools. (1) Design space: Sarikaya et al. \cite{sarikaya2018we} proposed seven dashboard types. (2) Authoring tool: Tableau's \cite{tableau2006} Working Window. (3) AI-supported Tool: LADV's \cite{ma2020ladv} system architecture. LADV\cite{ma2020ladv} provides a web-based interface for users to upload dashboard images or sketches as examples reformulated into dashboard templates. (4) AI-generator tool: Sisense \cite{SisenseFusionAnalytics2019} is an integrated, end-to-end analytics and BI platform that provides visual data exploration, dashboards, and advanced analytics capabilities.}
   % \label{fig:figures2.11} %交叉引用的标签
   \vspace{-2mm}
\end{figure*}

\begin{wrapfigure}{l}{0.055\textwidth}
  %\begin{center}
    \includegraphics[width=0.055\textwidth]{Figure/icon/icon-dashboard.png}
  %\end{center}
\end{wrapfigure} 

% 概念
Dashboards usually use a tiled chart layout to display data from multiple perspectives, revealing changes and connections between different data. Dashboards are commonly used in analysis and testing scenarios such as decision analysis and real-time monitoring \cite{few2007dashboard,park2015development}.

{\textbf{Design Space:}}
%Dashboards are ubiquitous and essential in a data-driven world. They are widely used in business, healthcare\cite{faiola2015supporting}\cite{wilbanks2014review}, and teaching\cite{bajzek2007inventing}\cite{sedrakyan2019guiding}\cite{molenaar2018teachers}. While driving the rapid development of dashboards, different dashboards have been generated. Sarikaya et al.\cite{sarikaya2018we} described seven significant types of dashboards through their design goals, interaction methods, and application scope. They proposed a design space beyond visual coding principles to construct a dashboard from design dimensions such as functional design, purpose, audience, and data semantics.  
With the prevalence of visualization techniques and tools, different dashboards have been designed and implemented in various domains \cite{faiola2015supporting, sedrakyan2019guiding}. Sarikaya et al. \cite{sarikaya2018we} described seven main types of dashboards through their design goals, interaction styles, and application scope. %And constructed the design space of the dashboard in terms of design dimensions such as functional design, purpose, audience, and data semantics.
%Effective design is crucial and challenging for creating dashboards \cite{sarikaya2018we}.
Designing a good dashboard requires three key considerations: understanding the data, making design decisions for proper data presentation, and visual aesthetics \cite{ma2020ladv}.
First, the \rv{designers need} to know the user community to clarify and understand the data.
Before developing a dashboard, designers need to decide the dashboard components and interaction behaviors according to the user's needs \cite{vazquez2019extending}. Second, to correctly present data for making design decisions, the size and density of the data content should be considered before choosing a dashboard layout \cite{froese2016lessons}. %Designers need to access and understand the data during the requirements gathering phase, so that visual design prototypes can be created more quickly and correct design decisions can be made. 
Finally, \rv{designers need} to pay attention to the visual aesthetics of the dashboard, such as the layout of the panel and the use of colors. Javed \& Elmqvist \cite{javed2012exploring} proposed four visual combinations of parallel, stacked, overloaded, and nested views of charts \rv{and discussed the advantages}, disadvantages, and application scenarios of different views. Chen et al. \cite{chen2020composition} presented the design space of the dashboard in terms of the relationship between view types, popular view layouts, and the correlation between view types and layouts.
%Chen et al. \cite{chen2020composition} provided a fine-grained annotation of view types and layouts for a large number of visual images, using quantitative metrics of term frequency and layout topology for composition and configuration analysis. The final design space of the dashboard was identified, which includes the relationship between view types, popular view layouts, and the correlation between view types and layouts. 
Qu \& Hullman \cite{qu2017keeping} developed a set of coding constraint models for detecting multi-view consistency that allows designers to spontaneously maintain consistent coding during multi-view creation. Apart from research on visual layout, color encoding is another important aesthetic factor.
For example, Gramazio et al. \cite{gramazio2014relation} studied how visual markers' color layout, number, and size affect the user's visual search time. %The results show that the number of features does not affect the visual search time when the colors are regularly grouped on the screen, but it has a more substantial effect when the colors are randomly placed.
In addition to the above three aspects of how to design a good dashboard, recent studies pointed out that the lack of narrative elements might be one of the reasons why many designers failed to create effective dashboards \cite{suprata2019data, fernandez2022beyond}.
% Creating dashboards with narrative properties should consider the narrative structure, such as the Pyramid Model \cite{berezhnaya2019data} (exposition, rising action, climax, falling action, denouement).
Suprata \cite{suprata2019data} proposed that the process of creating a dashboard with narrative properties is defining the audience, framing insights, establishing the setting or context, focusing on storytelling elements, and consolidating practices. In practice, Fernandez Nieto et al. \cite{fernandez2022beyond} enhanced the teacher's guidance of the content by including narrative attributes in designing learning analytics dashboards.
%Traditional visual design guidelines often focus on a single view rather than multiple views. However, such design guidelines that consider only a single view can ignore the overall layout of multiple views and coding consistency among multiple charts. The design space studies of dashboards investigate issues related to multi-view layout, coding consistency, color combination from the perspective of visual aesthetics. 
Adding narrative attributes to a dashboard can not only uncover more data insights but also increase user engagement and make the visualization more expressive. %However, all these studies are carried out from the theoretical level of creating dashboards, which requires users to have visualization expertise to understand and apply these guidelines, so as to hinder the creation and utilization of the dashboard by a broad audience \cite{ma2020ladv}.

{\textbf{Authoring Tool:}}
With the growing interest and demand for data-driven visual analytics, researchers have developed a series of authoring tools for creating dashboards. Tableau \cite{tableau2006}, the most common tool for creating dashboards, incorporates Tableau Story to generate narratives of dashboards. Spotfire \cite{ahlberg1996spotfire} provides a flexible drag-and-drop interface for instant customization of visualizations. However, the above tools have a significant learning curve and are not user-friendly for novice users. 
Elias \& Bezerianos \cite{elias2011exploration} found significant differences in interface creation and interaction styles between expert and novice users. Expert users require the support of detailed data exploration, while novice users mainly used dashboards for data communication and reporting.
% Due to the different familiarity with visualization between the two groups, visualization tools for novice users need to meet three conditions: (1) provide user-friendly data input for standard data formats; (2) automatically provide visualization or reasonable defaults based on data type; and (3) use contextual information to clarify the displayed data and coding. 
Based on this finding, they developed Exploration Views, which provides an intuitive environment for dynamically creating, rearranging, searching, and exploring multiple visual data representations from different data sources. 
In another work \cite{elias2012annotating}, the researchers developed a prototype dashboard supporting data and context-aware annotations for business intelligence (BI) dashboard environments. %The prototype is built on a shared data layer between different data sources and BI applications.%, and can be annotated across applications.

%Authough these authoring tools allow users to create dashboards that match the data types by simple dragging or clicking interactively, using these tools also requires basic visualization expertise and data analysis knowledge, and some authoring tools have a certain learning curve. Even for expert users, it is not easy to analyze and create excellent visualizations for different fields and data types.

{\textbf{AI-supported Tool:}}
In most cases, dashboards are directly presented to the end users, without considering their cognitive abilities, preferences, and needs. Belo et al. \cite{belo2014restructuring} proposed adaptive dashboards, where the dashboard monitors all the actions the user does on the dashboard and automatically reorganizes it into a new dashboard based on the user's usage. However, most ML/AI-supported tools for dashboard creation cannot generate dashboards for different users. Therefore, researchers have developed domain-oriented dashboard creation tools. For example, QualDash \cite{elshehaly2020qualdash} is a tool for generating dashboards in the healthcare domain to improve the quality of care by dynamically configuring and deploying visual dashboards. Dabbebi et al. \cite{dabbebi2017towards} built a dashboard generator for learning analytics based on a set of models, which supports the process of learning contextual dashboard design. 
To further ease the burden of creating dashboards, Ma et al. \cite{ma2020ladv} proposed LADV, a tool based on a deep learning scheme that can quickly transform bitmaps containing statistical charts or sketches drawn by designers into editable dashboards and support further interaction. 

%Compared with authoring tools, ML/AI-supported tools reduce the  difficulty of creating professional dashboards, and it is more targeted at the target users and can enhance the user experience.

\textcolor[RGB]{39,47,107}{\textbf{AI-generator Tool:}}
Apart from ML/AI-supported tools, some work supports the fully automatic process from data processing to the final presentation in the dashboard \cite{datapine2012, SisenseFusionAnalytics2019, thoughtspot2012, QlikSense2010}. Datapine \cite{datapine2012} provides different forms of dashboard templates from three aspects: function, industry, and platform, with a large number of built-in databases that can generate real-time dashboards and provide user interaction and collaborate with data. Sisense \cite{SisenseFusionAnalytics2019} is an integrated, end-to-end analytics and BI platform that simplifies complex data in a short time, providing data exploration, dashboard presentation, and embedded advanced analytics. Thoughtspot \cite{thoughtspot2012} applies a search-based visual analytics approach that can respond to billions of rows of searches. It also supports SpotIQ, an AI-driven analytics tool that allows users to run it directly on query data results and then use statistical and machine learning algorithms to discover data anomalies, trend lines, clusters, and other data characteristics. 
Apart from providing advanced automatic analytics techniques, Qlik sense \cite{QlikSense2010} offers a complete visualization system, supporting global search to optimize context and the ability to add annotations to facilitate dashboard storytelling. %The tool also supports loading multiple datasets, finding columns with something in common, and matching the data accordingly, which saves users much time in data analysis process. 

%Compared with ML/AI-supported tools, existing AI-generator tools for dashboard creation further helped with data processing and insight detection such as finding outliers, trends, and other potential information in the data. These tools are not only suitable for data analysts, but also enable visualization practitioners and novice designers to explore data in-depth and present the visualization more effectively.

\textbf{Summary:} Dashboards are ubiquitous and essential in a data-driven world \cite{sarikaya2018we}. Based on the above analysis, we found that researchers are exploring how to design a good dashboard from a global perspective at the design space level. The Authoring tool level mainly aims at practitioners with expertise in data analysis or visualization. For ML/AI-supported tools, the focus is on creating dashboards for specific contexts in specialized domains. For AI-generator tools, the current applications are mostly for BI platforms, which can present visualization information for data analysts and visualization practitioners. However, at any level of automation, designers need to pay attention to the preferences (data of interest to users) and other characteristics (background, expertise, literacy) of the target users in the pre-creation phase \cite{sarikaya2018we}. While dashboards present multiple visualizations together, some complex charts (e.g., parallel coordinate charts, sankey charts) could not provide a better \rv{user} experience for users \cite{froese2016lessons}. A potential research direction is how to simplify complex charts and extract only the core component for a better presentation of content in a dashboard. Moreover, although studies have been proposed to use dashboards for narrative visualization, such studies are still in the initial stage \cite{suprata2019data}. In the future, more research is still required to explore how to better apply narrative tactics through dashboards.
%In future work, the following areas can be focused on.
%First, dashboards combine multiple charts, but some complex charts (e.g., parallel coordinate charts, sankey charts) do not provide a better cognitive experience in a dashboard \cite{froese2016lessons}. A potential research direction is how to simplify complex charts and extract only the core content for a better presentation of content in a dashboard.
%Second, annotation is an essential part of visualization; we can use annotations to link and organize multiple charts related to their analysis, discover charts and annotations through annotation recommendations, understand the reasons behind them, and use annotation context to discover information outside the system \cite{elias2012annotating}. However, existing research on dashboard annotations is still lacking, so there is a need to strengthen this direction.
%Third, research work on adaptive dashboards is gradually increasing, but many design details of dashboards have not been sufficiently studied. Applying artificial intelligence techniques for mechanical design and development of dashboards \cite{vazquez2019information, suprata2019data}, automatic selection of suggested visualization concepts/diagrams, and automated extraction of essential parameters of data sets can better solve the problem of adaptive dashboards.
%Third, although studies have been proposed to use a dashboard for narrative, such studies are still in the initial stage \cite{suprata2019data}. In the future, user research on dashboards is still required to explore how to better apply narrative tactics through dashboards. %In this way, users' visual perceptions of the dashboard change?



==> sections/10-FutureNarrativeVisualization.tex <==
\section{Future Narrative Visualization}

\begin{figure*}[htp]%[hbt!]
\setlength{\abovecaptionskip}{-0.01cm}
\setlength{\belowcaptionskip}{-0.3cm}
    \centering
    \includegraphics[width=16cm]{Figure/09-narrative.png}
    \caption{On the left is an example of Immersive narrative; on the right is an example of physicalization. (1)The 3D parallel coordinate visualization in augmented reality is fixed on a touchable desktop screen where the user can conveniently manipulate it \cite{butscher2018clusters}. (2) DXR \cite{sicat2018dxr} enables rapid prototyping of immersive data visualization. Users can quickly iterate over visualization parameters with DXR's graphical user interface. (3) (a) and (b) are tools for creating physical visualizations, and (c) is a physical visualization created by the researcher \cite{karyda2020narrative}. (4) physicalization example. Non-experts can build understandable visualizations by arranging simple symbols \cite{huron2014constructing}.}
    \vspace{-2mm}
\end{figure*}

Apart from common narrative visualization genres, researchers have proposed some other types of narrative visualization to enhance human perception in recent years. %Visualizations can enhance human perception in a variety of ways. 
Willett et al. \cite{willett2021perception} describe common underlying visual, perceptual, and cognitive mechanisms that form the basis of many action abilities, as well as how visualizations and other cognitive tools can give those who use them as an enhanced ability to achieve goals. %The conceptual framework demonstrates a variety of visual and cognitive mechanisms (including visual association, enhanced computational abilities, and enhanced comparative abilities) that can be used to examine existing visualization systems and critically envision new ones. 
The researchers envisioned seven capabilities that could enhance human perception. They explored seven dimensions of scope, access, spatial relevance, temporal relevance, information enrichment, degree of control, and environmental reality that could change people's sense of empowerment and agency. From the perspective of environmental reality, we introduce two emerging visualization \rv{genres} which could be related to visual narrative and storytelling: immersive visualization and data physicalization.

%\subsection{Immersive visualization}

\textbf{Immserive Visualization(IV):} Immersion refers to a specific phenomenon that describes people's experience when exposed to a specific medium, such as books, movies, or games. However, When immersive is used with visualization, it usually refers to 3D visualization in a virtual reality environment \cite{isenberg2018immersive}. Because immersive visualization can exponentially improve the efficiency of desktop visualization, it is becoming a potential foundation for exploring the high levels of data dimensionality and abstraction \cite{donalek2014immersive}. There are many factors to consider when designing visualizations in an immersive environment, such as occlusion, clutter, user movement and interaction \cite{bach2017drawing}. Liu et al. \cite{liu2020design} explored 2D small multiples visualization on a flat-screen applied to 3D immersive spaces. %Moreover, the layout design space's proposed dimensions, curvature, aspect ratio, and orientation. It is shown through user studies that the performance of different layouts depends on the number of display multiples. If the number is small, flat layouts perform better, and as the number of multiples increases, users prefer semicircular layouts over fully wraparound or flat layouts. 
Vierjahn et al. \cite{vierjahn2017towards} proposed a design space for describing IV workflow from six dimensions: frequency, users, interactivity, hardware, availability, and costs. This design space supports system designers in integrating VR technologies into IV workflows to facilitate seamless IV.
However, only a few visualization \rv{genres} (3D scatterplots \cite{bach2017hologram}, parallel coordinates \cite{butscher2018clusters}, and network \cite{cordeil2016immersive}) have been applied to immersive in the existing studies. Filonik et al. \cite{filonik2016glance} proposed Glance, a GPU-based framework focused on fast and efficient rendering of abstract visualizations in AR and VR. Butscher et al. \cite{butscher2018clusters} proposed the ART system that can transform multiple scatter plots into a multidimensional data visualization in AR and connect the data points to form a 3D parallel coordinate visualization. The system is anchored to a touchable tabletop, which allows for fluid interaction. DXR \cite{sicat2018dxr} is a Unity-based toolkit for building immersive visualizations with reusable visualization libraries such as scatter plots, histograms, and flow visualizations that can be linked by sorting and linking. The system also provides a GUI interface that allows users to immerse themselves in the virtual world to easily and quickly edit and preview visual designs. %Donalek et al. \cite{donalek2014immersive} developed iViz, which provides a GUI for specifying visualization parameters for a collaborative VR analysis environment. These tools all require a vehicle (touchable desktop, screen, etc.) to display visualization information and interact with it. 
ImAxes \cite{cordeil2017imaxes} is a VR system for exploring multivariate data without menus or hotkeys; users can create scatterplots and parallel coordinates by directly manipulating objects in the virtual environment. %They can be explored and reconfigured through embedded interactions. 


%Immersive techniques allow users to perceive space better. Immersive interaction provides natural and direct interaction with data in an AR or VR environment, making the data more attractive and insightful. Although there have been related studies on immersive visualization, only three types of visualization, scatterplot, parallel coordinates, and network in immersive environments, have been studied, and other types of visualization, such as time series or graphical data, need to be investigated. Since immersive visualization can have the problems of occlusion and clutter in virtual environments, potential future research directions on Immersive visualization are to explore more deeply the data types, spatial layout, and user interaction in virtual environments.

%\subsection{Data physicalization}
\textbf{Data Physicalization} refers to ``physical artifacts whose geometry or material properties encode data'' \cite{jansen2015opportunities}. Karyda et al. \cite{karyda2020narrative} argues that data physicalization is felt with the body and can be used as a ticket to speak in everyday situations, allowing for reflection through physical engagement and spoken exchanges.
Data physicalization is explicitly concerned with the tangible and material features of physical data representation. It focuses on data-driven tasks such as data exploration and data communication \cite{dragicevic2020data}. Dragicevic et al. \cite{dragicevic2020data} discussed different application areas of data physicalization, elaborating on how it can be used for analysis, communication and education, accessibility, self-reflection, self-expression, etc. % It also mentions that creating data physicalization has three components: digital fabrication, actuation technologies, and specialized applications for creating data physicalization; and summarizes models and theories of data physicalization. 
Djavaherpour et al. \cite{djavaherpour2021data} surveyed the rendering process of data physicalization from digital design to digital fabrication. Karyda et al. \cite{karyda2020narrative} proposed the concept of narrative physicalization. Narrative physicalization draws on narrative visualization, enabling people to develop meaningful narratives around data and personal experiences. Narrative physicalization effectively leverages the ability of objects to provide and the fact that people know how to use them. Through narrative physicalization, people's reflective processes are enhanced.
Data physicalization promises to facilitate a more refined perception than traditional forms of information visualization \cite{hogan2013touch}. Several researchers argued that data physicalization to encode information in a perceptible form would gain more freedom because it can utilize various physical, material, and tangible features that humans can explore using all their senses and motor skills \cite{hogan2017towards, jansen2015opportunities}. However, research in data physicalization is still in its infancy and needs to be encouraged in the future to better understand its design space, and the benefits compared to traditional 2D visualization or 3D visualization in the virtual space \cite{dragicevic2020data}.


%Many researchers have conducted research related to the physicalization of data. Data physicalization is "the physical artifact whose geometry or material properties encode the data"\cite{jansen2015opportunities}. Karyda et al.\cite{karyda2020narrative} argues that Data physicalisation is experienced through the body and may become a ticket-to-talk in daily encounters facilitating reflection through physical interaction and speech encounters. The physicalization of data shares many research questions with visualization, but it is explicitly concerned with physical data representation's tangible and material characteristics. It focuses on data-driven tasks, such as data exploration and data communication. Dragicevic et al.\cite{dragicevic2020data} discusses the different application areas of data physicalization, elaborating on how it can be used for analysis, communication and education, accessibility, self-reflection, self-expression, etc. It also mentions three ways of creating data physicalizations: digital fabrication, actuation technologies, and specialized applications for creating data physicalizations, and summarizes the model and theory of data physicalization. Karyda et al.\cite{karyda2020narrative} refers to the concept of narrative physicalization. Narrative physicalization draws on narrative visualization, which allows for a meaningful narrative around data and personal experiences. Narrative physicalization effectively leverages the object's ability to provide and that people know how to use the object. Through narrative physicalization, people's reflective processes are enhanced.

\textbf{Summary:}
Immersive technologies allow users to perceive space better. Immersive interaction is natural and direct with data in an AR or VR environment, where help users gain more engagement and insights. While there is emerging research in immersive visualization, the design and application around visual narratives in immersive environment has not been sufficiently studied.  %only three visualization types, scatterplot, parallel coordinates, and network, have been studied so far. Other visualization types, such as time series or graphical data, need to be investigated. 
%Since immersive visualization can suffer from occlusion and clutter in virtual environments, it also requires exploration of data types, spatial layout, and user interaction in virtual environments.
Meanwhile, data physicalization is expected to facilitate a more granular form of perception than traditional forms of information visualization. Several researchers have argued that physicalizing data and encoding information in the perceptible form is potentially more freeing. This is because it can utilize various physical, material, and tangible features that humans can explore using all their senses and motor skills. There is still an urgent need for more fundamental research in data physicalization to better understand its design space and the practical benefits compared to flat or virtual presentations.
In summary, both immersive technology and data physicalization are new forms of visualization in terms of representation and interaction methods. Therefore, more opportunities are left for researchers to explore the narrative theories and tools of such emerging visualization genres. 
